texTENG: Fabricating Wearable Textile-Based Triboelectric Nanogenerators

Recently, there has been a surge of interest in sustainable energy sources, particularly for wearable computing. Triboelectric nanogenerators (TENGs) have shown promise in converting human motion into electric power. Textile-based TENGs, valued for their flexibility and breathability, offer an ideal form factor for wearables. However, uptake in maker communities has been slow due to commercially unavailable materials, complex fabrication processes, and structures incompatible with human motion. This paper introduces texTENG, a textile-based framework simplifying the fabrication of power harvesting and self-powered sensing applications. By leveraging accessible materials and familiar tools, texTENG bridges the gap between advanced TENG research and wearable applications. We explore a design menu for creating multidimensional TENG structures using braiding, weaving, and knitting. Technical evaluations and example applications highlight the performance and feasibility of these designs, offering DIY-friendly pathways for fabricating textile-based TENGs and promoting sustainable prototyping practices within the HCI and maker communities.

==> ACM_Files/ACM-draft.tex <==
\section{Introduction}
ACM's consolidated article template, introduced in 2017, provides a
consistent \LaTeX\ style for use across ACM publications, and
incorporates accessibility and metadata-extraction functionality
necessary for future Digital Library endeavors. Numerous ACM and
SIG-specific \LaTeX\ templates have been examined, and their unique
features incorporated into this single new template.

If you are new to publishing with ACM, this document is a valuable
guide to the process of preparing your work for publication. If you
have published with ACM before, this document provides insight and
instruction into more recent changes to the article template.

The ``\verb|acmart|'' document class can be used to prepare articles
for any ACM publication --- conference or journal, and for any stage
of publication, from review to final ``camera-ready'' copy, to the
author's own version, with {\itshape very} few changes to the source.

\section{Template Overview}
As noted in the introduction, the ``\verb|acmart|'' document class can
be used to prepare many different kinds of documentation --- a
dual-anonymous initial submission of a full-length technical paper, a
two-page SIGGRAPH Emerging Technologies abstract, a ``camera-ready''
journal article, a SIGCHI Extended Abstract, and more --- all by
selecting the appropriate {\itshape template style} and {\itshape
  template parameters}.

This document will explain the major features of the document
class. For further information, the {\itshape \LaTeX\ User's Guide} is
available from
\url{https://www.acm.org/publications/proceedings-template}.

\subsection{Template Styles}

The primary parameter given to the ``\verb|acmart|'' document class is
the {\itshape template style} which corresponds to the kind of publication
or SIG publishing the work. This parameter is enclosed in square
brackets and is a part of the {\verb|documentclass|} command:
\begin{verbatim}
  \documentclass[STYLE]{acmart}
\end{verbatim}

Journals use one of three template styles. All but three ACM journals
use the {\verb|acmsmall|} template style:
\begin{itemize}
\item {\verb|acmsmall|}: The default journal template style.
\item {\verb|acmlarge|}: Used by JOCCH and TAP.
\item {\verb|acmtog|}: Used by TOG.
\end{itemize}

The majority of conference proceedings documentation will use the {\verb|acmconf|} template style.
\begin{itemize}
\item {\verb|acmconf|}: The default proceedings template style.
\item{\verb|sigchi|}: Used for SIGCHI conference articles.
\item{\verb|sigchi-a|}: Used for SIGCHI ``Extended Abstract'' articles.
\item{\verb|sigplan|}: Used for SIGPLAN conference articles.
\end{itemize}

\subsection{Template Parameters}

In addition to specifying the {\itshape template style} to be used in
formatting your work, there are a number of {\itshape template parameters}
which modify some part of the applied template style. A complete list
of these parameters can be found in the {\itshape \LaTeX\ User's Guide.}

Frequently-used parameters, or combinations of parameters, include:
\begin{itemize}
\item {\verb|anonymous,review|}: Suitable for a ``dual-anonymous''
  conference submission. Anonymizes the work and includes line
  numbers. Use with the \verb|\acmSubmissionID| command to print the
  submission's unique ID on each page of the work.
\item{\verb|authorversion|}: Produces a version of the work suitable
  for posting by the author.
\item{\verb|screen|}: Produces colored hyperlinks.
\end{itemize}

This document uses the following string as the first command in the
source file:
\begin{verbatim}
\documentclass[sigconf]{acmart}
\end{verbatim}

\section{Modifications}

Modifying the template --- including but not limited to: adjusting
margins, typeface sizes, line spacing, paragraph and list definitions,
and the use of the \verb|\vspace| command to manually adjust the
vertical spacing between elements of your work --- is not allowed.

{\bfseries Your document will be returned to you for revision if
  modifications are discovered.}

\section{Typefaces}

The ``\verb|acmart|'' document class requires the use of the
``Libertine'' typeface family. Your \TeX\ installation should include
this set of packages. Please do not substitute other typefaces. The
``\verb|lmodern|'' and ``\verb|ltimes|'' packages should not be used,
as they will override the built-in typeface families.

\section{Title Information}

The title of your work should use capital letters appropriately -
\url{https://capitalizemytitle.com/} has useful rules for
capitalization. Use the {\verb|title|} command to define the title of
your work. If your work has a subtitle, define it with the
{\verb|subtitle|} command.  Do not insert line breaks in your title.

If your title is lengthy, you must define a short version to be used
in the page headers, to prevent overlapping text. The \verb|title|
command has a ``short title'' parameter:
\begin{verbatim}
  \title[short title]{full title}
\end{verbatim}

\section{Authors and Affiliations}

Each author must be defined separately for accurate metadata
identification. Multiple authors may share one affiliation. Authors'
names should not be abbreviated; use full first names wherever
possible. Include authors' e-mail addresses whenever possible.

Grouping authors' names or e-mail addresses, or providing an ``e-mail
alias,'' as shown below, is not acceptable:
\begin{verbatim}
  \author{Brooke Aster, David Mehldau}
  \email{dave,judy,steve@university.edu}
  \email{firstname.lastname@phillips.org}
\end{verbatim}

The \verb|authornote| and \verb|authornotemark| commands allow a note
to apply to multiple authors --- for example, if the first two authors
of an article contributed equally to the work.

If your author list is lengthy, you must define a shortened version of
the list of authors to be used in the page headers, to prevent
overlapping text. The following command should be placed just after
the last \verb|\author{}| definition:
\begin{verbatim}
  \renewcommand{\shortauthors}{McCartney, et al.}
\end{verbatim}
Omitting this command will force the use of a concatenated list of all
of the authors' names, which may result in overlapping text in the
page headers.

The article template's documentation, available at
\url{https://www.acm.org/publications/proceedings-template}, has a
complete explanation of these commands and tips for their effective
use.

Note that authors' addresses are mandatory for journal articles.

\section{Rights Information}

Authors of any work published by ACM will need to complete a rights
form. Depending on the kind of work, and the rights management choice
made by the author, this may be copyright transfer, permission,
license, or an OA (open access) agreement.

Regardless of the rights management choice, the author will receive a
copy of the completed rights form once it has been submitted. This
form contains \LaTeX\ commands that must be copied into the source
document. When the document source is compiled, these commands and
their parameters add formatted text to several areas of the final
document:
\begin{itemize}
\item the ``ACM Reference Format'' text on the first page.
\item the ``rights management'' text on the first page.
\item the conference information in the page header(s).
\end{itemize}

Rights information is unique to the work; if you are preparing several
works for an event, make sure to use the correct set of commands with
each of the works.

The ACM Reference Format text is required for all articles over one
page in length, and is optional for one-page articles (abstracts).

\section{CCS Concepts and User-Defined Keywords}

Two elements of the ``acmart'' document class provide powerful
taxonomic tools for you to help readers find your work in an online
search.

The ACM Computing Classification System ---
\url{https://www.acm.org/publications/class-2012} --- is a set of
classifiers and concepts that describe the computing
discipline. Authors can select entries from this classification
system, via \url{https://dl.acm.org/ccs/ccs.cfm}, and generate the
commands to be included in the \LaTeX\ source.

User-defined keywords are a comma-separated list of words and phrases
of the authors' choosing, providing a more flexible way of describing
the research being presented.

CCS concepts and user-defined keywords are required for for all
articles over two pages in length, and are optional for one- and
two-page articles (or abstracts).

\section{Sectioning Commands}

Your work should use standard \LaTeX\ sectioning commands:
\verb|section|, \verb|subsection|, \verb|subsubsection|, and
\verb|paragraph|. They should be numbered; do not remove the numbering
from the commands.

Simulating a sectioning command by setting the first word or words of
a paragraph in boldface or italicized text is {\bfseries not allowed.}

\section{Tables}

The ``\verb|acmart|'' document class includes the ``\verb|booktabs|''
package --- \url{https://ctan.org/pkg/booktabs} --- for preparing
high-quality tables.

Table captions are placed {\itshape above} the table.

Because tables cannot be split across pages, the best placement for
them is typically the top of the page nearest their initial cite.  To
ensure this proper ``floating'' placement of tables, use the
environment \textbf{table} to enclose the table's contents and the
table caption.  The contents of the table itself must go in the
\textbf{tabular} environment, to be aligned properly in rows and
columns, with the desired horizontal and vertical rules.  Again,
detailed instructions on \textbf{tabular} material are found in the
\textit{\LaTeX\ User's Guide}.

Immediately following this sentence is the point at which
Table~\ref{tab:freq} is included in the input file; compare the
placement of the table here with the table in the printed output of
this document.

\begin{table}
  \caption{Frequency of Special Characters}
  \label{tab:freq}
  \begin{tabular}{ccl}
    \toprule
    Non-English or Math&Frequency&Comments\\
    \midrule
    \O & 1 in 1,000& For Swedish names\\
    $\pi$ & 1 in 5& Common in math\\
    \$ & 4 in 5 & Used in business\\
    $\Psi^2_1$ & 1 in 40,000& Unexplained usage\\
  \bottomrule
\end{tabular}
\end{table}

To set a wider table, which takes up the whole width of the page's
live area, use the environment \textbf{table*} to enclose the table's
contents and the table caption.  As with a single-column table, this
wide table will ``float'' to a location deemed more
desirable. Immediately following this sentence is the point at which
Table~\ref{tab:commands} is included in the input file; again, it is
instructive to compare the placement of the table here with the table
in the printed output of this document.

\begin{table*}
  \caption{Some Typical Commands}
  \label{tab:commands}
  \begin{tabular}{ccl}
    \toprule
    Command &A Number & Comments\\
    \midrule
    \texttt{{\char'134}author} & 100& Author \\
    \texttt{{\char'134}table}& 300 & For tables\\
    \texttt{{\char'134}table*}& 400& For wider tables\\
    \bottomrule
  \end{tabular}
\end{table*}

Always use midrule to separate table header rows from data rows, and
use it only for this purpose. This enables assistive technologies to
recognise table headers and support their users in navigating tables
more easily.

\section{Math Equations}
You may want to display math equations in three distinct styles:
inline, numbered or non-numbered display.  Each of the three are
discussed in the next sections.

\subsection{Inline (In-text) Equations}
A formula that appears in the running text is called an inline or
in-text formula.  It is produced by the \textbf{math} environment,
which can be invoked with the usual
\texttt{{\char'134}begin\,\ldots{\char'134}end} construction or with
the short form \texttt{\$\,\ldots\$}. You can use any of the symbols
and structures, from $\alpha$ to $\omega$, available in
\LaTeX~\cite{Lamport:LaTeX}; this section will simply show a few
examples of in-text equations in context. Notice how this equation:
\begin{math}
  \lim_{n\rightarrow \infty}x=0
\end{math},
set here in in-line math style, looks slightly different when
set in display style.  (See next section).

\subsection{Display Equations}
A numbered display equation---one set off by vertical space from the
text and centered horizontally---is produced by the \textbf{equation}
environment. An unnumbered display equation is produced by the
\textbf{displaymath} environment.

Again, in either environment, you can use any of the symbols and
structures available in \LaTeX\@; this section will just give a couple
of examples of display equations in context.  First, consider the
equation, shown as an inline equation above:
\begin{equation}
  \lim_{n\rightarrow \infty}x=0
\end{equation}
Notice how it is formatted somewhat differently in
the \textbf{displaymath}
environment.  Now, we'll enter an unnumbered equation:
\begin{displaymath}
  \sum_{i=0}^{\infty} x + 1
\end{displaymath}
and follow it with another numbered equation:
\begin{equation}
  \sum_{i=0}^{\infty}x_i=\int_{0}^{\pi+2} f
\end{equation}
just to demonstrate \LaTeX's able handling of numbering.

\section{Figures}

The ``\verb|figure|'' environment should be used for figures. One or
more images can be placed within a figure. If your figure contains
third-party material, you must clearly identify it as such, as shown
in the example below.
\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{sample-franklin}
  \caption{1907 Franklin Model D roadster. Photograph by Harris \&
    Ewing, Inc. [Public domain], via Wikimedia
    Commons. (\url{https://goo.gl/VLCRBB}).}
  \Description{A woman and a girl in white dresses sit in an open car.}
\end{figure}

Your figures should contain a caption which describes the figure to
the reader.

Figure captions are placed {\itshape below} the figure.

Every figure should also have a figure description unless it is purely
decorative. These descriptions convey what’s in the image to someone
who cannot see it. They are also used by search engine crawlers for
indexing images, and when images cannot be loaded.

A figure description must be unformatted plain text less than 2000
characters long (including spaces).  {\bfseries Figure descriptions
  should not repeat the figure caption – their purpose is to capture
  important information that is not already provided in the caption or
  the main text of the paper.} For figures that convey important and
complex new information, a short text description may not be
adequate. More complex alternative descriptions can be placed in an
appendix and referenced in a short figure description. For example,
provide a data table capturing the information in a bar chart, or a
structured list representing a graph.  For additional information
regarding how best to write figure descriptions and why doing this is
so important, please see
\url{https://www.acm.org/publications/taps/describing-figures/}.

\subsection{The ``Teaser Figure''}

A ``teaser figure'' is an image, or set of images in one figure, that
are placed after all author and affiliation information, and before
the body of the article, spanning the page. If you wish to have such a
figure in your article, place the command immediately before the
\verb|\maketitle| command:
\begin{verbatim}
  \begin{teaserfigure}
    \includegraphics[width=\textwidth]{sampleteaser}
    \caption{figure caption}
    \Description{figure description}
  \end{teaserfigure}
\end{verbatim}

\section{Citations and Bibliographies}

The use of \BibTeX\ for the preparation and formatting of one's
references is strongly recommended. Authors' names should be complete
--- use full first names (``Donald E. Knuth'') not initials
(``D. E. Knuth'') --- and the salient identifying features of a
reference should be included: title, year, volume, number, pages,
article DOI, etc.

The bibliography is included in your source document with these two
commands, placed just before the \verb|\end{document}| command:
\begin{verbatim}
  \bibliographystyle{ACM-Reference-Format}
  \bibliography{bibfile}
\end{verbatim}
where ``\verb|bibfile|'' is the name, without the ``\verb|.bib|''
suffix, of the \BibTeX\ file.

Citations and references are numbered by default. A small number of
ACM publications have citations and references formatted in the
``author year'' style; for these exceptions, please include this
command in the {\bfseries preamble} (before the command
``\verb|\begin{document}|'') of your \LaTeX\ source:
\begin{verbatim}
  \citestyle{acmauthoryear}
\end{verbatim}

  Some examples.  A paginated journal article \cite{Abril07}, an
  enumerated journal article \cite{Cohen07}, a reference to an entire
  issue \cite{JCohen96}, a monograph (whole book) \cite{Kosiur01}, a
  monograph/whole book in a series (see 2a in spec. document)
  \cite{Harel79}, a divisible-book such as an anthology or compilation
  \cite{Editor00} followed by the same example, however we only output
  the series if the volume number is given \cite{Editor00a} (so
  Editor00a's series should NOT be present since it has no vol. no.),
  a chapter in a divisible book \cite{Spector90}, a chapter in a
  divisible book in a series \cite{Douglass98}, a multi-volume work as
  book \cite{Knuth97}, a couple of articles in a proceedings (of a
  conference, symposium, workshop for example) (paginated proceedings
  article) \cite{Andler79, Hagerup1993}, a proceedings article with
  all possible elements \cite{Smith10}, an example of an enumerated
  proceedings article \cite{VanGundy07}, an informally published work
  \cite{Harel78}, a couple of preprints \cite{Bornmann2019,
    AnzarootPBM14}, a doctoral dissertation \cite{Clarkson85}, a
  master's thesis: \cite{anisi03}, an online document / world wide web
  resource \cite{Thornburg01, Ablamowicz07, Poker06}, a video game
  (Case 1) \cite{Obama08} and (Case 2) \cite{Novak03} and \cite{Lee05}
  and (Case 3) a patent \cite{JoeScientist001}, work accepted for
  publication \cite{rous08}, 'YYYYb'-test for prolific author
  \cite{SaeediMEJ10} and \cite{SaeediJETC10}. Other cites might
  contain 'duplicate' DOI and URLs (some SIAM articles)
  \cite{Kirschmer:2010:AEI:1958016.1958018}. Boris / Barbara Beeton:
  multi-volume works as books \cite{MR781536} and \cite{MR781537}. A
  couple of citations with DOIs:
  \cite{2004:ITE:1009386.1010128,Kirschmer:2010:AEI:1958016.1958018}. Online
  citations: \cite{TUGInstmem, Thornburg01, CTANacmart}. Artifacts:
  \cite{R} and \cite{UMassCitations}.

\section{Acknowledgments}

Identification of funding sources and other support, and thanks to
individuals and groups that assisted in the research and the
preparation of the work should be included in an acknowledgment
section, which is placed just before the reference section in your
document.

This section has a special environment:
\begin{verbatim}
  \begin{acks}
  ...
  \end{acks}
\end{verbatim}
so that the information contained therein can be more easily collected
during the article metadata extraction phase, and to ensure
consistency in the spelling of the section heading.

Authors should not prepare this section as a numbered or unnumbered {\verb|\section|}; please use the ``{\verb|acks|}'' environment.

\section{Appendices}

If your work needs an appendix, add it before the
``\verb|\end{document}|'' command at the conclusion of your source
document.

Start the appendix with the ``\verb|appendix|'' command:
\begin{verbatim}
  \appendix
\end{verbatim}
and note that in the appendix, sections are lettered, not
numbered. This document has two appendices, demonstrating the section
and subsection identification method.

\section{Multi-language papers}

Papers may be written in languages other than English or include
titles, subtitles, keywords and abstracts in different languages (as a
rule, a paper in a language other than English should include an
English title and an English abstract).  Use \verb|language=...| for
every language used in the paper.  The last language indicated is the
main language of the paper.  For example, a French paper with
additional titles and abstracts in English and German may start with
the following command
\begin{verbatim}
\documentclass[sigconf, language=english, language=german,
               language=french]{acmart}
\end{verbatim}

The title, subtitle, keywords and abstract will be typeset in the main
language of the paper.  The commands \verb|\translatedXXX|, \verb|XXX|
begin title, subtitle and keywords, can be used to set these elements
in the other languages.  The environment \verb|translatedabstract| is
used to set the translation of the abstract.  These commands and
environment have a mandatory first argument: the language of the
second argument.  See \verb|sample-sigconf-i13n.tex| file for examples
of their usage.

\section{SIGCHI Extended Abstracts}

The ``\verb|sigchi-a|'' template style (available only in \LaTeX\ and
not in Word) produces a landscape-orientation formatted article, with
a wide left margin. Three environments are available for use with the
``\verb|sigchi-a|'' template style, and produce formatted output in
the margin:
\begin{itemize}
\item {\verb|sidebar|}:  Place formatted text in the margin.
\item {\verb|marginfigure|}: Place a figure in the margin.
\item {\verb|margintable|}: Place a table in the margin.
\end{itemize}

==> References.tex <==
@article{Zou_2020_Wearable,
title = {Wearable triboelectric nanogenerators for biomechanical energy harvesting},
journal = {Nano Energy},
volume = {77},
pages = {105303},
year = {2020},
issn = {2211-2855},
doi = {https://doi.org/10.1016/j.nanoen.2020.105303},
url = {https://www.sciencedirect.com/science/article/pii/S2211285520308806},
author = {Yongjiu Zou and Vidhur Raveendran and Jun Chen},
keywords = {Triboelectric nanogenerators, Electricity generation, Wearable bioelectronics, Internet of things},
abstract = {With compelling features of flexibility, conformability, and user friendliness, wearable bioelectronics have undergone tremendous development on account of miniaturization and multifunction advancements which could cater to the development trend of Internet of Things (IoT) and fifth-generation wireless technology. However, powering wearable bioelectronics sustainably and pervasively is beyond the capability of traditional power supply systems and remains a challenge and highly desired. By using the coupling effect of contact electrification and electrostatic induction, triboelectric nanogenerators (TENGs) were demonstrated to efficiently convert irregular and low-frequency biomechanical energy from human body movements into electrical energy for the sustainable powering of wearable bioelectronics. In this article, the latest representative achievements of wearable TENGs for electricity generation are comprehensively reviewed with the order of the accessible biomechanical energy on the human body from head to feet. This review not only covers the fundamental working mechanism, rational structural design, selection of the tribo-materials, and fabrication process of wearable TENGs, but also investigates the movement patterns and characteristics of each part of the body, as well as its feasibility and convenience for electricity generation. Finally, perspectives and challenges regarding wearable TENGs at present are discussed.}
}

@article{SmartFabric_Castano_2014,
doi = {10.1088/0964-1726/23/5/053001},
url = {https://dx.doi.org/10.1088/0964-1726/23/5/053001},
year = {2014},
month = {apr},
publisher = {IOP Publishing},
volume = {23},
number = {5},
pages = {053001},
author = {Castano, Lina M and Flatau, Alison B},
title = {Smart fabric sensors and e-textile technologies: a review},
journal = {Smart Materials and Structures},
abstract = {This paper provides a review of recent developments in the rapidly changing and advancing field of smart fabric sensor and electronic textile technologies. It summarizes the basic principles and approaches employed when building fabric sensors as well as the most commonly used materials and techniques used in electronic textiles. This paper shows that sensing functionality can be created by intrinsic and extrinsic modifications to textile substrates depending on the level of integration into the fabric platform. The current work demonstrates that fabric sensors can be tailored to measure force, pressure, chemicals, humidity and temperature variations. Materials, connectors, fabric circuits, interconnects, encapsulation and fabrication methods associated with fabric technologies prove to be customizable and versatile but less robust than their conventional electronics counterparts. The findings of this survey suggest that a complete smart fabric system is possible through the integration of the different types of textile based functional elements. This work intends to be a starting point for standardization of smart fabric sensing techniques and e-textile fabrication methods.}
}




@article{he2024flexible,
  title={Flexible Supercapacitor Integrated Systems},
  author={He, Aiqi and He, Jiangfeng and Cao, Lingyun and Chen, Jiaxiang and Cheng, Bin and Ma, Rui and Ding, Yi and Yang, Guowei and Yi, Fang},
  journal={Advanced Materials Technologies},
  pages={2301931},
  year={2024},
  publisher={Wiley Online Library}
}

@article{acssuschemeng,
author = {Prajesh, Neetu and Sharma, Vijay Bhan and Rajput, Shatruhan Singh and Singh, Chandan Kumar and Dixit, Prashant and Praveenkumar, Balu and Zarȩba, Jan K. and Kabra, Dinesh and Ogale, Satishchandra and Boomishankar, Ramamoorthy},
title = {Flexible Piezoelectric Nanogenerators Based on One-Dimensional Neutral Coordination Network Composites},
journal = {ACS Sustainable Chemistry \& Engineering},
volume = {10},
number = {30},
pages = {9911-9920},
year = {2022},
doi = {10.1021/acssuschemeng.2c02296},
URL = {https://doi.org/10.1021/acssuschemeng.2c02296},
eprint = {https://doi.org/10.1021/acssuschemeng.2c0229}
}


@inproceedings{WuLoomPedalsTEI,
author = {Wu, Shanel and Corr, Xavier A and Gao, Xi and De Koninck, Sasha and Bowers, Robin and Devendorf, Laura},
title = {Loom Pedals: Retooling Jacquard Weaving for Improvisational Design Workflows},
year = {2024},
isbn = {9798400704024},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3623509.3633358},
doi = {10.1145/3623509.3633358},
abstract = {We present the Loom Pedals, an open-source hardware/software interface for enhancing a weaver’s ability to create on-the-fly, improvised designs in Jacquard weaving. Learning from traditional handweaving and our own weaving experiences, we describe our process of designing, implementing, and using the prototype Loom Pedals system with a TC2 Digital Jacquard loom. The Loom Pedals include a set of modular, reconfigurable foot pedals which can be mapped to parametric Operations that generate and transform digital woven designs. Our novel interface integrates design and loom control, providing a customizable workflow for playful, improvisational Jacquard weaving. We conducted a formative evaluation of the prototype through autobiographical methods and collaboratively developed future Loom Pedals features. We contribute our prototype, design process, and conceptual reflections on weaving as a human-machine dialog between a weaver, the loom, and many other agents.},
booktitle = {Proceedings of the Eighteenth International Conference on Tangible, Embedded, and Embodied Interaction},
articleno = {10},
numpages = {16},
keywords = {Jacquard weaving, craft, design interfaces, interactive fabrication},
location = {Cork, Ireland},
series = {TEI '24}
}

@article{kim2024mediknit,
author = {Kim, Heather Jin Hee and Pourjafarian, Narjes and Choudhury, Arhan and Stilling, Joan and Kao, Cindy Hsin-Liu},
title = {MediKnit: Soft Medical Making for Personalized and Clinician-Designed Wearable Devices for Hand Edema},
year = {2024},
issue_date = {September 2024},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {8},
number = {3},
url = {https://doi.org/10.1145/3678504},
doi = {10.1145/3678504},
abstract = {Current rapid prototyping in medical domains relies on rigid 3D-printed materials, lacking flexibility, customization, and clinician-led input. This paper introduces MediKnit, a novel approach for the fabrication of soft medical devices, addressing critical limitations in existing design processes for medical devices. MediKnit provides a design tool empowering clinicians to personalize fabric-based devices for hand edema. This tool allows clinicians to adapt the design to individual patients' demands, thereby enhancing the overall effectiveness of therapy. The MediKnit device created by this tool consists of a machine-knit glove with active compression, which is programmable through a custom PCB. This device facilitates the mobilization of edema. To illustrate the practical implementation of our approach, this paper presents case studies involving six patients experiencing hand edema. The results demonstrate the adaptability and feasibility of our process for developing soft medical devices, highlighting its potential to broaden accessibility, facilitate personalized solutions, and empower clinicians as active medical makers.},
journal = {Proc. ACM Interact. Mob. Wearable Ubiquitous Technol.},
month = sep,
articleno = {110},
numpages = {30},
keywords = {Case study, Compression device, Design tool, Fabrication, Hand edema, Medical making, Robotic textiles, Textile-based device, User study, Workflows}
}

@inproceedings{Jiang2024embrogami,
author = {Jiang, Yu and Haynes, Alice C and Pourjafarian, Narjes and Borchers, Jan and Steimle, J\"{u}rgen},
title = {Embrogami: Shape-Changing Textiles with Machine Embroidery},
year = {2024},
isbn = {9798400706288},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3654777.3676431},
doi = {10.1145/3654777.3676431},
abstract = {Machine embroidery is a versatile technique for creating custom and entirely fabric-based patterns on thin and conformable textile surfaces. However, existing machine-embroidered surfaces remain static, limiting the interactions they can support. We introduce Embrogami, an approach for fabricating textile structures with versatile shape-changing behaviors. Inspired by origami, we leverage machine embroidery to form finger-tip-scale mountain-and-valley structures on textiles with customized shapes, bistable or elastic behaviors, and modular composition. The structures can be actuated by the user or the system to modify the local textile surface topology, creating interactive elements like toggles and sliders or textile shape displays with an ultra-thin, flexible, and integrated form factor. We provide a dedicated software tool and report results of technical experiments to allow users to flexibly design, fabricate, and deploy customized Embrogami structures. With four application cases, we showcase Embrogami’s potential to create functional and flexible shape-changing textiles with diverse visuo-tactile feedback.},
booktitle = {Proceedings of the 37th Annual ACM Symposium on User Interface Software and Technology},
articleno = {63},
numpages = {15},
keywords = {Fabrication, e-textiles., machine embroidery, shape-change},
location = {Pittsburgh, PA, USA},
series = {UIST '24}
}

@inproceedings{leeEDarningTEI,
author = {Jones, Lee},
title = {The E-darning Sampler: Exploring E-textile Repair with Darning Looms},
year = {2021},
isbn = {9781450382137},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3430524.3444700},
doi = {10.1145/3430524.3444700},
abstract = {Extending the life of our clothes is the most effective intervention of all current sustainable textile practices. Taking this into consideration, this paper explores how we can upcycle and repair our clothes with e-textiles, and how to share these techniques with other makers and crafters. To do so the author interviewed 4 visible mending educators about their teaching practices and personal experiences with mending. These interviews were then used to inform the design of the E-Darning Sampler for the TEI 2021 swatchbook, which includes examples of different e-textile darning patterns and functionalities made with darning looms. This paper contributes insights on how to design educational samples for encouraging sustainable making practices.},
booktitle = {Proceedings of the Fifteenth International Conference on Tangible, Embedded, and Embodied Interaction},
articleno = {82},
numpages = {5},
keywords = {crafting, e-textiles, education, sustainability},
location = {Salzburg, Austria},
series = {TEI '21}
}

@inproceedings{kuznetsov2018ScreenprintTEI,
author = {Kuznetsov, Stacey and Fernando, Piyum and Ritter, Emily and Barrett, Cassandra and Weiler, Jennifer and Rohr, Marissa},
title = {Screenprinting and TEI: Supporting Engagement with STEAM through DIY Fabrication of Smart Materials},
year = {2018},
isbn = {9781450355681},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3173225.3173253},
doi = {10.1145/3173225.3173253},
abstract = {This paper focuses on manual screenprinting as a DIY fabrication technique for embedding interactive behavior onto a rage of substrates such as paper, fabric, plastic, wood, or vinyl. We frame screenprinting as a process that operates at the intersection of art, technology, and material science and iteratively examine its potential in two STEAM contexts. We conducted youth and adult workshops whereby participants worked with our low-cost thermochromic, UV-sensitive, and conductive screenprinting inks to develop a range of concepts and final projects. Our findings highlight several unique features of screenprinting: it affords a low barrier to entry for smart material fabrication, supports a collaborative maker practice, and scaffolds creative engagement with STEAM concepts. By being widely-accessible and substrate-agnostic, screenprinting presents exciting opportunities for TEI: DIY fabrication of smart materials in domains such as fine arts, information visualization, and slow technology; and bridging diverse disciplines through STEAM screenprinting initiatives at youth and adult levels.},
booktitle = {Proceedings of the Twelfth International Conference on Tangible, Embedded, and Embodied Interaction},
pages = {211–220},
numpages = {10},
keywords = {diy fabrication, screenprinting, smart materials, steam},
location = {Stockholm, Sweden},
series = {TEI '18}
}
@inproceedings{gemperle1998designforwearability,
  title={Design for wearability},
  author={Gemperle, Francine and Kasabach, Chris and Stivoric, John and Bauer, Malcolm and Martin, Richard},
  booktitle={digest of papers. Second international symposium on wearable computers (cat. No. 98EX215)},
  pages={116--122},
  year={1998},
  organization={IEEE}
}

@inproceedings{disalvo2010sustinablehci,
  title={Mapping the landscape of sustainable HCI},
  author={DiSalvo, Carl and Sengers, Phoebe and Brynjarsd{\'o}ttir, Hr{\"o}nn},
  booktitle={Proceedings of the SIGCHI conference on human factors in computing systems},
  pages={1975--1984},
  year={2010}
}


@INPROCEEDINGS{wicaksono3Dknits2022,
  author={Wicaksono, Irmandy and Hwang, Peter G. and Droubi, Samir and Wu, Franny Xi and Serio, Allison N. and Yan, Wei and Paradiso, Joseph A.},
  booktitle={2022 44th Annual International Conference of the IEEE Engineering in Medicine \& Biology Society (EMBC)}, 
  title={3DKnITS: Three-dimensional Digital Knitting of Intelligent Textile Sensor for Activity Recognition and Biomechanical Monitoring}, 
  year={2022},
  volume={},
  number={},
  pages={2403-2409},
  keywords={Fabrication;Wireless communication;Wireless sensor networks;Three-dimensional displays;Wearable computers;Thermoforming;Sensors},
  doi={10.1109/EMBC48229.2022.9871651}}

@inproceedings{Shi-WooDowel,
author = {Shi, Yonghao and Su, Yuning and Wu, Te-Yen and Li, Chenzheng and Yang, Xing-Dong},
title = {WooDowel: Electrode Isolation for Electromagnetic Shielding in Triboelectric Plywood Sensors},
year = {2024},
isbn = {9781450368162},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
booktitle = {Proceedings of the 2021 CHI Conference on Human Factors in Computing Systems-to be appeared},
location = {Honolulu, USA},
series = {CHI '24}
}

@article{KwakStretchable2017,
author = {Kwak, Sung Soo and Kim, Han and Seung, Wanchul and Kim, Jihye and Hinchet, Ronan and Kim, Sang-Woo},
title = {Fully Stretchable Textile Triboelectric Nanogenerator with Knitted Fabric Structures},
journal = {ACS Nano},
volume = {11},
number = {11},
pages = {10733-10741},
year = {2017},
doi = {10.1021/acsnano.7b05203},
    note ={PMID: 28968064},
URL = { 
        https://doi.org/10.1021/acsnano.7b05203
},
eprint = { 
    
        https://doi.org/10.1021/acsnano.7b05203
}
}


@article{Greinke-Folded,
    author = {Greinke, Berit and Wood, Emma and Skach, Sophie and Vilas, Arantza and Vierne, Pauline},
    title = "{Folded Electronic Textiles: Weaving, Knitting, Pleating and Coating Three-Dimensional Sensor Structures}",
    journal = {Leonardo},
    volume = {55},
    number = {3},
    pages = {235-239},
    year = {2022},
    month = {05},
    abstract = "{This article reports findings from a one-month design research project in which four textile and fashion designers engaged in collaborative exploration of technical and artistic knowledge inherent in folds and folding. They experimented with textile technologies and construction methods to design, fabricate and analyze three-dimensional dynamic materiality in electronic textiles (e-textiles). The focus was on sensor structures achieved by knitting, weaving, pleating and coating techniques. The analysis of measurements of electrical resistance between one and 36 sensing areas per sample demonstrate the added value of folds integrated into textile sensor structures. The authors discuss types of folding and their aesthetic, textural and sensorial advantages. Detailed information on design, fabrication and experimental results is provided in supplemental materials to the article.}",
    issn = {0024-094X},
    doi = {10.1162/leon_a_02183},
    url = {https://doi.org/10.1162/leon\_a\_02183},
    eprint = {https://direct.mit.edu/leon/article-pdf/55/3/235/2025230/leon\_a\_02183.pdf},
}


@inproceedings{albaugh2021engineering,
  title={Engineering Multifunctional Spacer Fabrics Through Machine Knitting},
  author={Albaugh, Lea and McCann, James and Hudson, Scott E and Yao, Lining},
  booktitle={Proceedings of the 2021 CHI Conference on Human Factors in Computing Systems},
  pages={1--12},
  year={2021}
}

@inproceedings{Hofmann-KnitPicking,
author = {Hofmann, Megan and Albaugh, Lea and Sethapakadi, Ticha and Hodgins, Jessica and Hudson, Scott E. and McCann, James and Mankoff, Jennifer},
title = {KnitPicking Textures: Programming and Modifying Complex Knitted Textures for Machine and Hand Knitting},
year = {2019},
isbn = {9781450368162},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3332165.3347886},
doi = {10.1145/3332165.3347886},
abstract = {Knitting creates complex, soft fabrics with unique texture properties that can be used to create interactive objects.However, little work addresses the challenges of designing and using knitted textures computationally. We present KnitPick: a pipeline for interpreting hand-knitting texture patterns into KnitGraphs which can be output to machine and hand-knitting instructions. Using KnitPick, we contribute a measured and photographed data set of 472 knitted textures. Based on findings from this data set, we contribute two algorithms for manipulating KnitGraphs. KnitCarving shapes a graph while respecting a texture, and KnitPatching combines graphs with disparate textures while maintaining a consistent shape. KnitPick is the first system to bridge the gap between hand- and machine-knitting when creating complex knitted textures.},
booktitle = {Proceedings of the 32nd Annual ACM Symposium on User Interface Software and Technology},
pages = {5–16},
numpages = {12},
keywords = {compiler, fabrication, knitspeak, knitting, machine knitting, soft fabrication},
location = {New Orleans, LA, USA},
series = {UIST '19}
}

@article{wu2020automatic,
  title={Automatic structure synthesis for 3D woven relief.},
  author={Wu, Rundong and Harvey, Claire and Zhang, Joy Xiaoji and Kroszner, Sean and Hagan, Brooks and Marschner, Steve},
  journal={ACM Trans. Graph.},
  volume={39},
  number={4},
  pages={102},
  year={2020}
}

@inproceedings{Devendorf-adacad,
author = {Devendorf, Laura and Walters, Kathryn and Fairbanks, Marianne and Sandry, Etta and Goodwill, Emma R},
title = {AdaCAD: Parametric Design as a New Form of Notation for Complex Weaving},
year = {2023},
isbn = {9781450394215},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3544548.3581571},
doi = {10.1145/3544548.3581571},
abstract = {Woven textiles are increasingly a medium through which HCI is inventing new technologies. Key challenges in integrating woven textiles in HCI include the high level of textile knowledge required to make effective use of the new possibilities they afford and the need for tools that bridge the concerns of textile designers and concerns of HCI researchers. This paper presents AdaCAD, a parametric design tool for designing woven textile structures. Through our design and evaluation of AdaCAD we found that parametric design helps weavers notate and explain the logics behind the complex structures they generate. We discuss these finding in relation to prior work in integrating craft and/or weaving in HCI, histories of woven notation, and boundary object theory to illuminate further possibilities for collaboration between craftspeople and HCI practitioners.},
booktitle = {Proceedings of the 2023 CHI Conference on Human Factors in Computing Systems},
articleno = {127},
numpages = {18},
keywords = {computer-aided design, first-person methods, open-source, parametric design, smart textiles, textile fabrication, weaving},
location = {Hamburg, Germany},
series = {CHI '23}
}

@inproceedings{Pin-Sung-PATCH-o,
author = {Ku, Pin-Sung and Huang, Kunpeng and Kao, Cindy Hsin-Liu},
title = {Patch-O: Deformable Woven Patches for On-body Actuation},
year = {2022},
isbn = {9781450391573},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3491102.3517633},
doi = {10.1145/3491102.3517633},
abstract = {We present Patch-O, a novel deformable interface devised as a woven patch that enables diverse movement-based interactions adaptive to garments or on-skin wearing. Patch-O interfaces are uniquely detachable and relocatable soft actuation units that can be sewn or attached to clothing or skin at various locations. To optimize the morphing effect while preserving a slim form factor, we introduce a construction approach that integrates actuators at a structural level and varies the texture and stiffness of the woven substrate locally. We implement three basic actuation primitives, including bending, expanding, and shrinking, and experiment with aggregation parameters to exhaustively extend the design space. A final workshop study inviting textile practitioners to create personalized designs of Patch-O provides insights into the expressiveness of the approach for wearable interactions. We conclude with three applications inspired by users’ designs and showcase the aesthetic and functional usages enabled by the deformable woven patches.},
booktitle = {Proceedings of the 2022 CHI Conference on Human Factors in Computing Systems},
articleno = {615},
numpages = {12},
keywords = {Wearable Computers, Fashion/Clothing, Fabrication},
location = {New Orleans, LA, USA},
series = {CHI '22}
}

@article{xia2019universal,
  title={A universal standardized method for output capability assessment of nanogenerators},
  author={Xia, Xin and Fu, Jingjing and Zi, Yunlong},
  journal={Nature communications},
  volume={10},
  number={1},
  pages={4428},
  year={2019},
  publisher={Nature Publishing Group UK London}
}



@article{Yu-acrylic,
author = {Yu, Aifang and Zhu, Yaxing and Wang, Wei and Zhai, Junyi},
title = {Progress in Triboelectric Materials: Toward High Performance and Widespread Applications},
journal = {Advanced Functional Materials},
volume = {29},
number = {41},
pages = {1900098},
keywords = {micro/nanostructures, molecular surface functionalization, multifunctional triboelectric materials, triboelectric charge density, triboelectric nanogenerator},
doi = {https://doi.org/10.1002/adfm.201900098},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/adfm.201900098},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/adfm.201900098},
abstract = {Abstract Triboelectric phenomena can be observed everywhere; however, they are consistently omitted from applications. Although almost all substances exhibit a triboelectrification effect in daily life, chemists as well as materials scientists have performed extensive investigations in both the aspects of basic science and practical applications to promote the development of triboelectric nanogenerators (TENGs). Here, a detailed survey of materials engineering for high triboelectric performance and multifunctional materials toward specific applications is summarized, including constructing micro/nanostructures, chemically modifying the frication surface, modulating bulk friction materials, the mechanism for improved performance, and preparing materials for implantable medical devices, bionic skin, and wearable electronic devices. Moreover, an in depth discussion of the current challenges and future efforts for strengthening the performance of TENGs is elaborated in detail, which will better guide new researchers toward a deeper understanding of and explorations about TENGs.},
year = {2019}
}


@article{pyo2020all,
  title={All-textile wearable triboelectric nanogenerator using pile-embroidered fibers for enhancing output power},
  author={Pyo, Soonjae and Kim, Min-Ook and Kwon, Dae-Sung and Kim, Wondo and Yang, Jin-Hee and Cho, Hyun Seung and Lee, Joo Hyeon and Kim, Jongbaeg},
  journal={Smart Materials and Structures},
  volume={29},
  number={5},
  pages={055026},
  year={2020},
  publisher={IOP Publishing}
}

@article{Zhang-screenPrinting,
author = {Zhang, Chi and Zhang, Lei and Bao, Bo and Ouyang, Wenyu and Chen, Weiyu and Li, Qingtong and Li, Dachao},
title = {Customizing Triboelectric Nanogenerator on Everyday Clothes by Screen-Printing Technology for Biomechanical Energy Harvesting and Human-Interactive Applications},
journal = {Advanced Materials Technologies},
volume = {8},
number = {4},
pages = {2201138},
keywords = {energy harvesting, HMIs, screen-printing, TENG, textile},
doi = {https://doi.org/10.1002/admt.202201138},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/admt.202201138},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/admt.202201138},
abstract = {Abstract Integrating self-powered sensors or energy harvesters with everyday clothes brings a novel insight into wearable electronics and improves personal intelligence in the era of the Internet of Things. This work develops a customizable screen-printed textile triboelectric nanogenerator (SPT-TENG) for biomechanical energy harvesting and human-interactive applications. The as-fabricated textile TENG not only presents excellent wearing experiences such as lightweight, permeability, and washability, but also exhibits high electrical output performance to power sustainably some portable electronics such as a watch or calculator. The system-level wearable human-interactive applications, including a wireless keyboard and a smart home appliance control, are also demonstrated with the advantages of cyber security, easy operation, low cost, and wearability through screen-printing pattern-customized TENG arrays. Benefiting from these features, the SPT-TENG shows promising applications in wearable electronics, human-machine interfaces, and artificial intelligence.},
year = {2023}
}


@article{cheng2017stretchable,
  title={A stretchable fiber nanogenerator for versatile mechanical energy harvesting and self-powered full-range personal healthcare monitoring},
  author={Cheng, Yin and Lu, Xin and Chan, Kwok Hoe and Wang, Ranran and Cao, Zherui and Sun, Jing and Ho, Ghim Wei},
  journal={Nano Energy},
  volume={41},
  pages={511--518},
  year={2017},
  publisher={Elsevier}
}

@article{MAO2021105918,
title = {Triboelectric nanogenerator/supercapacitor in-one self-powered textile based on PTFE yarn wrapped PDMS/MnO2NW hybrid elastomer},
journal = {Nano Energy},
volume = {84},
pages = {105918},
year = {2021},
issn = {2211-2855},
doi = {https://doi.org/10.1016/j.nanoen.2021.105918},
url = {https://www.sciencedirect.com/science/article/pii/S2211285521001762},
author = {Yongyun Mao and Yong Li and Jiyang Xie and Huan Liu and Changjin Guo and Wanbiao Hu},
keywords = {Supercapacitor, Nanogenerators, Energy harvesting, Pressure sensing, MnO nanowire},
abstract = {Triboelectric nanogenerator/supercapacitor (TENG-SC) is believed to have great potential for wearable/portable bio-motion energy harvesting/storage electronics, but many TENGs could rarely be satisfactory to wearable electronics because of their poor wearability and complex configurations. Herein, a round-tripping-knitting strategy is devised to directly knit flexible PTFE yarn closing around polydimethylsiloxane/MnO2 nanowire (PDMS/MnO2NW)-coated conductive carbon cloth yarns (CCT@PDMS/MnO2NW) that can be used as wearable TENG textile to harvest bio-motion energy. Superior power generation performance was obtained by modulating the dielectric permittivity of PDMS/MnO2NW elastomer based on variations in the mass-loading of MnO2NW. The obtained TENG textile can convert various forms of bio-motion energy into electrical signal and the maximum output voltage of about 380 V can be obtained and easily light up 200 serially connected LEDs. Additionally, all-solid-state yarn-type asymmetric supercapacitor was woven with TENG and act as energy storage unit, which demonstrates high volumetric energy density and excellent cyclic stability. Because of the flexible all yarn-type structure of the entire system, the SC and TENG can be easily woven into cloth to continuously harvest and store bio-motion energy, which demonstrates great convenience and immense applications as wearable, lightweight, comfortable continuous bio-motion energy harvesting/storage device and versatile pressure sensing.}
}

@online{ottoman-stitch,
    author = "Wikipedia",
    title = "Ottoman (textile)",
    url  = "https://en.wikipedia.org/wiki/Ottoman_(textile)",
    addendum = "(accessed: 03.01.2024)",
    keywords = "ottoman"
}


@article{PAOSANGTHONG2022106739,
title = {Textile-based triboelectric nanogenerator with alternating positive and negative freestanding woven structure for harvesting sliding energy in all directions},
journal = {Nano Energy},
volume = {92},
pages = {106739},
year = {2022},
issn = {2211-2855},
doi = {https://doi.org/10.1016/j.nanoen.2021.106739},
url = {https://www.sciencedirect.com/science/article/pii/S2211285521009885},
author = {Watcharapong Paosangthong and Mahmoud Wagih and Russel Torah and Steve Beeby},
keywords = {Triboelectric nanogenerator, E-textile, Woven structure, All directions harvester},
abstract = {A novel textile-based triboelectric nanogenerator (TENG) with woven structure operating in freestanding triboelectric-layer mode, defined as a woven-TENG, has been developed. Whereas most woven-structured TENGs operate in contact-separation mode and consist of one type of triboelectric material, this woven-TENG comprises woven electrodes and woven strips of positive and negative triboelectric material, which form a checker-like pattern over the electrodes with matching periodicity. The implementation of the positive and negative triboelectric material significantly improves the performance of the woven-TENG. Furthermore, in contrast to the conventional grating-structured and woven-structured TENG, which are designed to operate only in one moving direction, this new design also allows the woven-TENG to harvest energy from all-planar directions of movement. The woven-TENG with woven strips of nylon and polytetrafluoroethylenevinyl (PTFE) fabric can generate a root mean square (RMS) open-circuit voltage of 62.9 V, an RMS short-circuit current of 1.77 µA and a maximum RMS power of 34.8 µW at a load resistance of 50 MΩ, a mechanical oscillation of 2 Hz and a contact force of 5 N. This corresponds to a maximum RMS power density of 5.43 mW/m2.}
}

@article{bairagi2022high,
  title={High-performance triboelectric nanogenerators based on commercial textiles: electrospun nylon 66 nanofibers on silk and PVDF on polyester},
  author={Bairagi, Satyaranjan and Khandelwal, Gaurav and Karagiorgis, Xenofon and Gokhool, Shravan and Kumar, Charchit and Min, Guanbo and Mulvihill, Daniel M},
  journal={ACS Applied Materials \& Interfaces},
  volume={14},
  number={39},
  pages={44591--44603},
  year={2022},
  publisher={ACS Publications}
}

@Article{nanoenergyadv1010004,
AUTHOR = {Ibrahim, Mervat and Jiang, Jinxing and Wen, Zhen and Sun, Xuhui},
TITLE = {Surface Engineering for Enhanced Triboelectric Nanogenerator},
JOURNAL = {Nanoenergy Advances},
VOLUME = {1},
YEAR = {2021},
NUMBER = {1},
PAGES = {58--80},
URL = {https://www.mdpi.com/2673-706X/1/1/4},
ISSN = {2673-706X},
ABSTRACT = {Triboelectric nanogenerator (TENG) is the new technique that can convert low-frequency mechanical energy into effective electricity. As an energy collector, the pursuit of high output characteristics is understandable. Although high charge density has been achieved by working in high vacuum or charge pumping techniques, it remains challenging to obtain the high output performance directly in the atmosphere. Herein, surface-engineering of the triboelectric layer for enhancing output performance has been reviewed carefully. By constructing surface morphology or developing surface modification, high performance of TENGs is finally presented in the review.},
DOI = {10.3390/nanoenergyadv1010004}
}

@article{Davison:2010:techniques,
  title={Techniques for robust touch sensing design},
  author={Davison, Burke},
  journal={AN1334 Microchip Technology Inc},
  pages={53},
  year={2010}
}

@article{ZouOptimizeTENGs,
  title={Advances in nanostructures for high-performance triboelectric nanogenerators},
  author={Zou, Yongjiu and Xu, Jing and Chen, Kyle and Chen, Jun},
  journal={Advanced Materials Technologies},
  volume={6},
  number={3},
  pages={2000916},
  year={2021},
  publisher={Wiley Online Library}
}

@article{NamForceTouchMeasurement,
author = {Choonsung Nam and DongRyeol Shin},
title ={Force-touch measurement methodology based on user experience},
journal = {International Journal of Distributed Sensor Networks},
volume = {14},
number = {4},
pages = {1550147718767794},
year = {2018},
doi = {10.1177/1550147718767794},
URL = {https://doi.org/10.1177/1550147718767794},
eprint = {https://doi.org/10.1177/1550147718767794},
abstract = { The touch interface is an input method widely used in smart devices. Recently, new touch interface which supports force value has been introduced. The force-touch interface adds a factor called depth to the plane coordinates as compared to the existing touch interface. Despite the advantages of force-touch, which can provide touch position and force intensity information with one input, there are still many devices that cannot support force values. To provide them with a force-touch interface, we developed a force-touch cover for existing smart devices that do not support the existing force value. It is a way to provide the force value to the smart device by recognizing the force value through the sensor installed in smartphone case. However, it is difficult to apply the force value obtained through such a device directly to the force-touch interface, because it is necessary to distinguish between force touch and general touch. Therefore, in order to use the force-touch interface using the force-touch cover proposed in this article, the force value measured at the time of general touch is analyzed by user experiment to set the general touch area. Also, an area outside the general touch area is set as the force-touch area. In the force-touch and general touch area, the area is applied considering the error of the force value actually measured in the developed force-touch cover. Therefore, in this article, we analyze the force value input through the proposed force-touch cover and find a reference value that can distinguish force touch from general touch by user experiment and propose a method to apply it. }
}

@article{TriboelectricSeriesPUPTFE,
title = {Sustainable powering triboelectric nanogenerators: Approaches and the path towards efficient use},
journal = {Nano Energy},
volume = {51},
pages = {270-285},
year = {2018},
issn = {2211-2855},
doi = {https://doi.org/10.1016/j.nanoen.2018.06.075},
url = {https://www.sciencedirect.com/science/article/pii/S2211285518304701},
author = {Hong-Joon Yoon and Hanjun Ryu and Sang-Woo Kim},
keywords = {Triboelectric nanogenerators, Sustainable, Fluoropolymers, Powering devices, Efficiency},
abstract = {Triboelectric nanogenerators (TENGs), which have demonstrated that all moving things in the universe can generate electricity in a sustainable way are currently being developed to be integrated with electronics, and to improve user convenience. The electrically charged surface upon a contact electrification phenomenon caused by contact of the materials determines the output performance of TENGs. This review focuses on the electrification and surface charge density characteristics of various fluoropolymer-based materials as active materials that have been investigated to realize high performance TENGs, and the results of the study of their applications. Furthermore, the characteristics of electrification with differently polymerized P(VDF-TrFE) as TENGs’ active materials and their applications are reviewed. The boosted output performance characteristics when used as a matrix material and integrated with a composite system with a high dielectric constant material are also reviewed. Finally, the paper presents three perspectives on the direction of TENG research for future improvement, namely material, structure, and circuitry.}
}


@book{tao2001smartfibres,
  title={Smart Fibres, Fabrics and Clothing: Fundamentals and Applications},
  author={Tao, X.},
  isbn={9781855737600},
  series={Woodhead Publishing Series in Textiles},
  url={https://books.google.com/books?id=plWkAgAAQBAJ},
  year={2001},
  publisher={Elsevier Science}
}

@article{LuPowerManagementCircuit,
title = {Regulating the high-voltage and high-impedance characteristics of triboelectric nanogenerator toward practical self-powered sensors},
journal = {Nano Energy},
volume = {87},
pages = {106137},
year = {2021},
issn = {2211-2855},
doi = {https://doi.org/10.1016/j.nanoen.2021.106137},
url = {https://www.sciencedirect.com/science/article/pii/S2211285521003931},
author = {Shan Lu and Wenqian Lei and Lingxiao Gao and Xin Chen and Daqiao Tong and Pengfei Yuan and Xiaojing Mu and Hua Yu}
}

@article{HarmonPowerManagementSystem,
title = {Self-driven power management system for triboelectric nanogenerators},
journal = {Nano Energy},
volume = {71},
pages = {104642},
year = {2020},
issn = {2211-2855},
doi = {https://doi.org/10.1016/j.nanoen.2020.104642},
url = {https://www.sciencedirect.com/science/article/pii/S2211285520301993},
author = {William Harmon and David Bamgboje and Hengyu Guo and Tingshu Hu and Zhong Lin Wang},
}

@article{ZARGARI2021114489,
title = {A new Mylar-based triboelectric energy harvester with an innovative design for mechanical energy harvesting applications},
journal = {Energy Conversion and Management},
volume = {244},
pages = {114489},
year = {2021},
issn = {0196-8904},
doi = {https://doi.org/10.1016/j.enconman.2021.114489},
url = {https://www.sciencedirect.com/science/article/pii/S0196890421006658},
author = {Siavash Zargari and Ziaddin {Daie Koozehkanani} and Hadi Veladi and Jafar Sobhi and Alireza Rezania},
keywords = {Energy harvesting, Triboelectric nanogenerator, Triboelectric energy harvester, Origami TENG, Mylar-based TENG, Power management circuit},
abstract = {In this paper, an innovative origami structure is deployed to create a novel, flexible, lightweight, and low-cost triboelectric nanogenerator (Miura-Ori-TENG). For the first time, Mylar film is used as a supporting and flexible spring-like structure to develop the first Mylar-based origami TENG, eliminating the need for any external auxiliary system to ensure continuous operation of the TENG. Subsequently, a self-powered power management circuit with a novel self-controlled switching mechanism is designed and implemented for direct use of Miura-Ori-TENG electrical output and maximizing the harvested energy. The performance of the Miura-Ori-TENG and power management circuit are evaluated under different practical conditions. The open-circuit voltage and short-circuit current reached 308.6 V and 55.5 µA, respectively, with a peak power of 5.1 mW under a linear reciprocating motion with an operating frequency of 4 Hz. Moreover, open-circuit voltage, short-circuit current, and instant output power of 1050 V, 131 µA, and 40 mW are obtained using footsteps during human walking. Furthermore, in a 1000 µF capacitor charging experiment using the proposed power management circuit, the stored energy increased up to 117.5 times compared to a direct charging experiment. In order to prove that the Miura-Ori-TENG, in combination with the proposed power management circuit, could be used as a power source in many applications, its ability to charge the capacitors and rechargeable batteries and drive the electronics is shown with proof-of-concept demonstrations. The results of this study demonstrated potential applications of the Miura-Ori-TENG in converting rotational, vibrational, and impact kinetic energies into electrical energy, as well as the outstanding performance of the proposed power management circuit in managing the harvested energy.}
}



@article{zou2019quantifying,
  title={Quantifying the triboelectric series},
  author={Zou, Haiyang and Zhang, Ying and Guo, Litong and Wang, Peihong and He, Xu and Dai, Guozhang and Zheng, Haiwu and Chen, Chaoyu and Wang, Aurelia Chi and Xu, Cheng and others},
  journal={Nature communications},
  volume={10},
  number={1},
  pages={1427},
  year={2019},
  publisher={Nature Publishing Group UK London}
}

@article{LIU2018383,
title = {Triboelectric charge density of porous and deformable fabrics made from polymer fibers},
journal = {Nano Energy},
volume = {53},
pages = {383-390},
year = {2018},
issn = {2211-2855},
doi = {https://doi.org/10.1016/j.nanoen.2018.08.071},
url = {https://www.sciencedirect.com/science/article/pii/S2211285518306335},
author = {Shirui Liu and Wei Zheng and Bao Yang and Xiaoming Tao},
keywords = {Triboelectrification, Triboelectric series, Charge density, Porous materials, Contact area},
abstract = {Triboelectricity has attracted much attention for its potential applications in harvesting mechanical energy by triboelectric nanogenerators, whose output performance is dominated by triboelectric charge density. The number of electric charges generated on interactive surfaces is an intrinsic property of the materials directly related to their chemical structure and high-order structures. This paper deals with a sliding-mode triboelectrification system and measurement methods of the charge density on highly porous and deformable materials like textile fabrics with a structural hierarchy. Effects of operational parameters of the system, structures and properties of fabrics made from twenty one types of polymer fibers were investigated. It is found that the effective charge density of fabrics can be reliably measured when the tribo-electrification process reaches its saturation under the fabric densification pressure. An extended table of measured tribo-electric charge density is compiled with highly porous and deformable knitted fabrics made from twenty one types of polymer fibers.}
}

@ARTICLE{TextileBiomedicalWearables,
  author={Park, Sungmee and Jayaraman, Sundaresan},
  journal={IEEE Transactions on Information Technology in Biomedicine}, 
  title={Smart Textile-Based Wearable Biomedical Systems: A Transition Plan for Research to Reality}, 
  year={2010},
  volume={14},
  number={1},
  pages={86-92},
  keywords={Biomedical monitoring;Textile technology;Business;Projectiles;Remote monitoring;Polymers;Textile fibers;Medical services;Biomedical computing;Public policy;Healthcare monitoring;intelligent textiles;research commercialization;Smart Shirt;wearable biomedical systems;Wearable Motherboard},
  doi={10.1109/TITB.2009.2025817}}


@article{PentlandWearableIntelligence,
  title={Wearable intelligence},
  author={Pentland, Alex},
  journal={Scientific American},
  volume={276},
  number={11},
  year={1998}
}

@book{WangTENGHandbook,
  title = {Handbook of Triboelectric Nanogenerators},
  ISBN = {9783031057229},
  url = {http://dx.doi.org/10.1007/978-3-031-05722-9},
  DOI = {10.1007/978-3-031-05722-9},
  publisher = {Springer International Publishing},
  author = {Wang, Zhong Lin and Yang, Ya and Zhai, Junyi and Wang, Jie},
  year = {2023}
}

@inproceedings{IOBraid,
author = {Olwal, Alex and Moeller, Jon and Priest-Dorman, Greg and Starner, Thad and Carroll, Ben},
title = {I/O Braid: Scalable Touch-Sensitive Lighted Cords Using Spiraling, Repeating Sensing Textiles and Fiber Optics},
year = {2018},
isbn = {9781450359481},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3242587.3242638},
doi = {10.1145/3242587.3242638},
booktitle = {Proceedings of the 31st Annual ACM Symposium on User Interface Software and Technology},
pages = {485–497},
numpages = {13},
keywords = {wearables, ubiquitous computing, soft electronics, sensor, interactive textiles, input, capacitive sensing},
series = {UIST '18}
}

@inproceedings{DierkHairIO,
author = {Dierk, Christine and Sterman, Sarah and Nicholas, Molly Jane Pearce and Paulos, Eric},
title = {H\"{a}irI\"{O}: Human Hair as Interactive Material},
year = {2018},
isbn = {9781450355681},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3173225.3173232},
doi = {10.1145/3173225.3173232},
booktitle = {Proceedings of the Twelfth International Conference on Tangible, Embedded, and Embodied Interaction},
pages = {148–157},
numpages = {10},
keywords = {wearables, hair, cosmetic computing, ambient displays},
location = {Stockholm, Sweden},
series = {TEI '18}
}

@article{DongFiberFabricTENG,
author = {Dong, Kai and Peng, Xiao and Wang, Zhong Lin},
title = {Fiber/Fabric-Based Piezoelectric and Triboelectric Nanogenerators for Flexible/Stretchable and Wearable Electronics and Artificial Intelligence},
journal = {Advanced Materials},
volume = {32},
number = {5},
pages = {1902549},
keywords = {fiber/fabric-based, piezoelectric nanogenerators, smart textiles, triboelectric nanogenerators, wearable electronics},
doi = {https://doi.org/10.1002/adma.201902549},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/adma.201902549},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/adma.201902549},
abstract = {Abstract Integration of advanced nanogenerator technology with conventional textile processes fosters the emergence of textile-based nanogenerators (NGs), which will inevitably promote the rapid development and widespread applications of next-generation wearable electronics and multifaceted artificial intelligence systems. NGs endow smart textiles with mechanical energy harvesting and multifunctional self-powered sensing capabilities, while textiles provide a versatile flexible design carrier and extensive wearable application platform for their development. However, due to the lack of an effective interactive platform and communication channel between researchers specializing in NGs and those good at textiles, it is rather difficult to achieve fiber/fabric-based NGs with both excellent electrical output properties and outstanding textile-related performances. To this end, a critical review is presented on the current state of the arts of wearable fiber/fabric-based piezoelectric nanogenerators and triboelectric nanogenerators with respect to basic classifications, material selections, fabrication techniques, structural designs, and working principles, as well as potential applications. Furthermore, the potential difficulties and tough challenges that can impede their large-scale commercial applications are summarized and discussed. It is hoped that this review will not only deepen the ties between smart textiles and wearable NGs, but also push forward further research and applications of future wearable fiber/fabric-based NGs.},
year = {2020}
}


@inbook{Zhang-StructuresOfTENG-2019,
author = {Zhang, Haixia},
publisher = {John Wiley \& Sons, Ltd},
isbn = {9783527820153},
title = {Structures of Triboelectric Nanogenerators},
booktitle = {Flexible and Stretchable Triboelectric Nanogenerator Devices},
chapter = {2},
pages = {19-40},
doi = {https://doi.org/10.1002/9783527820153.ch2},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/9783527820153.ch2},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/9783527820153.ch2},
year = {2019},
keywords = {arch-shaped TENGs, contact-separation mode, freestanding mode, plane-shaped TENGs, relative-sliding mode, rotor-shaped TENGs, single-electrode mode, triboelectric nanogenerators, wavy-shaped TENGs, zig-zag-shaped TENGs},
abstract = {Summary Triboelectric nanogenerators (TENGs) can be applied in various environments. There are four modes of TENGs to harvest the energy based on operation mechanisms, i.e. contact-separation (CS), relative-sliding (RS), single-electrode (SE), and freestanding (FS). This chapter introduces the several major operation modes and several typical structures of TENGs. After analyzing CS, RS, SE, and FS modes of TENGs, one can find that both vertical and horizontal directional contact can achieve power generation based on suitable operation mechanisms. The chapter lists and analyzes the typical TENG structures, such as plane-shaped, arch-shaped, zig-zag-shaped, wavy-shaped, and rotor-shaped, besides introducing successful applications. Plane-shaped TENG is the most common structure. It can be divided into two groups: 2D and 3D. The Z. L. Wang group demonstrated a simple 3D plane-shaped TENG, in which two different friction layers are separated by a spacer. This structure is suitable for vertical operations based on the CS mode.}
}

@article{Wang-Triboelectric-13,
author = {Wang, Zhong Lin},
title = {Triboelectric Nanogenerators as New Energy Technology for Self-Powered Systems and as Active Mechanical and Chemical Sensors},
journal = {ACS Nano},
volume = {7},
number = {11},
pages = {9533-9557},
year = {2013},
doi = {10.1021/nn404614z},
note ={PMID: 24079963},
URL = {https://doi.org/10.1021/nn404614z},
eprint = {https://doi.org/10.1021/nn404614z}
}

@article{WaldenTextileTENG,
title = {Textile-Triboelectric nanogenerators (T-TENGs) for wearable energy harvesting devices},
journal = {Chemical Engineering Journal},
volume = {451},
pages = {138741},
year = {2023},
issn = {1385-8947},
doi = {https://doi.org/10.1016/j.cej.2022.138741},
url = {https://www.sciencedirect.com/science/article/pii/S138589472204222X},
author = {Ryan Walden and Irthasa Aazem and Aswathy Babu and Suresh C. Pillai},
keywords = {Textile triboelectric, Wearable, Self-powered sensors},
}


@article{TianTextileBasedTENGs,
author = {Tian, Xiao and Dong, Shanshan and Yang, Mengyan and Ng, Hoiyan and Liu, Yanping and Hu, Hong and Hua, Tao},
title = {Textile-Based Triboelectric Nanogenerators for Smart Wearable Systems: Comfort, Integration, and Application},
journal = {Advanced Materials Technologies},
volume = {8},
number = {8},
pages = {2201294},
keywords = {applications, comfort, integrations, textile-based triboelectric nanogenerators},
doi = {https://doi.org/10.1002/admt.202201294},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/admt.202201294},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/admt.202201294},
year = {2023}
}

@article{HeMultiFunctionalTENGs,
title = {Beyond energy harvesting - multi-functional triboelectric nanosensors on a textile},
journal = {Nano Energy},
volume = {57},
pages = {338-352},
year = {2019},
issn = {2211-2855},
doi = {https://doi.org/10.1016/j.nanoen.2018.12.032},
url = {https://www.sciencedirect.com/science/article/pii/S221128551830939X},
author = {Tianyiyi He and Qiongfeng Shi and Hao Wang and Feng Wen and Tao Chen and Jianyong Ouyang and Chengkuo Lee},
keywords = {Triboelectric, Self-powered, Textile, PEDOT:PSS, Sensor},
}

@article{HurdoganogluReviewOfTENGs,
    author = {Hurdoganoglu, Dogus and Safaei, Babak and Cheng, Jia and Qin, Zhaoye and Sahmani, Saeid},
    title = "{A Comprehensive Review on the Novel Principles, Development and Applications of Triboelectric Nanogenerators}",
    journal = {Applied Mechanics Reviews},
    volume = {76},
    number = {1},
    pages = {010802},
    year = {2023},
    month = {07},
    doi = {10.1115/1.4056391},
    url = {https://doi.org/10.1115/1.4056391},
    eprint = {https://asmedigitalcollection.asme.org/appliedmechanicsreviews/article-pdf/76/1/010802/7032232/amr\_076\_01\_010802.pdf},
}

@article{VeraAnayaNearFieldTENGs,
title = {Self-powered eye motion sensor based on triboelectric interaction and near-field electrostatic induction for wearable assistive technologies},
journal = {Nano Energy},
volume = {72},
pages = {104675},
year = {2020},
issn = {2211-2855},
doi = {https://doi.org/10.1016/j.nanoen.2020.104675},
url = {https://www.sciencedirect.com/science/article/pii/S2211285520302329},
author = {David {Vera Anaya} and Tianyiyi He and Chengkuo Lee and Mehmet R. Yuce},
keywords = {Triboelectric sensor, Eye motion, Wearable HMI, Disabled-people aid, Hands-free computer control},
}

@article{SHI2017479,
title = {Self-powered wireless smart patch for healthcare monitoring},
journal = {Nano Energy},
volume = {32},
pages = {479-487},
year = {2017},
issn = {2211-2855},
doi = {https://doi.org/10.1016/j.nanoen.2017.01.008},
url = {https://www.sciencedirect.com/science/article/pii/S2211285517300071},
author = {Mayue Shi and Hanxiang Wu and Jinxin Zhang and Mengdi Han and Bo Meng and Haixia Zhang},
keywords = {Smart patch, Self-powered, Wireless, Wearable electronics, Physiological monitoring},
abstract = {Wearable electronics provides an opportunity for everyone to own personal healthcare systems. Convenience, versatility and energy conservation are vital elements to extend the functions of wearable electronics. Here we present a self-powered smart patch with wireless transmission ability based on triboelectric effect and electrostatic induction to monitor the temperature and motion status of individuals. Spontaneous friction charges are utilized to make the system self-powered. The energy and signal are wirelessly transmitted to the receiver through electrostatic induction. The wireless transmission efficiency achieved 26.6% with a 16cm2 receiver while the distance is 1cm, which shows remarkable capability of near-field wireless transmission. With different load resistances from 1Ω to 1MΩ, the output current of the receiver keeps constant like a current source. Using a method that transmits energy and signal at the same time, our smart patch can not only collect energy to drive the commercial sensors, but also work as an active sensor monitoring the motion status of people. To realize the wearable electrode, a fabric-based conductor with high stability is developed. A transparent and stretchable silver nanowire (Ag NW) based electrode is fabricated to ensure the compatibility between the receiver and various surfaces such as smartphones.}
}

@article{DongKnittedTENGs,
title = {Seamlessly knitted stretchable comfortable textile triboelectric nanogenerators for E-textile power sources},
journal = {Nano Energy},
volume = {78},
pages = {105327},
year = {2020},
issn = {2211-2855},
doi = {https://doi.org/10.1016/j.nanoen.2020.105327},
url = {https://www.sciencedirect.com/science/article/pii/S2211285520309046},
author = {Shanshan Dong and Fan Xu and Yilan Sheng and Zihao Guo and Xiong Pu and Yanping Liu},
keywords = {Triboelectric nanogeneroators, Electronic textiles, Stretchable, Wearable electronics, Intarsia technique},
}

@article{ChengTENGPrimer,
  title = {Triboelectric nanogenerators},
  volume = {3},
  ISSN = {2662-8449},
  url = {http://dx.doi.org/10.1038/s43586-023-00220-3},
  pages={39},
  DOI = {10.1038/s43586-023-00220-3},
  number = {1},
  journal = {Nature Reviews Methods Primers},
  publisher = {Springer Science and Business Media LLC},
  author = {Cheng,  Tinghai and Shao,  Jiajia and Wang,  Zhong Lin},
  year = {2023},
  month = may 
}

@article{AlamIntroToTENG,
  title = {An introduction to triboelectric nanogenerators},
  volume = {34},
  ISSN = {2352-507X},
  url = {http://dx.doi.org/10.1016/j.nanoso.2023.100980},
  DOI = {10.1016/j.nanoso.2023.100980},
  journal = {Nano-Structures \& Nano-Objects},
  publisher = {Elsevier BV},
  author = {Alam,  Syed Nasimul and Ghosh,  Arka and Shrivastava,  Pankaj and Shukla,  Uddeshya and Garg,  Kamal and Edara,  Abhay Chowdary and Sahoo,  Nityananada},
  year = {2023},
  month = apr,
  pages = {100980}
}

@article{NingFiberTENGRespiratoryMonitoring,
  title = {Helical Fiber Strain Sensors Based on Triboelectric Nanogenerators for Self-Powered Human Respiratory Monitoring},
  volume = {16},
  ISSN = {1936-086X},
  url = {http://dx.doi.org/10.1021/acsnano.1c09792},
  DOI = {10.1021/acsnano.1c09792},
  number = {2},
  journal = {ACS Nano},
  publisher = {American Chemical Society (ACS)},
  author = {Ning,  Chuan and Cheng,  Renwei and Jiang,  Yang and Sheng,  Feifan and Yi,  Jia and Shen,  Shen and Zhang,  Yihan and Peng,  Xiao and Dong,  Kai and Wang,  Zhong Lin},
  year = {2022},
  month = jan,
  pages = {2811–2821}
}

@article{LinTextileTENGSleepTracking,
  title = {Large‐Scale and Washable Smart Textiles Based on Triboelectric Nanogenerator Arrays for Self‐Powered Sleeping Monitoring},
  volume = {28},
  ISSN = {1616-3028},
  pages = {1704112},
  url = {http://dx.doi.org/10.1002/adfm.201704112},
  DOI = {10.1002/adfm.201704112},
  number = {1},
  journal = {Advanced Functional Materials},
  publisher = {Wiley},
  author = {Lin,  Zhiming and Yang,  Jun and Li,  Xiaoshi and Wu,  Yufen and Wei,  Wei and Liu,  Jun and Chen,  Jun and Yang,  Jin},
  year = {2017},
  month = nov 
}

@article{RepouliasTriboelectricityTextile,
  title = {Triboelectricity and textile structures},
  volume = {112},
  ISSN = {1754-2340},
  url = {http://dx.doi.org/10.1080/00405000.2020.1829331},
  DOI = {10.1080/00405000.2020.1829331},
  number = {10},
  journal = {The Journal of The Textile Institute},
  publisher = {Informa UK Limited},
  author = {Repoulias,  Aristeidis and Vassiliadis,  Savvas and Galata,  Sotiria F.},
  year = {2020},
  month = oct,
  pages = {1580–1587}
}

@Article{NingWashable2018,
author ="Ning, Chuan and Tian, Lan and Zhao, Xinya and Xiang, Shengxin and Tang, Yingjie and Liang, Erjun and Mao, Yanchao",
title  ="Washable textile-structured single-electrode triboelectric nanogenerator for self-powered wearable electronics",
journal  ="J. Mater. Chem. A",
year  ="2018",
volume  ="6",
issue  ="39",
pages  ="19143-19150",
publisher  ="The Royal Society of Chemistry",
doi  ="10.1039/C8TA07784C",
url  ="http://dx.doi.org/10.1039/C8TA07784C",
abstract  ="Wearable electronics guide the next generation of traditional personal electronics. However{,} their conventional batteries are required to be frequently charged or replaced{,} greatly limiting the development of wearable electronics. Thus{,} a wearable power source that can in situ harvest biomechanical energy to continuously power wearable electronics is extremely desirable. In this work{,} we report for the first time a washable textile-structured single-electrode triboelectric nanogenerator (TS-TENG) based on a nanofibrous polytetrafluoroethylene (PTFE) polymer with high hydrophobicity. A stained TS-TENG can be easily and quickly cleaned by washing in water. The TS-TENG can be sewed on clothes{,} and then it can effectively convert mechanical energy to electricity by the friction with the material of clothes. When operated by swinging arms while people are walking or running{,} the output voltage and current of the TS-TENG obtained were 1050 V and 22 μA{,} respectively. This generated electric energy could directly power a night running light and a digital watch without any energy storage process. The development of this TS-TENG could provide great opportunities for developing self-powered wearable electronics due to its flexibility{,} breathability{,} washability{,} and capability to harvest biomechanical energy from human motions."}

@article{FengWeaving2020,
title = {Scalable, washable and lightweight triboelectric-energy-generating fibers by the thermal drawing process for industrial loom weaving},
journal = {Nano Energy},
volume = {74},
pages = {104805},
year = {2020},
issn = {2211-2855},
doi = {https://doi.org/10.1016/j.nanoen.2020.104805},
url = {https://www.sciencedirect.com/science/article/pii/S2211285520303621},
author = {Ziang Feng and Shuo Yang and Sixian Jia and Yujing Zhang and Shan Jiang and Li Yu and Rui Li and Guowen Song and Anbo Wang and Thomas Martin and Lei Zuo and Xiaoting Jia},
keywords = {Scalable fiber, Triboelectric nanogenerator, Thermal drawing, Loom weaving},
abstract = {In the era of the internet of things (IoTs), it is desired to equip the decentralized electronics with distributed power sources. The fiber-based triboelectric nanogenerator (FTENG) provides one of the soundest solutions due to its high efficiency, easy deployment, excellent wearability, low cost, and eco-friendliness. Compared with other forms of TENGs, it can be woven into fabrics as wearable devices, offering good compactness and comfortability. However, the industrial-loom-compatible FTENGs have yet to be fabricated; the fiber diameter and length are typical challenges in the large scale weaving. In this paper, the thermal drawing process (TDP) is introduced to produce FTENGs that are compatible with industrial looms. The diameter of the polymer-cladding and metal-core fiber has been reduced to ~350μm, and the length of a single fiber has been scaled up to sub-kilometer. Both hand-woven and loom-woven swatches are demonstrated, showing good flexibility, stretchability, power density, stability, washability, and breathability. Besides serving as power sources, such swatches have been used as self-powered sensors for body motion monitoring and communication. These applications show that the thermally drawn FTENGs can serve as powerful and reliable wearable devices in modern electronics.}
}

@Article{ChenFiberYarn2022,
AUTHOR = {Chen, Yu and Ling, Yali and Yin, Rong},
TITLE = {Fiber/Yarn-Based Triboelectric Nanogenerators (TENGs): Fabrication Strategy, Structure, and Application},
JOURNAL = {Sensors},
VOLUME = {22},
YEAR = {2022},
NUMBER = {24},
ARTICLE-NUMBER = {9716},
URL = {https://www.mdpi.com/1424-8220/22/24/9716},
PubMedID = {36560085},
ISSN = {1424-8220},
ABSTRACT = {With the demand of a sustainable, wearable, environmentally friendly energy source, triboelectric nanogenerators (TENGs) were developed. TENG is a promising method to convert mechanical energy from motion into electrical energy. The combination of textile and TENG successfully enables wearable, self-driving electronics and sensor systems. As the primary unit of textiles, fiber and yarn become the focus of research in designing of textile-TENGs. In this review, we introduced the preparation, structure, and design strategy of fiber/yarn TENGs in recent research. We discussed the structure design and material selection of fiber/yarn TENGs according to the different functions it realizes. The fabrication strategy of fiber/yarn TENGs into textile-TENG are provided. Finally, we summarize the main applications of existing textile TENGs and give forward prospects for their subsequent development.},
DOI = {10.3390/s22249716}
}

@article{PaosangthongTextileTENGs2019,
title = {Recent progress on textile-based triboelectric nanogenerators},
journal = {Nano Energy},
volume = {55},
pages = {401-423},
year = {2019},
issn = {2211-2855},
doi = {https://doi.org/10.1016/j.nanoen.2018.10.036},
url = {https://www.sciencedirect.com/science/article/pii/S2211285518307626},
author = {Watcharapong Paosangthong and Russel Torah and Steve Beeby},
keywords = {Triboelectric nanogenerator, Textile, Fabric, Fibre},
abstract = {Triboelectric nanogenerators (TENG) are one of the most promising candidates for powering wearable and portable devices. Example TENGs have demonstrated flexibility, light weight, biocompatibility, versatility and good performance. Textiles are a potential substrate onto, or into, which wearable technology is increasingly being incorporated but supplying power remains an enduring challenge. TENGs are a potential textile based mechanical energy harvesting power supply and there has been an increasing effort to combine TENGs with fabrics. A significant challenge exists in the integration without losing the performance of the TENG or the original properties (appearance, breathability, washability, and durability) and feel of the textile. Various approaches towards the realisation of textile-based TENGs (T-TENGs) have been demonstrated. Depending on its structure, T-TENGs can be divided into two main types, fabric-based TENG and fibre-based TENG. The fabric-based TENG is composed of conventional and/or modified fabrics, which serve as a substrate and/or a triboelectric material. The fibre-based TENG is fabricated as a single fibre or a collection of interlaced fibres. This paper provides an up to date review of the progress in the research of T-TENGs. The paper covers the basic operating principles, possible operation modes, textile manufacturing methods, material selections, T-TENG fabrication process, surface modification and structural designs. Issues, such as standardised measurement parameters, the challenges and limitations of T-TENG are discussed.}
}

@article{ChenWovenTENGGait,
  title = {Woven Fabric Triboelectric Nanogenerator for Biomotion Energy Harvesting and as Self-Powered Gait-Recognizing Socks},
  volume = {13},
  ISSN = {1996-1073},
  url = {http://dx.doi.org/10.3390/en13164119},
  DOI = {10.3390/en13164119},
  number = {16},
  journal = {Energies},
  publisher = {MDPI AG},
  author = {Chen,  Chaoyu and Zhang,  Lei and Ding,  Wenbo and Chen,  Lijun and Liu,  Jinkang and Du,  Zhaoqun and Yu,  Weidong},
  year = {2020},
  month = aug,
  pages = {4119}
}

@inproceedings{GowrishankarTENGTextilesWeaving,
  series = {UbiComp ’17},
  title = {Constructing triboelectric textiles with weaving},
  url = {http://dx.doi.org/10.1145/3123021.3123037},
  DOI = {10.1145/3123021.3123037},
  booktitle = {Proceedings of the 2017 ACM International Symposium on Wearable Computers},
  publisher = {ACM},
  author = {Gowrishankar,  Ramyah},
  year = {2017},
  month = sep,
  collection = {UbiComp ’17}
}

@article{CuiFlexibleSingleElectrodeTENG,
  title = {Flexible Single-Electrode Triboelectric Nanogenerator and Body Moving Sensor Based on Porous Na2CO3/Polydimethylsiloxane Film},
  volume = {10},
  ISSN = {1944-8252},
  url = {http://dx.doi.org/10.1021/acsami.7b17585},
  DOI = {10.1021/acsami.7b17585},
  number = {4},
  journal = {ACS Applied Materials \& Interfaces},
  publisher = {American Chemical Society (ACS)},
  author = {Cui,  Chunmei and Wang,  Xingzhao and Yi,  Zhiran and Yang,  Bin and Wang,  Xiaolin and Chen,  Xiang and Liu,  Jingquan and Yang,  Chunsheng},
  year = {2018},
  month = jan,
  pages = {3652–3659}
}
@inproceedings{Extail,
author = {Suyama, Yuiko and Baba, Tetsuaki},
title = {Extail: Wearable Hair Device that Enables Body Motion Exaggerations},
year = {2024},
isbn = {9798400704024},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3623509.3635259},
doi = {10.1145/3623509.3635259},
booktitle = {Proceedings of the Eighteenth International Conference on Tangible, Embedded, and Embodied Interaction},
articleno = {78},
numpages = {6},
keywords = {Augmented Body, Embodied Interaction, Hair, Organic User Interfaces, Tangible Interaction, Wearable},
series = {TEI '24}
}

@article{DogaFabricBasedWearableTENG,
title = {Fabric based wearable triboelectric nanogenerators for human machine interface},
journal = {Nano Energy},
volume = {89},
pages = {106412},
year = {2021},
issn = {2211-2855},
doi = {https://doi.org/10.1016/j.nanoen.2021.106412},
url = {https://www.sciencedirect.com/science/article/pii/S2211285521006674},
author = {Doga Doganay and Melih Ogeday Cicek and Mete Batuhan Durukan and Burak Altuntas and Erdem Agbahca and Sahin Coskun and Husnu Emrah Unalan},
}

@article{jahan2017effect,
  title={Effect of fabric structure on the mechanical properties of woven fabrics},
  author={Jahan, I},
  journal={Advance Research in Textile Engineering},
  volume={2},
  number={2},
  pages={1018},
  year={2017}
}

@article{somkuwar2020structurally,
  title={Structurally engineered textile-based triboelectric nanogenerator for energy harvesting application},
  author={Somkuwar, Viraj Uttamrao and Pragya, Akanksha and Kumar, Bipin},
  journal={Journal of materials science},
  volume={55},
  number={12},
  pages={5177--5189},
  year={2020},
  publisher={Springer}
}

@article{chen2016micro,
  title={Micro-cable structured textile for simultaneously harvesting solar and mechanical energy},
  author={Chen, Jun and Huang, Yi and Zhang, Nannan and Zou, Haiyang and Liu, Ruiyuan and Tao, Changyuan and Fan, Xing and Wang, Zhong Lin},
  journal={Nature Energy},
  volume={1},
  number={10},
  pages={1--8},
  year={2016},
  publisher={Nature Publishing Group}
}

@inproceedings{Woven-eTextiles-in-HCI_Pouta_DIS22,
author = {Pouta, Emmi and Mikkonen, Jussi Ville},
title = {Woven eTextiles in HCI — a Literature Review},
year = {2022},
isbn = {9781450393584},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3532106.3533566},
doi = {10.1145/3532106.3533566},
abstract = {Advances to functional materials and flexible electronics have yielded new means of integrating electrical properties into textile materials, which invite researchers in various fields to apply woven-textile construction methods in eTextile development. However, common ground for woven eTextiles’ prototyping is still taking shape. This calls for greater understanding of how the knowledge now scattered across diverse research fields can benefit the textiles’ development for HCI. To investigate how eTextile research has employed weaving and extract insight for HCI purposes, the authors reviewed and categorised applications of woven structures and electrical functions, then identified specifically HCI-relevant qualities and means of creating them via weaving. The paper outlines those woven structures useful for HCI and advocates consistent weaving-related terminology, to improve knowledge transfer across disciplines. In addition, the results point to research opportunities involving haptic qualities, the ability to weave multiple layers, functionality integration, and tools and methods.},
booktitle = {Proceedings of the 2022 ACM Designing Interactive Systems Conference},
pages = {1099–1118},
numpages = {20},
keywords = {weaving, smart textiles, eTextiles},
series = {DIS '22}
}


@inproceedings{FibeRobo_Forman_UIST23,
author = {Forman, Jack and Kilic Afsar, Ozgun and Nicita, Sarah and Lin, Rosalie Hsin-Ju and Yang, Liu and Hofmann, Megan and Kothakonda, Akshay and Gordon, Zachary and Honnet, Cedric and Dorsey, Kristen and Gershenfeld, Neil and Ishii, Hiroshi},
title = {FibeRobo: Fabricating 4D Fiber Interfaces by Continuous Drawing of Temperature Tunable Liquid Crystal Elastomers},
year = {2023},
isbn = {9798400701320},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3586183.3606732},
doi = {10.1145/3586183.3606732},
abstract = {We present FibeRobo, a thermally-actuated liquid crystal elastomer (LCE) fiber that can be embedded or structured into textiles and enable silent and responsive interactions with shape-changing, fiber-based interfaces. Three definitive properties distinguish FibeRobo from other actuating threads explored in HCI. First, they exhibit rapid thermal self-reversing actuation with large displacements (∼40\%) without twisting. Second, we present a reproducible UV fiber drawing setup that produces hundreds of meters of fiber with a sub-millimeter diameter. Third, FibeRobo is fully compatible with existing textile manufacturing machinery such as weaving looms, embroidery, and industrial knitting machines. This paper contributes to developing temperature-responsive LCE fibers, a facile and scalable fabrication pipeline with optional heating element integration for digital control, mechanical characterization, and the establishment of higher hierarchical textile structures and design space. Finally, we introduce a set of demonstrations that illustrate the design space FibeRobo enables.},
booktitle = {Proceedings of the 36th Annual ACM Symposium on User Interface Software and Technology},
articleno = {19},
numpages = {17},
keywords = {tangible, shape-changing interfaces, morphing textiles, maker culture, liquid crystal elastomer},
series = {UIST '23}
}

@article{Yu2017CoreShellYarnBasedTN,
  title={Core-Shell-Yarn-Based Triboelectric Nanogenerator Textiles as Power Cloths.},
  author={Aifang Yu and Xiong Pu and Rongmei Wen and Mengmeng Liu and Tao Zhou and Ke Zhang and Yang Zhang and Junyi Zhai and Weiguo Hu and Zhong Lin Wang},
  journal={ACS nano},
  year={2017},
  volume={11 12},
  pages={
          12764-12771
        },
  url={https://api.semanticscholar.org/CorpusID:206717452}
}


@Inbook{Wang2023-chapter1,
author="Wang, Zhong Lin",
editor="Wang, Zhong Lin
and Yang, Ya
and Zhai, Junyi
and Wang, Jie",
title="Introduction to Triboelectric Nanogenerators",
bookTitle="Handbook of Triboelectric Nanogenerators",
year="2023",
publisher="Springer International Publishing",
address="Cham",
pages="3--32",
abstract="Triboelectric nanogenerator (TENG) was first invented by Zhong Lin Wang's group in 2012 for converting small-scale mechanical energy into electricity by a conjunction of triboelectrification and electrostatic induction. TENG is a paradigm shift technology and has unprecedented performances. TENG uses neither magnets nor coils; it is light in mass, low in density, low in cost, and can be fabricated using most of organic materials. Most importantly, in contrast to the classical electromagnetic generator, TENG works the best at low frequency (<5--10 Hz); thus, it is the unique choice for harvesting low-frequency energy from body motion and ocean waves (the blue energy). TENG can also be used as a self-powered sensor for actively detecting the static and dynamic processes arising from mechanical agitation using the voltage and current output signals, respectively, with applications such as mechanical sensors, physiological detection, motion sensing, touchpad, and electronic skin technologies.",
isbn="978-3-031-28111-2",
doi="10.1007/978-3-031-28111-2_1",
url="https://doi.org/10.1007/978-3-031-28111-2_1"
}

@article{High-Energy-Asymmetric-Supercapacitor,
author = {Liu, Mengmeng and Cong, Zifeng and Pu, Xiong and Guo, Wenbin and Liu, Ting and Li, Meng and Zhang, Yang and Hu, Weiguo and Wang, Zhong Lin},
title = {High-Energy Asymmetric Supercapacitor Yarns for Self-Charging Power Textiles},
journal = {Advanced Functional Materials},
volume = {29},
number = {41},
pages = {1806298},
keywords = {asymmetric supercapacitors, self-charging power textile, smart textiles, triboelectric nanogenerators},
doi = {https://doi.org/10.1002/adfm.201806298},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/adfm.201806298},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/adfm.201806298},
abstract = {Abstract Rapid growth of electronic textile increases the demand for textile-based power sources, which should have comparable lightweight, flexibility, and comfort. In this work, a self-charging power textile interwoven by all-yarn-based energy-harvesting triboelectric nanogenerators (TENG) and energy-storing yarn-type asymmetric supercapacitors (Y-ASC) is reported. Common polyester yarns with conformal Ni/Cu coating are utilized as 1D current collectors in Y-ASCs and electrodes in TENGs. The solid-state Y-ASC achieves high areal energy density (≈78.1 µWh cm−2), high power density (14 mW cm−2), stable cycling performance (82.7\% for 5000 cycles), and excellent flexibility (1000 cycles bending for 180°). The TENG yarn can be woven into common fabrics with desired stylish designs to harvest energy from human daily motions at high output (≈60 V open-circuit voltage and ≈3 µA short-circuit current). The integrated self-charging power textile is demonstrated to power an electronic watch without extra recharging by other power sources, suggesting its promising applications in electronic textiles and wearable electronics.},
year = {2019}
}


-- Related Works --

@article{HuangHapticWearable,
title = {Recent advances in multi-mode haptic feedback technologies towards wearable interfaces},
journal = {Materials Today Physics},
volume = {22},
pages = {100602},
year = {2022},
issn = {2542-5293},
doi = {https://doi.org/10.1016/j.mtphys.2021.100602},
url = {https://www.sciencedirect.com/science/article/pii/S2542529321002637},
author = {Ya Huang and Kuanming Yao and Jiyu Li and Dengfeng Li and Huiling Jia and Yiming Liu and Chun Ki Yiu and Wooyoung Park and Xinge Yu},
keywords = {Haptic interfaces, Wearable technologies, Mechanical actuators, Thermal actuators, Electrostimulation},
}

@ARTICLE{JiangWearableGestureControl,
  author={Jiang, Shuo and Kang, Peiqi and Song, Xinyu and Lo, Benny P.L. and Shull, Peter B.},
  journal={IEEE Reviews in Biomedical Engineering}, 
  title={Emerging Wearable Interfaces and Algorithms for Hand Gesture Recognition: A Survey}, 
  year={2022},
  volume={15},
  number={},
  pages={85-102},
  keywords={Gesture recognition;Prosthetics;Wrist;Exoskeletons;Training;Stroke (medical condition);Machine learning algorithms;Rehabilitation;human-computer interaction;machine learning;electromyography;forcemyography},
  doi={10.1109/RBME.2021.3078190}
}

@article{LegnerSweatSensing,
title = {Sweat sensing in the smart wearables era: Towards integrative, multifunctional and body-compliant perspiration analysis},
journal = {Sensors and Actuators A: Physical},
volume = {296},
pages = {200-221},
year = {2019},
issn = {0924-4247},
doi = {https://doi.org/10.1016/j.sna.2019.07.020},
url = {https://www.sciencedirect.com/science/article/pii/S0924424719307915},
author = {Christopher Legner and Upender Kalwa and Vishal Patel and Austin Chesmore and Santosh Pandey},
keywords = {Sweat sensing, Physiological sensors, Wearable devices, Big Data, Data analytics, Flexible electronics, Multifunctional sensing, Wearable sensor companies}
}

@inproceedings{ChoiBodyPrinter,
author = {Choi, Youngkyung and Ryu, Neung and Kim, Myung Jin and Dementyev, Artem and Bianchi, Andrea},
title = {BodyPrinter: Fabricating Circuits Directly on the Skin at Arbitrary Locations Using a Wearable Compact Plotter},
year = {2020},
isbn = {9781450375146},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3379337.3415840},
doi = {10.1145/3379337.3415840},
booktitle = {Proceedings of the 33rd Annual ACM Symposium on User Interface Software and Technology},
pages = {554–564},
numpages = {11},
keywords = {on-body fabrication, skin electronics, wearable},
location = {Virtual Event, USA},
series = {UIST '20}
}

@inproceedings{PourjafarianBodyPrinter,
author = {Pourjafarian, Narjes and Koelle, Marion and Fruchard, Bruno and Mavali, Sahar and Klamka, Konstantin and Groeger, Daniel and Strohmeier, Paul and Steimle, J\"{u}rgen},
title = {BodyStylus: Freehand On-Body Design and Fabrication of Epidermal Interfaces},
year = {2021},
isbn = {9781450380966},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3411764.3445475},
doi = {10.1145/3411764.3445475},
booktitle = {Proceedings of the 2021 CHI Conference on Human Factors in Computing Systems},
articleno = {504},
numpages = {15},
keywords = {wearable computing, skin, pen-based interaction, on-body fabrication, epidermal devices, craft, On-body design},
series = {CHI '21}
}

@inproceedings{KaoNailO,
author = {Kao, Hsin-Liu (Cindy) and Dementyev, Artem and Paradiso, Joseph A. and Schmandt, Chris},
title = {NailO: Fingernails as an Input Surface},
year = {2015},
isbn = {9781450331456},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/2702123.2702572},
doi = {10.1145/2702123.2702572},
booktitle = {Proceedings of the 33rd Annual ACM Conference on Human Factors in Computing Systems},
pages = {3015–3018},
numpages = {4},
keywords = {beauty technology, capacitive touch, gesture recognition, printed electronics, wearable electronics},
location = {Seoul, Republic of Korea},
series = {CHI '15}
}

@inproceedings{ZhuBioWeave,
author = {Zhu, Jingwen and El Nesr, Nadine and Simon, Christina and Rettenmaier, Nola and Beiler, Kaitlyn and Kao, Cindy Hsin-Liu},
title = {BioWeave: Weaving Thread-Based Sweat-Sensing On-Skin Interfaces},
year = {2023},
isbn = {9798400701320},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3586183.3606769},
doi = {10.1145/3586183.3606769},
booktitle = {Proceedings of the 36th Annual ACM Symposium on User Interface Software and Technology},
articleno = {35},
numpages = {11},
keywords = {weaving, wearables, textiles, sweat sensing, on-skin interfaces, biosensing},
series = {UIST '23}
}

@article{SinghaWearableSmartTextiles,
title = {Recent Advancements in Wearable \& Smart Textiles: An Overview},
journal = {Materials Today: Proceedings},
volume = {16},
pages = {1518-1523},
year = {2019},
note = {Shape Memory Applications, Research and Technology 2018},
issn = {2214-7853},
doi = {https://doi.org/10.1016/j.matpr.2019.05.334},
url = {https://www.sciencedirect.com/science/article/pii/S2214785319311903},
author = {Kunal Singha and Jayant Kumar and Pintu Pandit},
keywords = {Wearable e textiles, Smart textiles, Conductive polymers},
}

@inproceedings{ZhuETextileProduction,
author = {Zhu, Jingwen and Kao, Hsin-Liu (Cindy)},
title = {Scaling E-Textile Production: Understanding the Challenges of Soft Wearable Production for Individual Creators},
year = {2022},
isbn = {9781450394246},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3544794.3558475},
doi = {10.1145/3544794.3558475},
booktitle = {Proceedings of the 2022 ACM International Symposium on Wearable Computers},
pages = {94–99},
numpages = {6},
keywords = {wearable technology, low-volume manufacturing, E-textiles},
location = {Cambridge, United Kingdom},
series = {ISWC '22}
}

@inproceedings{YuPositionAwareKnit,
author = {Yu, Tianhong Catherine and Arakawa, Riku and McCann, James and Goel, Mayank},
title = {uKnit: A Position-Aware Reconfigurable Machine-Knitted Wearable for Gestural Interaction and Passive Sensing using Electrical Impedance Tomography},
year = {2023},
isbn = {9781450394215},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3544548.3580692},
doi = {10.1145/3544548.3580692},
booktitle = {Proceedings of the 2023 CHI Conference on Human Factors in Computing Systems},
articleno = {628},
numpages = {17},
keywords = {Electrical Impedance Tomography, Gestural Interaction, Machine Knitting, Reconfigurable Wearable, Smart Textile},
series = {CHI '23}
}

@inproceedings{PoupyrevJacquard,
author = {Poupyrev, Ivan and Gong, Nan-Wei and Fukuhara, Shiho and Karagozler, Mustafa Emre and Schwesig, Carsten and Robinson, Karen E.},
title = {Project Jacquard: Interactive Digital Textiles at Scale},
year = {2016},
isbn = {9781450333627},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/2858036.2858176},
doi = {10.1145/2858036.2858176},
booktitle = {Proceedings of the 2016 CHI Conference on Human Factors in Computing Systems},
pages = {4216–4227},
numpages = {12},
keywords = {information interfaces and presentation},
location = {San Jose, California, USA},
series = {CHI '16}
}

@article{AtalayTextileMotionTracking,
author = {Atalay, Asli and Sanchez, Vanessa and Atalay, Ozgur and Vogt, Daniel M. and Haufe, Florian and Wood, Robert J. and Walsh, Conor J.},
title = {Batch Fabrication of Customizable Silicone-Textile Composite Capacitive Strain Sensors for Human Motion Tracking},
journal = {Advanced Materials Technologies},
volume = {2},
number = {9},
pages = {1700136},
keywords = {capacitive, motion tracking, soft sensors, stretchable, textile-based sensors},
doi = {https://doi.org/10.1002/admt.201700136},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/admt.201700136},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/admt.201700136},
year = {2017}
}

@article{ZhangCarbonNanotube,
title = {Carbon nanotube polymer coatings for textile yarns with good strain sensing capability},
journal = {Sensors and Actuators A: Physical},
volume = {179},
pages = {83-91},
year = {2012},
issn = {0924-4247},
doi = {https://doi.org/10.1016/j.sna.2012.03.029},
url = {https://www.sciencedirect.com/science/article/pii/S0924424712001938},
author = {Rui Zhang and Hua Deng and Renata Valenca and Junhong Jin and Qiang Fu and Emiliano Bilotti and Ton Peijs},
keywords = {Carbon nanotube, Conductive, Polymer, Composite, Fibre, Sensor},
abstract = {In this study, a commercially available Spandex multifilament yarn was coated with a thermoplastic polyurethane/carbon nanotube (TPU/CNT) conductive polymer composite (CPC), and conductive elastic yarns with good strain sensing ability were achieved with equivalent CNT concentrations as low as 0.015wt.%. The resistance per meter coated yarn decreased with increasing CNT concentration in the CPC coating, while in the case of a homogeneous coating, the CPC concentration in the coating solution did not have a significant effect on the resistance per meter coated yarn. Upon cyclic loading, the strain sensing behaviour showed partial recovery of resistance in the first loading cycle, while good reversibility was observed a number of cycles, giving these materials good potential as sensors for smart textiles.}
}

@inproceedings{ShahmiriSerpentine,
author = {Shahmiri, Fereshteh and Chen, Chaoyu and Waghmare, Anandghan and Zhang, Dingtian and Mittal, Shivan and Zhang, Steven L. and Wang, Yi-Cheng and Wang, Zhong Lin and Starner, Thad E. and Abowd, Gregory D.},
title = {Serpentine: A Self-Powered Reversibly Deformable Cord Sensor for Human Input},
year = {2019},
isbn = {9781450359702},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3290605.3300775},
doi = {10.1145/3290605.3300775},
abstract = {We introduce Serpentine, a self-powered sensor that is a reversibly deformable cord capable of sensing a variety of human input. The material properties and structural design of Serpentine allow it to be flexible, twistable, stretchable and squeezable, enabling a broad variety of expressive input modalities. The sensor operates using the principle of Triboelectric Nanogenerators (TENG), which allows it to sense mechanical deformation without an external power source. The affordances of the cord include six interactions---Pluck, Twirl, Stretch, Pinch, Wiggle and Twist. Serpentine demonstrates the ability to simultaneously recognize these inputs through a single physical interface. A 12-participant user study illustrates 95.7\% accuracy for a user-dependent recognition model using a realtime system and 92.17\% for user-independent offline detection. We conclude by demonstrating how Serpentine can be employed in everyday ubiquitous computing applications.},
booktitle = {Proceedings of the 2019 CHI Conference on Human Factors in Computing Systems},
pages = {1–14},
numpages = {14},
keywords = {input devices, self-powered sensor, soft electronics, tangible interfaces, triboelectric nanogenerator, ubiquitous computing},
location = {Glasgow, Scotland Uk},
series = {CHI '19}
}

@inproceedings{DevendorfPlyingSmartTextiles,
author = {Devendorf, Laura and Di Lauro, Chad},
title = {Adapting Double Weaving and Yarn Plying Techniques for Smart Textiles Applications},
year = {2019},
isbn = {9781450361965},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3294109.3295625},
doi = {10.1145/3294109.3295625},
abstract = {Smart textiles integrate sensing and actuation components into their structures to bring interactivity to fabrics. We describe how we adapted two existing fiber arts techniques, double weaving and yarn plying, for the purpose of creating a woven textile that changes color in response to touch. We draw from this experience to make three core contributions: descriptions of our experiments plying yarns that change between three color states; descriptions of double weaving structures that allow us to support interactivity while hiding circuitry from view; and suggestions for how these techniques could be adapted and extended by other researchers to make richly crafted and technologically sophisticated fabrics.},
booktitle = {Proceedings of the Thirteenth International Conference on Tangible, Embedded, and Embodied Interaction},
pages = {77–85},
numpages = {9},
keywords = {craft, hand-weaving, smart textiles, yarn plying},
location = {Tempe, Arizona, USA},
series = {TEI '19}
}

@inproceedings{KiaghadiFabricAsSensor,
author = {Kiaghadi, Ali and Baima, Morgan and Gummeson, Jeremy and Andrew, Trisha and Ganesan, Deepak},
title = {Fabric as a Sensor: Towards Unobtrusive Sensing of Human Behavior with Triboelectric Textiles},
year = {2018},
isbn = {9781450359528},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3274783.3274845},
doi = {10.1145/3274783.3274845},
abstract = {Smart apparel with embedded sensors have the potential to revolutionize human behavior sensing by leveraging everyday clothing as the sensing substrate. However, existing textile-based sensing techniques rely on tight-fitting garments to obtain sufficient signal to noise, making it uncomfortable to wear and limiting the technology to niche applications like athletic performance monitoring.Our solution leverages functionalized fabric to measure the triboelectric charges induced by folding and compression of the textile itself, making it a more natural fit for everyday clothing. However, the large sensing surface of a functionalized textile also increases body-coupled noise and motion artifacts, and introduces new challenges in how we suppress noise to detect the weak triboelectric signal. We address these challenges using a combination of textile, electronics, and signal analysis-based innovations, and robustly sense joint motions by improving SNR and extracting highly discriminative features from the signal. Additionally, we demonstrate how the same sensor can be used to measure relative changes in skin moisture levels induced by sweating. Our design uses a simple-to-manufacture layered architecture that can be incorporated into any conventional, loosely worn textile. We show that the sensor has high performance in natural conditions by benchmarking the accuracy of sensing several kinematic metrics as well as sweat level. Additionally, we provide real-world performance evaluations across three application case studies including activity classification, perspiration measurements during exercise, and comfort level detection for HVAC systems.},
booktitle = {Proceedings of the 16th ACM Conference on Embedded Networked Sensor Systems},
pages = {199–210},
numpages = {12},
keywords = {Ubiquitous sensing, smart textile},
location = {Shenzhen, China},
series = {SenSys '18}
}

@inproceedings{ChenSPIN,
author = {Chen, Christopher and Howard, David and Zhang, Steven L. and Do, Youngwook and Sun, Sienna and Cheng, Tingyu and Wang, Zhong Lin and Abowd, Gregory D. and Oh, HyunJoo},
title = {SPIN (Self-powered Paper Interfaces): Bridging Triboelectric Nanogenerator with Folding Paper Creases},
year = {2020},
isbn = {9781450361071},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3374920.3374946},
doi = {10.1145/3374920.3374946},
abstract = {We present Self-powered Paper INterfaces (SPIN) combining folding paper creases with triboelectric nanogenerator (TENG). Embedding TENG into paper creases, we developed a design editor and set of fabrication techniques to create paper-based interfaces that power sensors and actuators. Our SPIN design editor enables users to design their own crease pattern by changing parameters, embed power generating modules into the design, estimate total power generation, and export the files. Then following the fabrication instructions, users can cut and crease materials, and assemble them to build their own interfaces. We employ repetitive push-and-pull based embodied interactions with the mechanism of paper creases and demonstrate four application examples that show new expressive possibilities applying different scales of embodied interactions.},
booktitle = {Proceedings of the Fourteenth International Conference on Tangible, Embedded, and Embodied Interaction},
pages = {431–442},
numpages = {12},
keywords = {teng (triboelectric nanogenerator), self-powered tangible interface, paper interface, paper electronics},
location = {Sydney NSW, Australia},
series = {TEI '20}
}

@Article{HossainPiezoelectricTextile,
AUTHOR = {Hossain, Ishtia Zahir and Khan, Ashaduzzaman and Hossain, Gaffar},
TITLE = {A Piezoelectric Smart Textile for Energy Harvesting and Wearable Self-Powered Sensors},
JOURNAL = {Energies},
VOLUME = {15},
YEAR = {2022},
NUMBER = {15},
ARTICLE-NUMBER = {5541},
URL = {https://www.mdpi.com/1996-1073/15/15/5541},
ISSN = {1996-1073},
ABSTRACT = {Today’s wearable electronics have dramatically altered our daily lives and created an urgent demand for new and intelligent sensor technologies. As a new energy source, self-powering sensors are currently seen as critically important units for wearable and non-wearable textile–electronic systems. To this aim, this paper presents a smart textile-based piezoelectric energy-autonomous harvester and a self-powered sensor for wearable application, where the sandwich structure of the wearable sensor consists of top and bottom textile conductors, and in between the two textile electrodes there is a piezoelectric PVDF thin film. The generating voltage, current, charge, power, and capacitor charging–discharging behaviour of the device were confirmed using multimeter, oscilloscope, Keithley, etc., analyses. Finally, a piezoelectric-textile sensor was integrated into wearable clothes for breathing detection; a shoe insole for footstep recognition; and it can store energy by tapping, to power electronics, such as a calculator, timer, LED, etc., at a later time. The sensitivity of the sensor was enough for generating voltage from a tiny water droplet. Thus, we can assume raindrops to be utilized as a power-generating source on days when no sun is available to solar cells.},
DOI = {10.3390/en15155541}
}









@article{LeeElectromagneticWearable,
author = {Hyewon Lee and Jung-Sim Roh},
title ={Wearable electromagnetic energy-harvesting textiles based on human walking},
journal = {Textile Research Journal},
volume = {89},
number = {13},
pages = {2532-2541},
year = {2019},
doi = {10.1177/0040517518797349},
URL = {https://doi.org/10.1177/0040517518797349},eprint = {https://doi.org/10.1177/0040517518797349},
abstract = { The need for self-generating energy for outdoor environments is growing. To cope with emergencies in outdoor environments, sustainable, environment-independent energy-harvesting methods based on natural human movements are necessary. In this study, we developed a wearable energy-harvesting textile with a structure capable of generating the maximum energy from the swinging motion that occurs during walking. Two types of conductive yarn were manufactured and, when used as coils, are as durable as wire coils and have excellent flexibility and wearability, allowing easy integration into outdoor garments. Design variables related to the effect of energy production were investigated and the wearable energy-harvesting textile was evaluated by the average current generated. The conductive yarn coils can be connected in a serial circuit method and were evaluated to generate energy at a greater efficiency than wire coils. The average current increased as the number of turns of coil, the magnetic field, and the coil swing speed increased. The average currents along the distance between the magnet and the coil varied with magnet forces inversely proportional to distance. }
}



@inproceedings{PointnerKnittedResi,
author = {Pointner, Andreas and Preindl, Thomas and Mlakar, Sara and Aigner, Roland and Haller, Michael},
title = {Knitted RESi: A Highly Flexible, Force-Sensitive Knitted Textile Based on Resistive Yarns},
year = {2020},
isbn = {9781450379670},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3388534.3407292},
doi = {10.1145/3388534.3407292},
abstract = {We demonstrate a force sensing knitted textile, based on a piezo-resistive yarn. The resulting elastic, stretchable, and robust textile exhibits sensors based on the widespread Force Sensitive Resistor (FSR) principle. As a proof-of-concept, we implemented a knit consisting of multiple piezo-resistive wales, each intersecting with a single vertical piezo-resistive insert, spawning discrete FSRs at the respective intersection points. While enabling monitoring of external stress, such as pressure, stretch, and deformation, the textile features inherent pleasant haptic qualities.},
booktitle = {ACM SIGGRAPH 2020 Emerging Technologies},
articleno = {21},
numpages = {2},
keywords = {Conductive Yarn, FSR, Interactive Textiles, Smart Textiles, Textile Sensor, Wearables},
location = {Virtual Event, USA},
series = {SIGGRAPH '20}
}

@article{OuSensorKnit,
  title={SensorKnit: architecting textile sensors with machine knitting},
  author={Ou, Jifei and Oran, Daniel and Haddad, Don Derek and Paradiso, Joseph and Ishii, Hiroshi},
  journal={3D Printing and Additive Manufacturing},
  volume={6},
  number={1},
  pages={1--11},
  year={2019},
  publisher={Mary Ann Liebert, Inc., publishers 140 Huguenot Street, 3rd Floor New~…}
}

@inproceedings{WuIWood,
author = {Wu, Te-Yen and Yang, Xing-Dong},
title = {iWood: Makeable Vibration Sensor for Interactive Plywood},
year = {2022},
isbn = {9781450393201},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3526113.3545640},
doi = {10.1145/3526113.3545640},
abstract = {iWood is interactive plywood that can sense vibration based on triboelectric effect. As a material, iWood survives common woodworking operations, such as sawing, screwing, and nailing and can be used to create furniture and artifacts. Things created using iWood inherit its sensing capability and can detect a variety of user input and activities based on their unique vibration patterns. Through a series of experiments and machine simulations, we carefully chose the size of the sensor electrodes, the type of triboelectric materials, and the bonding method of the sensor layers to optimize the sensitivity and fabrication complexity. The sensing performance of iWood was evaluated with 4 gestures and 12 daily activities carried out on a table, nightstand, and cutting board, all created using iWood. Our result suggested over 90\% accuracies for activity and gesture recognition.},
booktitle = {Proceedings of the 35th Annual ACM Symposium on User Interface Software and Technology},
articleno = {11},
numpages = {12},
keywords = {vibration sensing, makeable sensor, Interactive wood},
location = {Bend, OR, USA},
series = {UIST '22}
}

@article{AroraSATURN,
author = {Arora, Nivedita and Starner, Thad and Abowd, Gregory D.},
title = {SATURN: an introduction to the internet of materials},
year = {2020},
issue_date = {December 2020},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {63},
number = {12},
issn = {0001-0782},
url = {https://doi.org/10.1145/3429948},
doi = {10.1145/3429948},
abstract = {We envision a new generation of computation devices, computational materials, which are self-sustainable, cheaply manufactured at scale and exhibit form factors that are easily incorporated into everyday environments. These materials can enable ordinary objects such as walls, carpet, furniture, jewelry, and cups to do computational things without looking like today's computational devices. Self-powered Audio Triboelectric Ultra-thin Rollable Nanogenerator (SATURN) is an early example of a computational material that can sense vibration, such as sound. SATURN can be manufactured from inexpensive components, is flexible so that it can be integrated into many different surfaces, and powers itself through the sound or vibration it is sensing. Using radio backscatter, we demonstrate that SATURN's sensed data is passively transmitted to remote computers, alleviating the need for batteries or any wired power for the material itself. The proliferation of these types of computational materials ushers an era of Internet of Materials, further blurring the distinction between the physical and digital worlds.},
journal = {Commun. ACM},
month = {nov},
pages = {92–99},
numpages = {8}
}

@article{VallettCapacitiveTouchFabric, title={Development of a Carbon Fiber Knitted Capacitive Touch Sensor}, volume={1}, DOI={10.1557/adv.2016.498}, number={38}, journal={MRS Advances}, author={Vallett, Richard and Young, Ryan and Knittel, Chelsea and Kim, Youngmoo and Dion, Genevieve}, year={2016}, pages={2641–2651}} <div></div>



@phdthesis{underwood2009design,
  title={The design of 3D shape knitted preforms},
  author={Underwood, Jenny},
  year={2009},
  school={RMIT University}
}

@inproceedings{Skinergy_UIST23,
author = {Yu, Tianhong Catherine and Wang, Nancy and Ellenbogen, Sarah and Kao, Cindy Hsin-Liu},
title = {Skinergy: Machine-Embroidered Silicone-Textile Composites as On-Skin Self-Powered Input Sensors},
year = {2023},
isbn = {9798400701320},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3586183.3606729},
doi = {10.1145/3586183.3606729},
abstract = {We propose Skinergy for self-powered on-skin input sensing, a step towards prolonged on-skin device usages. In contrast to prior on-skin gesture interaction sensors, Skinergy’s sensor operation does not require external power. Enabled by the triboelectric nanogenerator (TENG) phenomenon, the machine-embroidered silicone-textile composite sensor converts mechanical energy from the input interaction into electrical energy. Our proof-of-concept untethered sensing system measures the voltages of generated electrical signals which are then processed for a diverse set of sensing tasks: discrete touch detection, multi-contact detection, contact localization, and gesture recognition. Skinergy is fabricated with off-the-shelf materials. The aesthetic and functional designs can be easily customized and digitally fabricated. We characterize Skinergy and conduct a 10-participant user study to (1) evaluate its gesture recognition performance and (2) probe user perceptions and potential applications. Skinergy achieves 92.8\% accuracy for a 11-class gesture recognition task. Our findings reveal that human factors (e.g., individual differences in skin properties, and aesthetic preferences) are key considerations in designing self-powered on-skin sensors for human inputs.},
booktitle = {Proceedings of the 36th Annual ACM Symposium on User Interface Software and Technology},
articleno = {33},
numpages = {15},
location = {San Francisco, CA, USA},
series = {UIST '23}
}

@article{lu2021regulating,
  title={Regulating the high-voltage and high-impedance characteristics of triboelectric nanogenerator toward practical self-powered sensors},
  author={Lu, Shan and Lei, Wenqian and Gao, Lingxiao and Chen, Xin and Tong, Daqiao and Yuan, Pengfei and Mu, Xiaojing and Yu, Hua},
  journal={Nano Energy},
  volume={87},
  pages={106137},
  year={2021},
  publisher={Elsevier}
}




%---added by cindy 


@book{watkins2015functional,
  title={Functional clothing design: From sportswear to spacesuits},
  author={Watkins, Susan M and Dunne, Lucy},
  year={2015},
  publisher={Bloomsbury Publishing USA}
}

@article{valchinov2004bsn,
  title={An active electrode for biopotential recording from small localized bio-sources},
  author={Valchinov, Emil S and Pallikarakis, Nicolas E},
  journal={BioMedical Engineering OnLine},
  volume={3},
  number={1},
  pages={25},
  year={2004},
  publisher={BioMed Central}
}

@book{yang2006bsn,
  title={Body sensor networks},
  author={Yang, Guang-Zhong and Yang, Guangzhong},
  volume={1},
  year={2006},
  publisher={Springer}
}

@inproceedings{atallah2010bsn,
  title={Sensor placement for activity detection using wearable accelerometers},
  author={Atallah, Louis and Lo, Benny and King, Rachel and Yang, Guang-Zhong},
  booktitle={2010 International Conference on Body Sensor Networks},
  pages={24--29},
  year={2010},
  organization={IEEE}
}

@inproceedings{chi2010bsn,
  title={Wireless non-contact EEG/ECG electrodes for body sensor networks},
  author={Chi, Yu M and Cauwenberghs, Gert},
  booktitle={2010 International Conference on Body Sensor Networks},
  pages={297--301},
  year={2010},
  organization={IEEE}
}

@article{epstein1965cell,
  title={Cell renewal in human epidermis},
  author={Epstein, William L and Maibach, Howard I},
  journal={Archives of Dermatology},
  volume={92},
  number={4},
  pages={462--468},
  year={1965},
  publisher={American Medical Association}
}

@inproceedings{costa2016emotioncheck,
  title={EmotionCheck: leveraging bodily signals and false feedback to regulate our emotions},
  author={Costa, Jean and Adams, Alexander T and Jung, Malte F and Guimbreti{\`e}re, Fran{\c{c}}ois and Choudhury, Tanzeem},
  booktitle={Proceedings of the 2016 ACM International Joint Conference on Pervasive and Ubiquitous Computing},
  pages={758--769},
  year={2016},
  organization={ACM}
}

@inproceedings{li2011quantifiedself,
  title={Understanding my data, myself: supporting self-reflection with ubicomp technologies},
  author={Li, Ian and Dey, Anind K and Forlizzi, Jodi},
  booktitle={Proceedings of the 13th international conference on Ubiquitous computing},
  pages={405--414},
  year={2011},
  organization={ACM}
}


@article{weiser2002computer,
  title={The computer for the 21st century},
  author={Weiser, Mark},
  journal={IEEE pervasive computing},
  volume={1},
  number={1},
  pages={19--25},
  year={2002},
  publisher={IEEE}
}

@inproceedings{hofmann2019knitpicking,
  title={KnitPicking Textures: Programming and Modifying Complex Knitted Textures for Machine and Hand Knitting},
  author={Hofmann, Megan and Albaugh, Lea and Sethapakadi, Ticha and Hodgins, Jessica and Hudson, Scott E and McCann, James and Mankoff, Jennifer},
  booktitle={Proceedings of the 32nd Annual ACM Symposium on User Interface Software and Technology},
  pages={5--16},
  year={2019},
  organization={ACM}
}

@ARTICLE{vega2014beautytechnology, 
author={K. {Vega} and H. {Fuks}}, 
journal={Computer}, 
title={Beauty Technology: Body Surface Computing}, 
year={2014}, 
volume={47}, 
number={4}, 
pages={71-75}, 
keywords={social sciences computing;beauty technology;body surface computing;sensors;electronic devices;artificial nails;artificial makeup;wearable technology;Wearable computers;Wearable sensors;Radiofrequency identification;Human factors;wearable technology;miniature wearable devices;beauty technology}, 
doi={10.1109/MC.2014.81}, 
ISSN={0018-9162}, 
month={Apr},}

@misc{logicink,
  title         = "LogicInk",
  howpublished  = "\url{https://logicink.com}",
  note = {Accessed: 2020-11-12}
}

@misc{arvr,
  title         = "New Electronic Skin Allows You to Manipulate Virtual Objects",
  howpublished  = "\url{https://futurism.com/new-electronic-skin-manipulates-virtual-objects}",
  note = {Accessed: 2020-11-12}
}

@article{beans2018tattoo,
  title={Science and Culture: Wearable tech meets tattoo art in a bid to revolutionize both},
  author={Beans, Carolyn},
  journal={Proceedings of the National Academy of Sciences},
  volume={115},
  number={14},
  pages={3504--3506},
  year={2018},
  publisher={National Acad Sciences}
}

@inproceedings{you2019understanding,
  title={Understanding social perceptions towards interacting with on-skin interfaces in public},
  author={You, Chuang-Wen and Lin, Ya-Fang and Luo, Elle and Lin, Hung-Yeh and Kao, Hsin-Liu Cindy},
  booktitle={Proceedings of the 23rd International Symposium on Wearable Computers},
  pages={244--253},
  year={2019},
  organization={ACM}
}

@misc{skin7billion,
  title = {The growing \$7.5 billion market for Electronic Skin Patches | IDTechEx Research Article},
  howpublished = {\url{https://www.idtechex.com/en/research-article/the-growing-7-5-billion-market-for-electronic-skin-patches/17421}},
  note = {Accessed: 2020-11-12}
}

@misc{wearable50billion,
  title = {Wearable Technology Forecasts 2019-2029},
  howpublished = {\url{https://www.idtechex.com/en/research-report/wearable-technology-forecasts-2019-2029/680}},
  note = {Accessed: 2020-11-12}
}

@inproceedings{qi2010electronic,
  title={Electronic popables: exploring paper-based computing through an interactive pop-up book},
  author={Qi, Jie and Buechley, Leah},
  booktitle={Proceedings of the fourth international conference on Tangible, embedded, and embodied interaction},
  pages={121--128},
  year={2010},
  organization={ACM}
}

@inproceedings{duvall2016active,
  title={Active hugging vest for deep touch pressure therapy},
  author={Duvall, Julia C and Dunne, Lucy E and Schleif, Nicholas and Holschuh, Brad},
  booktitle={Proceedings of the 2016 ACM International Joint Conference on Pervasive and Ubiquitous Computing: Adjunct},
  pages={458--463},
  year={2016},
  organization={ACM}
}

@inproceedings{buechley2008lilypad,
  title={The LilyPad Arduino: using computational textiles to investigate engagement, aesthetics, and diversity in computer science education},
  author={Buechley, Leah and Eisenberg, Mike and Catchen, Jaime and Crockett, Ali},
  booktitle={Proceedings of the SIGCHI conference on Human factors in computing systems},
  pages={423--432},
  year={2008},
  organization={ACM}
}

@inproceedings{foo2019pressure,
  title={Iterative design and development of remotely-controllable, dynamic compression garment for novel haptic experiences},
  author={Foo, Esther W and Lee, J Walter and Ozbek, Simon and Compton, Crystal and Holschuh, Brad},
  booktitle={Proceedings of the 23rd International Symposium on Wearable Computers},
  pages={267--273},
  year={2019},
  organization={ACM}
}

@article{koester1991fashion,
  title={Fashion terms and styles for women's garments},
  author={Koester, Ardis W and Bryant, Nancy O and others},
  year={1991}
}

@book{chandler1995weaving,
  title={Learning to weave},
  author={Chandler, Deborah},
  year={1995},
  publisher={Interweave Press}
}

@article{fallman2010rtd,
  title={Establishing criteria of rigour and relevance in interaction design research},
  author={Fallman, Daniel and Stolterman, Erik},
  journal={Digital Creativity},
  volume={21},
  number={4},
  pages={265--272},
  year={2010},
  publisher={Taylor \& Francis}
}

@inproceedings{zimmerman2007rtd,
  title={Research through design as a method for interaction design research in HCI},
  author={Zimmerman, John and Forlizzi, Jodi and Evenson, Shelley},
  booktitle={Proceedings of the SIGCHI conference on Human factors in computing systems},
  pages={493--502},
  year={2007},
  organization={ACM}
}

@inproceedings{wang2017animskin,
  title={AnimSkin: fabricating epidermis with interactive, functional and aesthetic color animation},
  author={Wang, Yanan and Luo, Shijian and Lu, Yujia and Gong, Hebo and Zhou, Yexing and Liu, Shuai and Hansen, Preben},
  booktitle={Proceedings of the 2017 Conference on Designing Interactive Systems},
  pages={397--401},
  year={2017},
  organization={ACM}
}

@inproceedings{kao2016chromoskin,
  title={Chromoskin: Towards interactive cosmetics using thermochromic pigments},
  author={Kao, Hsin-Liu Cindy and Mohan, Manisha and Schmandt, Chris and Paradiso, Joseph A and Vega, Katia},
  booktitle={Proceedings of the 2016 CHI Conference Extended Abstracts on Human Factors in Computing Systems},
  pages={3703--3706},
  year={2016},
  organization={ACM}
}

@article{granberry2019compression,
  title={Functionally Graded Knitted Actuators with NiTi-Based Shape Memory Alloys for Topographically Self-Fitting Wearables},
  author={Granberry, Rachael and Eschen, Kevin and Holschuh, Brad and Abel, Julianna},
  journal={Advanced Materials Technologies},
  year={2019},
  publisher={Wiley Online Library}
}

@inproceedings{eschen2018compression,
  title={Active-Contracting Variable-Stiffness Fabrics for Self-Fitting Wearables},
  author={Eschen, Kevin and Abel, Julianna and Granberry, Rachael and Holschuh, Brad},
  booktitle={ASME 2018 Conference on Smart Materials, Adaptive Structures and Intelligent Systems},
  year={2018},
  organization={American Society of Mechanical Engineers Digital Collection}
}

@article{paradiso2005knit,
  title={A wearable health care system based on knitted integrated sensors},
  author={Paradiso, Rita and Loriga, Giannicola and Taccini, Nicola},
  journal={IEEE transactions on Information Technology in biomedicine},
  volume={9},
  number={3},
  pages={337--344},
  year={2005},
  publisher={IEEE}
}

@inproceedings{nittala2018multitouchskin,
  title={Multi-touch skin: A thin and flexible multi-touch sensor for on-skin input},
  author={Nittala, Aditya Shekhar and Withana, Anusha and Pourjafarian, Narjes and Steimle, J{\"u}rgen},
  booktitle={Proceedings of the 2018 CHI Conference on Human Factors in Computing Systems},
  pages={33},
  year={2018},
  organization={ACM}
}

@inproceedings{kao2018skinmorph,
  title={Skinmorph: texture-tunable on-skin interface through thin, programmable gel},
  author={Kao, Hsin-Liu Cindy and Bamforth, Miren and Kim, David and Schmandt, Chris},
  booktitle={Proceedings of the 2018 ACM International Symposium on Wearable Computers},
  pages={196--203},
  year={2018},
  organization={ACM}
}

@inproceedings{hamdan2019springlets,
  title={Springlets: Expressive, Flexible and Silent On-Skin Tactile Interfaces},
  author={Hamdan, Nur Al-huda and Wagner, Adrian and Voelker, Simon and Steimle, J{\"u}rgen and Borchers, Jan},
  booktitle={Proceedings of the 2019 CHI Conference on Human Factors in Computing Systems},
  pages={488},
  year={2019},
  organization={ACM}
}

@inproceedings{withana2018tacttoo,
  title={Tacttoo: A thin and feel-through tattoo for on-skin tactile output},
  author={Withana, Anusha and Groeger, Daniel and Steimle, J{\"u}rgen},
  booktitle={The 31st Annual ACM Symposium on User Interface Software and Technology},
  pages={365--378},
  year={2018},
  organization={ACM}
}

@inproceedings{hinckley2004stitching,
  title={Stitching: pen gestures that span multiple displays},
  author={Hinckley, Ken and Ramos, Gonzalo and Guimbretiere, Francois and Baudisch, Patrick and Smith, Marc},
  booktitle={Proceedings of the working conference on Advanced visual interfaces},
  pages={23--31},
  year={2004},
  organization={ACM}
}

@inproceedings{chen2014duet,
  title={Duet: exploring joint interactions on a smart phone and a smart watch},
  author={Chen, Xiang'Anthony' and Grossman, Tovi and Wigdor, Daniel J and Fitzmaurice, George},
  booktitle={Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
  pages={159--168},
  year={2014},
  organization={ACM}
}

@article{niu2019bodynet,
  title={A wireless body area sensor network based on stretchable passive tags},
  author={Niu, Simiao and Matsuhisa, Naoji and Beker, Levent and Li, Jinxing and Wang, Sihong and Wang, Jiechen and Jiang, Yuanwen and Yan, Xuzhou and Yun, Youngjun and Burnett, William and others},
  journal={Nature Electronics},
  volume={2},
  number={8},
  pages={361--368},
  year={2019},
  publisher={Nature Publishing Group}
}

@article{roetenberg2009xsens,
  title={Xsens MVN: Full 6DOF human motion tracking using miniature inertial sensors},
  author={Roetenberg, Daniel and Luinge, Henk and Slycke, Per},
  journal={Xsens Motion Technologies BV, Tech. Rep},
  volume={1},
  year={2009}
}

@inproceedings{guy2006wsn,
  title={Wireless sensor networks},
  author={Guy, Chris},
  booktitle={Sixth International Symposium on Instrumentation and Control Technology: Signal Analysis, Measurement Theory, Photo-Electronic Technology, and Artificial Intelligence},
  volume={6357},
  pages={63571I},
  year={2006},
  organization={International Society for Optics and Photonics}
}

@article{ruiz2006berkeleymote,
  title={Sensor development using Berkeley Mote platform},
  author={Ruiz-Sandoval, Manuel and Nagayama, Tomonori and Spencer Jr, BF},
  journal={Journal of Earthquake Engineering},
  volume={10},
  number={02},
  pages={289--309},
  year={2006},
  publisher={World Scientific}
}

@article{lai2013bodysensornetwork,
  title={A survey of body sensor networks},
  author={Lai, Xiaochen and Liu, Quanli and Wei, Xin and Wang, Wei and Zhou, Guoqiao and Han, Guangyi},
  journal={Sensors},
  volume={13},
  number={5},
  pages={5406--5447},
  year={2013},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@inproceedings{friske2019adacad,
 author = {Friske, Mikhaila and Wu, Shanel and Devendorf, Laura},
 title = {AdaCAD: Crafting Software For Smart Textiles Design},
 booktitle = {Proceedings of the 2019 CHI Conference on Human Factors in Computing Systems},
 series = {CHI '19},
 year = {2019},
 isbn = {978-1-4503-5970-2},
 location = {Glasgow, Scotland Uk},
 pages = {345:1--345:13},
 articleno = {345},
 numpages = {13},
 url = {http://doi.acm.org/10.1145/3290605.3300575},
 doi = {10.1145/3290605.3300575},
 acmid = {3300575},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {computer-aided design, smart textiles, weaving},
} 


@article{dhawan2004wovencircuits1,
author = {Dhawan, Anuj and Seyam, Abdelfattah and Ghosh, Tushar and Muth, John},
year = {2004},
month = {10},
pages = {913-919},
title = {Woven Fabric-Based Electrical Circuits: Part I: Evaluating Interconnect Methods},
volume = {74},
journal = {Textile Research Journal},
doi = {10.1177/004051750407401011}
}


@article{dhawan2004wovencircuits2,
author = {Dhawan, Anuj and Ghosh, Tushar K. and Seyam, Abdelfattah M. and Muth, John F.},
title ={Woven Fabric-Based Electrical Circuits: Part II: Yarn and Fabric Structures to Reduce Crosstalk Noise in Woven Fabric-Based Circuits},
journal = {Textile Research Journal},
volume = {74},
number = {11},
pages = {955-960},
year = {2004},
doi = {10.1177/004051750407401103},
URL = { 
        https://doi.org/10.1177/004051750407401103
    
},}
}


@ARTICLE{kim2010screenprinttextile, 
author={Y. {Kim} and H. {Kim} and H. {Yoo}}, 
journal={IEEE Transactions on Advanced Packaging}, 
title={Electrical Characterization of Screen-Printed Circuits on the Fabric}, 
year={2010}, 
volume={33}, 
number={1}, 
pages={196-205}, 
doi={10.1109/TADVP.2009.2034536}, 
ISSN={}, 
month={Feb},}

@article{yoshioka2006inkjetprint,
title = "Desktop inkjet printer as a tool to print conducting polymers",
journal = "Synthetic Metals",
volume = "156",
number = "11",
pages = "779 - 783",
year = "2006",
issn = "0379-6779",
doi = "https://doi.org/10.1016/j.synthmet.2006.03.013",
url = "http://www.sciencedirect.com/science/article/pii/S0379677906000919",
author = {Yoshioka, Yuka and Jabbour, Ghassan E.},
}


@INPROCEEDINGS{wijesiriwardana2004knitcircuit,
author={R. {Wijesiriwardana} and K. {Mitcham} and T. {Dias}},
booktitle={Eighth International Symposium on Wearable Computers},
title={Fibre-meshed transducers based real time wearable physiological information monitoring system},
year={2004},
volume={1},
number={},
pages={40-47},
doi={10.1109/ISWC.2004.20},
ISSN={},
month={Oct}}

@article{ou2019knitsensors,
author = {Ou, Jifei and Oran, Daniel and Haddad, Don D. and Paradiso, Joesph and Ishii, Hiroshi},
year = {2019},
month = {03},
pages = {1-11},
title = {SensorKnit: Architecting Textile Sensors with Machine Knitting},
volume = {6},
journal = {3D Printing and Additive Manufacturing},
doi = {10.1089/3dp.2018.0122},
}

@inproceedings{albaugh2019softactuatedobjects,
 author = {Albaugh, Lea and Hudson, Scott and Yao, Lining},
 title = {Digital Fabrication of Soft Actuated Objects by Machine Knitting},
 booktitle = {Proceedings of the 2019 CHI Conference on Human Factors in Computing Systems},
 series = {CHI '19},
 year = {2019},
 isbn = {978-1-4503-5970-2},
 location = {Glasgow, Scotland Uk},
 pages = {184:1--184:13},
 articleno = {184},
 numpages = {13},
 url = {http://doi.acm.org/10.1145/3290605.3300414},
 doi = {10.1145/3290605.3300414},
 acmid = {3300414},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {additive manufacturing, computational crafts, soft actuator, soft materials},
} 

@inproceedings{bonderover2004woveninverter,
  author={E. {Bonderover} and S. {Wagner}},
  journal={IEEE Electron Device Letters},
  title={A woven inverter circuit for e-textile applications},
  year={2004},
  volume={25},
  number={5},
  pages={295-297},
  keywords={thin film transistors;amorphous semiconductors;invertors;silicon;woven inverter circuit;electronic circuits;specialized component fibers;electronic components integration;contact pads;flexible fabric;amorphous silicon thin-film transistors;active device;device fiber;electronic textile;Si;Inverters;Circuits;Optical fiber devices;Thin film transistors;Conductors;Weaving;Textile fibers;Contacts;Silicon;Fabrics},
  doi={10.1109/LED.2004.826537},
  ISSN={},
  month={May},
}

@inproceedings{hamdan2018chi,
 author = {Hamdan, Nur Al-huda and Voelker, Simon and Borchers, Jan},
 title = {Sketch\&\#38;Stitch: Interactive Embroidery for E-textiles},
 booktitle = {Proceedings of the 2018 CHI Conference on Human Factors in Computing Systems},
 series = {CHI '18},
 year = {2018},
 isbn = {978-1-4503-5620-6},
 location = {Montreal QC, Canada},
 pages = {82:1--82:13},
 articleno = {82},
 numpages = {13},
 url = {http://doi.acm.org/10.1145/3173574.3173656},
 doi = {10.1145/3173574.3173656},
 acmid = {3173656},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {e-textile, embroidery, interactive fabrication, physical sketching},
} 



@INPROCEEDINGS{zeagler2012jogwheel,
author={C. {Zeagler} and S. {Gilliland} and H. {Profita} and T. {Starner}},
booktitle={2012 16th International Symposium on Wearable Computers},
title={Textile Interfaces: Embroidered Jog-Wheel, Beaded Tilt Sensor, Twisted Pair Ribbon, and Sound Sequins},
year={2012},
volume={},
number={},
pages={60-63},
doi={10.1109/ISWC.2012.29},
ISSN={},
month={June},}

@inproceedings{karrer2011pinstripe,
author = {Karrer, Thorsten and Wittenhagen, Moritz and Lichtschlag, Leonhard and Heller, Florian and Borchers, Jan},
title = {Pinstripe: Eyes-Free Continuous Input on Interactive Clothing},
year = {2011},
isbn = {9781450302289},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/1978942.1979137},
doi = {10.1145/1978942.1979137},
booktitle = {Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
pages = {1313–1322},
numpages = {10},
keywords = {smart textiles, continuous input, wearable computing, eyes-free interaction},
location = {Vancouver, BC, Canada},
series = {CHI '11}
}

@inproceedings{schneegass2015simpleskin,
author = {Schneegass, Stefan and Hassib, Mariam and Zhou, Bo and Cheng, Jingyuan and Seoane, Fernando and Amft, Oliver and Lukowicz, Paul and Schmidt, Albrecht},
title = {SimpleSkin: Towards Multipurpose Smart Garments},
year = {2015},
isbn = {9781450335751},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/2800835.2800935},
doi = {10.1145/2800835.2800935},
pages = {241–244},
numpages = {4},
keywords = {system prototype, smart textiles},
location = {Osaka, Japan},
series = {UbiComp/ISWC'15 Adjunct}
}

@inproceedings{chan2017data,
author = {Chan, Justin and Gollakota, Shyamnath},
title = {Data Storage and Interaction Using Magnetized Fabric},
year = {2017},
isbn = {9781450349819},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3126594.3126620},
doi = {10.1145/3126594.3126620},
booktitle = {Proceedings of the 30th Annual ACM Symposium on User Interface Software and Technology},
pages = {655–663},
numpages = {9},
keywords = {wearables computing, conductive thread, e-textiles, data storage, smart fabrics, gesture interaction},
location = {Qu\'{e}bec City, QC, Canada},
series = {UIST '17}
}

@inproceedings{williams2015swarm,
author = {Williams, Michele A. and Roseway, Asta and O'Dowd, Chris and Czerwinski, Mary and Morris, Meredith Ringel},
title = {SWARM: An Actuated Wearable for Mediating Affect},
year = {2015},
isbn = {9781450333054},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/2677199.2680565},
doi = {10.1145/2677199.2680565},
booktitle = {Proceedings of the Ninth International Conference on Tangible, Embedded, and Embodied Interaction},
pages = {293–300},
numpages = {8},
keywords = {emotions, accessibility, universal design, affective computing, stress management, wearable technology},
location = {Stanford, California, USA},
series = {TEI '15}
}

@inproceedings{kuusk2015lace,
author = {Kuusk, Kristi and Kooroshnia, Marjan and Mikkonen, Jussi},
title = {Crafting Butterfly Lace: Conductive Multi-Color Sensor-Actuator Structure},
year = {2015},
isbn = {9781450335751},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/2800835.2801669},
doi = {10.1145/2800835.2801669},
pages = {595–600},
numpages = {6},
keywords = {thermochromic inks, smart textiles, craft qualities},
location = {Osaka, Japan},
series = {UbiComp/ISWC'15 Adjunct}
}

@inproceedings{perner2010handcrafting,
author = {Perner-Wilson, Hannah and Buechley, Leah and Satomi, Mika},
title = {Handcrafting Textile Interfaces from a Kit-of-No-Parts},
year = {2010},
isbn = {9781450304788},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/1935701.1935715},
doi = {10.1145/1935701.1935715},
booktitle = {Proceedings of the Fifth International Conference on Tangible, Embedded, and Embodied Interaction},
pages = {61–68},
numpages = {8},
keywords = {construction kits, e-textiles, sensors, design methodology, workshops, personalization, craft materials, documentation, diy},
location = {Funchal, Portugal},
series = {TEI '11}
}

@INPROCEEDINGS{buechley2006lilypad,  author={L. {Buechley}},  booktitle={2006 10th IEEE International Symposium on Wearable Computers},   title={A Construction Kit for Electronic Textiles},   year={2006},  volume={},  number={},  pages={83-90},  doi={10.1109/ISWC.2006.286348}}


@inproceedings{berzowska2005kukkia,
  title={Kukkia and vilkas: Kinetic electronic garments},
  author={Berzowska, Joanna and Coelho, Marcelo},
  booktitle={Ninth IEEE International Symposium on Wearable Computers (ISWC'05)},
  pages={82--85},
  year={2005},
  organization={IEEE}
}

@inproceedings{hudson2014teddybear,
  title={Printing teddy bears: a technique for 3D printing of soft interactive objects},
  author={Hudson, Scott E},
  booktitle={Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
  pages={459--468},
  year={2014}
}


@inproceedings{nabil2019seamless,
  title={Seamless Seams: Crafting Techniques for Embedding Fabrics with Interactive Actuation},
  author={Nabil, Sara and Ku{\v{c}}era, Jan and Karastathi, Nikoletta and Kirk, David S and Wright, Peter},
  booktitle={Proceedings of the 2019 on Designing Interactive Systems Conference},
  pages={987--999},
  year={2019}
}

@inproceedings{lo2016dis,
 title = {Skintillates: Designing and Creating Epidermal Interactions},
 author = {Lo, Joanne and Lee, Doris Jung Lin and Wong, Nathan and Bui, David and Paulos, Eric},
 booktitle = {Proceedings of the 2016 ACM Conference on Designing Interactive Systems},
 series = {DIS '16},
 year = {2016},
 location = {Brisbane, QLD, Australia},
 publisher = {ACM},
}

@inproceedings{orth2018ubicomp,
 author = {Orth, Maggie and Smith, J. R. and Post, E. R. and Strickon, J. A. and Cooper, E. B.},
 title = {Musical Jacket},
 booktitle = {ACM SIGGRAPH 98  Electronic Art and Animation Catalog},
 series = {SIGGRAPH '98},
 year = {1998},
 isbn = {1-58113-045-7},
 location = {Orlando, Florida, USA},
 pages = {38--},
 url = {http://doi.acm.org/10.1145/281388.281456},
 doi = {10.1145/281388.281456},
 acmid = {281456},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@inproceedings{Weigel2016skinmarks,
 author = {Weigel, Martin and Nittala, Aditya Shekhar and Olwal, Alex and Steimle, J\"{u}rgen},
 title = {SkinMarks: Enabling Interactions on Body Landmarks Using Conformal Skin Electronics},
 booktitle = {Proc. CHI '17},
 pages = {3095--3105},
 year = {2017},
} 

@article {Araki2016LorealUVsensor,
author = {Araki, Hitoshi et al.},
title = {Materials and Device Designs for an Epidermal UV Colorimetric Dosimeter with Near Field Communication Capabilities},
journal = {Advanced Functional Materials},
volume = {27},
number = {2},
pages = {1604465--n/a},
year = {2017},
note = {1604465},
}


@article {Kim2011EpidermalElectronics,
	author = {Kim, Dae-Hyeong et al.},
	title = {Epidermal Electronics},
	volume = {333},
	number = {6044},
	pages = {838--843},
	year = {2011},
	publisher = {American Association for the Advancement of Science},
	journal = {Science}
}



@online{GoogleGlass,
    author = "Google",
    title = "Google Glass",
    url  = "https://www.x.company/glass",
    addendum = "(accessed: 03.01.2024)",
    keywords = "google glass",
}

@misc{SamsungGear,
  title = "Samsung Gear",
   howpublished = "\url{https://www.samsung.com/us/mobile/wearables/}",
  note = {Accessed: 2020-11-12}
}


@misc{AppleWatch,
  title =        "Apple Watch",
  howpublished = "\url{https://www.apple.com/watch/}",
  note = {Accessed: 2020-11-12}
}

@misc{MlCore,
  title =  "LSM6DSOX: Machine Learning Core",
  howpublished = "\url{https://www.st.com/resource/en/application_note/dm00563460-lsm6dsox-machine-learning-core-stmicroelectronics.pdf}",
  note = {Accessed: 2020-11-12}
}


@INPROCEEDINGS{rekimoto2011gesturewrist, 
author={J. Rekimoto}, 
booktitle={Proc. ISWC '01}, 
title={GestureWrist and GesturePad: unobtrusive wearable interaction devices},  
pages={21-27}, 
year = {2001},
}


@inproceedings{Ogata12,
 author = {Ogata, Masa and Sugiura, Yuta and Osawa, Hirotaka and Imai, Michita},
 title = {iRing: Intelligent Ring Using Infrared Reflection},
 booktitle = {Proc. UIST '12},
 year = {2012},
 pages = {131--136},
}


@INPROCEEDINGS{knight2002wearability, 
author={J. F. Knight and C. Baber and A. Schwirtz and H. W. Bristow}, 
booktitle={Proc. ISWC '02}, 
title={The comfort assessment of wearable computers}, 
pages={65-72}, 
year = {2002},
}



@inproceedings{Gemperle1998wearability,
  title={Design for wearability},
  author={Gemperle, Francine and Kasabach, Chris and Stivoric, John and Bauer, Malcolm and Martin, Richard},
  booktitle={Proc. ISWC '98},
  pages={116--122},
  year={1998},
}


@inproceedings{Zeagler2017wearablity,
 author = {Zeagler, Clint},
 title = {Where to Wear It: Functional, Technical, and Social Considerations in On-body Location for Wearable Technology 20 Years of Designing for Wearability},
 booktitle = {Proc. ISWC '17},
 pages = {150--157},
 year = {2017},
} 



@ARTICLE{Dipietro2008glovesurvey, 
author={L. Dipietro and A. M. Sabatini and P. Dario}, 
journal={IEEE Transactions on Systems, Man, and Cybernetics, Part C (Applications and Reviews)}, 
title={A Survey of Glove-Based Systems and Their Applications}, 
year={2008}, 
volume={38}, 
number={4}, 
pages={461-482},  
month={July},}


@INPROCEEDINGS{perng1999ASG, 
author={J. K. Perng and B. Fisher and S. Hollar and K. S. J. Pister}, 
booktitle={Proc. ISWC '99}, 
title={Acceleration sensing glove (ASG)}, 
pages={178-180}, 
year = {1999},
}


@INPROCEEDINGS{kevin2004cyberglove, 
author={N. Y. Y. Kevin and S. Ranganath and D. Ghosh}, 
booktitle={Proc. IEEE Region 10 Conference TENCON 2004}, 
title={Trajectory modeling in gesture recognition using CyberGloves and magnetic trackers}, 
volume={A}, 
number={}, 
pages={571-574 Vol. 1},
year = {2004},
month={Nov},}

@online{5DTGlove,
  title =        "Data Gloves - 5DT",
  howpublished = "\url{http://www.5dt.com/}",
  note = {Accessed: 2020-11-12}
}


@inproceedings{Zhang2015tomo,
 author = {Zhang, Yang and Harrison, Chris},
 title = {Tomo: Wearable, Low-Cost Electrical Impedance Tomography for Hand Gesture Recognition},
 booktitle = {Proc. UIST '15},
 pages = {167--173},
 year = {2015},
} 

@inproceedings{Fukui2011wristcontoursensor,
 author = {Fukui, Rui and Watanabe, Masahiko and Gyota, Tomoaki and Shimosaka, Masamichi and Sato, Tomomasa},
 title = {Hand Shape Classification with a Wrist Contour Sensor: Development of a Prototype Device},
 booktitle = {Proc. UbiComp '11},
 pages = {311--314},
 year = {2011},
} 

@inproceedings{Silina2015jewelry,
 author = {Silina, Yulia and Haddadi, Hamed},
 title = {New Directions in Jewelry: A Close Look at Emerging Trends and Developments in Jewelry-like Wearable Devices},
 booktitle = {Proc. ISWC '15},
 pages = {49--56},
 year = {2015},
} 

@online{Ringly,
  author =       "",
  year =         "2014",
  title =        "Ringly",
  url =           "https://ringly.com/",
  month = 	"",
  lastaccessed = "Oct 4, 2017",
}

@misc{IntelMICA,
  title =        "MICA Smart Bracelet Switches on New Fashion, Lifestyle Alerts",
  howpublished = "\url{"https://iq.intel.com/mica-smart-bracelet-switches-on-new-fashion-lifestyle-alerts/}",
    note = {Accessed: 2020-11-12}
}


@inproceedings{Liu2016wearability,
 author = {Liu, Xin and Vega, Katia and Maes, Pattie and Paradiso, Joe A.},
 title = {Wearability Factors for Skin Interfaces},
 booktitle = {Proc. AH '16},
 pages = {21:1--21:8},
 year = {2016},
} 


@inproceedings{Gemperle1998wearability,
  title={Design for wearability},
  author={Gemperle, Francine and Kasabach, Chris and Stivoric, John and Bauer, Malcolm and Martin, Richard},
  booktitle={Proc. ISWC '98},
  pages={116--122},
  year={1998},
}


@inproceedings{Zeagler2017wearablity,
 author = {Zeagler, Clint},
 title = {Where to Wear It: Functional, Technical, and Social Considerations in On-body Location for Wearable Technology 20 Years of Designing for Wearability},
 booktitle = {Proc. ISWC '17},
 pages = {150--157},
 year = {2017},
} 


@inproceedings{devendorf2019weaving,
  title={Adapting Double Weaving and Yarn Plying Techniques for Smart Textiles Applications},
  author={Devendorf, Laura and Di Lauro, Chad},
  booktitle={Proceedings of the Thirteenth International Conference on Tangible, Embedded, and Embodied Interaction},
  pages={77--85},
  year={2019},
  organization={ACM}
}

@inproceedings{markvicka2019electrodermis,
  title={ElectroDermis: Fully Untethered, Stretchable, and Highly-Customizable Electronic Bandages},
  author={Markvicka, Eric and Wang, Guanyun and Lee, Yi-Chin and Laput, Gierad and Majidi, Carmel and Yao, Lining},
  booktitle={Proceedings of the 2019 CHI Conference on Human Factors in Computing Systems},
  pages={632},
  year={2019},
  organization={ACM}
}


@inproceedings{granberry2017activestocking,
  title={Active knit compression stockings for the treatment of orthostatic hypotension},
  author={Granberry, Rachael and Abel, Julianna and Holschuh, Brad},
  booktitle={Proceedings of the 2017 ACM International Symposium on Wearable Computers},
  pages={186--191},
  year={2017},
  organization={ACM}
}

@inproceedings{gagliardi2018microclimate,
  title={Design of a Stitched Textile-Based Thermal Actuator Garment to Attenuate Peripheral Microclimate Experience},
  author={Gagliardi, Nika and Foo, Esther and Dupler, Ellen and Ozbek, Simon and Dunne, Lucy},
  booktitle={2018 Design of Medical Devices Conference},
  year={2018},
  organization={American Society of Mechanical Engineers Digital Collection}
}

@inproceedings{poupyrev2016jacquard,
  title={Project Jacquard: interactive digital textiles at scale},
  author={Poupyrev, Ivan and Gong, Nan-Wei and Fukuhara, Shiho and Karagozler, Mustafa Emre and Schwesig, Carsten and Robinson, Karen E},
  booktitle={Proceedings of the 2016 CHI Conference on Human Factors in Computing Systems},
  pages={4216--4227},
  year={2016},
  organization={ACM}
}

@incollection{feidakis2016physiolo,
  title={A review of emotion-aware systems for e-learning in virtual environments},
  author={Feidakis, M},
  booktitle={Formative assessment, learning data analytics and gamification},
  pages={217--242},
  year={2016},
  publisher={Elsevier}
}

@article{kim2019wearable,
  title={Wearable biosensors for healthcare monitoring},
  author={Kim, Jayoung and Campbell, Alan S and de {\'A}vila, Berta Esteban-Fern{\'a}ndez and Wang, Joseph},
  journal={Nature biotechnology},
  volume={37},
  number={4},
  pages={389--406},
  year={2019},
  publisher={Nature Publishing Group}
}

@inproceedings{liu2016wearability,
  title={Wearability factors for skin interfaces},
  author={Liu, Xin and Vega, Katia and Maes, Pattie and Paradiso, Joe A},
  booktitle={Proceedings of the 7th Augmented Human International Conference 2016},
  pages={21},
  year={2016},
  organization={ACM}
}

@inproceedings{weigel2015iskin,
  title={Iskin: flexible, stretchable and visually customizable on-body touch sensors for mobile computing},
  author={Weigel, Martin and Lu, Tong and Bailly, Gilles and Oulasvirta, Antti and Majidi, Carmel and Steimle, J{\"u}rgen},
  booktitle={Proceedings of the 33rd Annual ACM Conference on Human Factors in Computing Systems},
  pages={2991--3000},
  year={2015},
  organization={ACM}
}
@inproceedings{kao2016duoskin,
  title={DuoSkin: Rapidly prototyping on-skin user interfaces using skin-friendly materials},
  author={Kao, Hsin-Liu Cindy and Holz, Christian and Roseway, Asta and Calvo, Andres and Schmandt, Chris},
  booktitle={Proceedings of the 2016 ACM International Symposium on Wearable Computers},
  pages={16--23},
  year={2016},
  organization={ACM}
}

@inproceedings{lo2016skintillates,
 title = {Skintillates: Designing and Creating Epidermal Interactions},
 author = {Lo, Joanne and Lee, Doris Jung Lin and Wong, Nathan and Bui, David and Paulos, Eric},
 booktitle = {Proceedings of the 2016 ACM Conference on Designing Interactive Systems},
 series = {DIS '16},
 year = {2016},
 location = {Brisbane, QLD, Australia},
 publisher = {ACM},
}

@article{kim2011epidermal,
  author = {Kim, Dae-Hyeong and Lu, Nanshu and Ma, Rui and Kim, Yun-Soung and Kim, Rak-Hwan and Wang, Shuodao and Wu, Jian and Min Won, Sang and Tao, Hu and Islam, Ahmad and Yu, Ki and Kim, Tae-il and Chowdhury, Raeed and Ying, Ming and Xu, Lizhi and li, Ming and Chung, Hyun-joong and Keum, Hohyun and McCormick, Martin and A Rogers, John},
  year = {2011},
  month = {08},
  pages = {838-43},
  title = {Epidermal Electronics},
  volume = {333},
  journal = {Science (New York, N.Y.)},
  doi = {10.1126/science.1206157}
}

@article{kao2018skinwire,
  title={SkinWire: Fabricating a Self-Contained On-Skin PCB for the Hand},
  author={Kao, Hsin-Liu Cindy and Bedri, Abdelkareem and Lyons, Kent},
  journal={Proceedings of the ACM on Interactive, Mobile, Wearable and Ubiquitous Technologies},
  volume={2},
  number={3},
  pages={116},
  year={2018},
  publisher={ACM}
}

@Article{sample_ref,
  author = 	 {Fake Author1 and Imaginary Author2},
  title = 	 {Artificial generation of titles for research reports},
  journal =  {Journal of Imaginary Research},
  year = 	 {2002},
  volume = 	 {i},
  pages = 	 {1-2},
}

@inproceedings{sun2020wovenskin,
  title={Weaving a Second Skin: Exploring Opportunities for Crafting On-Skin Interfaces Through Weaving},
 author = {Sun, Ruojia and Onese, Ryosuke and Dunne, Margaret and Ling, Andrea and Denham, Amanda and Kao, Hsin-Liu (Cindy)},
 booktitle = {Proceedings of the 2020 ACM Conference on Designing Interactive Systems},
 series = {DIS '20},
 year = {2020},
 location = {Eindhoven, The Netherlands},
 publisher = {ACM},
}

@inproceedings{kao2017kino,
  title={Exploring interactions and perceptions of kinetic wearables},
  author={Kao, Hsin-Liu and Ajilo, Deborah and Anilionyte, Oksana and Dementyev, Artem and Choi, Inrak and Follmer, Sean and Schmandt, Chris},
  booktitle={Proceedings of the 2017 Conference on Designing Interactive Systems},
  pages={391--396},
  year={2017}
}

@article{shneiderman2006creativity,
  title={Creativity support tools: Report from a US National Science Foundation sponsored workshop},
  author={Shneiderman, Ben and Fischer, Gerhard and Czerwinski, Mary and Resnick, Mitch and Myers, Brad and Candy, Linda and Edmonds, Ernest and Eisenberg, Mike and Giaccardi, Elisa and Hewett, Tom and others},
  journal={International Journal of Human-Computer Interaction},
  volume={20},
  number={2},
  pages={61--77},
  year={2006},
  publisher={Taylor \& Francis}
}

@article{shneiderman2007creativity,
  title={Creativity support tools: Accelerating discovery and innovation},
  author={Shneiderman, Ben},
  journal={Communications of the ACM},
  volume={50},
  number={12},
  pages={20--32},
  year={2007},
  publisher={ACM New York, NY, USA}
}

@online{pbs2014challenges_on_skin,
  title =        "In 10 Years, You Won't Even Know You're Wearing Them",
  howpublished = "\url{https://www.pbs.org/wgbh/nova/article/wearable-health-sensors/}",
  note = {Accessed: 2020-06-10}
}


@misc{wu2017challenges_on_skin,
  title={Opportunities and challenges in flexible and stretchable electronics: A panel discussion at ISFSE2016},
  author={Wu, Zhigang and Huang, Yongan and Chen, Rong},
  year={2017},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@article{resnick2005design,
  title={Design principles for tools to support creative thinking},
  author={Resnick, Mitchel and Myers, Brad and Nakakoji, Kumiyo and Shneiderman, Ben and Pausch, Randy and Selker, Ted and Eisenberg, Mike},
  year={2005},
  publisher={Carnegie Mellon University}
}

@article{myers2000past,
  title={Past, present, and future of user interface software tools},
  author={Myers, Brad and Hudson, Scott E and Pausch, Randy},
  journal={ACM Transactions on Computer-Human Interaction (TOCHI)},
  volume={7},
  number={1},
  pages={3--28},
  year={2000},
  publisher={ACM New York, NY, USA}
}

@inproceedings{kao2017earthtones,
  title={Earthtones: Chemical sensing powders to detect and display environmental hazards through color variation},
  author={Kao, Cindy Hsin-Liu and Nguyen, Bichlien and Roseway, Asta and Dickey, Michael},
  booktitle={Proceedings of the 2017 CHI Conference Extended Abstracts on Human Factors in Computing Systems},
  pages={872--883},
  year={2017}
}


@inproceedings{kao2015nailo,
  title={NailO: fingernails as an input surface},
  author={Kao, Hsin-Liu and Dementyev, Artem and Paradiso, Joseph A and Schmandt, Chris},
  booktitle={Proceedings of the 33rd Annual ACM Conference on Human Factors in Computing Systems},
  pages={3015--3018},
  year={2015}
}


@inproceedings{dementyev2016rovables,
  title={Rovables: Miniature on-body robots as mobile wearables},
  author={Dementyev, Artem and Kao, Hsin-Liu and Choi, Inrak and Ajilo, Deborah and Xu, Maggie and Paradiso, Joseph A and Schmandt, Chris and Follmer, Sean},
  booktitle={Proceedings of the 29th Annual Symposium on User Interface Software and Technology},
  pages={111--120},
  year={2016}
}

@article{von2005democratizing,
  title={Democratizing Innovation MIT Press},
  author={Von Hippel, E},
  journal={Cambridge, MA},
  year={2005}
}


@article{papert1980mindstorms,
  title={Mindstorms: children, computers, and powerful ideas Basic Books},
  author={Papert, Seymour},
  journal={Inc. New York, NY},
  year={1980}
}

@book{buechley2013textilemessages,
  title={Textile Messages: Dispatches from the World of E-Textiles and Education. New Literacies and Digital Epistemologies. Volume 62.},
  author={Buechley, Leah and Peppler, Kylie and Eisenberg, Michael and Yasmin, Kafai},
  year={2013},
  publisher={ERIC}
}


@inproceedings{posch2019etextilekitreview,
  title={eTextiles: reviewing a practice through its tool/kits},
  author={Posch, Irene and Stark, Liza and Fitzpatrick, Geraldine},
  booktitle={Proceedings of the 23rd International Symposium on Wearable Computers},
  pages={195--205},
  year={2019}
}

@inproceedings{buechley2010longtail,
  title={LilyPad in the wild: how hardware's long tail is supporting new engineering and design communities},
  author={Buechley, Leah and Hill, Benjamin Mako},
  booktitle={Proceedings of the 8th ACM conference on designing interactive systems},
  pages={199--207},
  year={2010}
}


@inproceedings{buechley2005quiltsnaps,
  title={Quilt snaps: A fabric based computational construction kit},
  author={Buechley, Leah and Elumeze, Nwanua and Dodson, Camille and Eisenberg, Michael},
  booktitle={IEEE International Workshop on Wireless and Mobile Technologies in Education (WMTE'05)},
  pages={3--pp},
  year={2005},
  organization={IEEE}
}

@inproceedings{buechley2006constructionkitiswc,
  title={A construction kit for electronic textiles},
  author={Buechley, Leah},
  booktitle={2006 10th IEEE international symposium on wearable computers},
  pages={83--90},
  year={2006},
  organization={IEEE}
}

@inproceedings{kazemitabaar2017makerwear,
  title={Makerwear: A tangible approach to interactive wearable creation for children},
  author={Kazemitabaar, Majeed and McPeak, Jason and Jiao, Alexander and He, Liang and Outing, Thomas and Froehlich, Jon E},
  booktitle={Proceedings of the 2017 chi conference on human factors in computing systems},
  pages={133--145},
  year={2017}
}

@online{pbs2014challenges_on_skin,
  title =        "In 10 Years, You Won't Even Know You're Wearing Them",
  howpublished = "\url{https://www.pbs.org/wgbh/nova/article/wearable-health-sensors/}",
  note = {Accessed: 2020-06-10}
}

@online{flora,
  title =        "Announcing the FLORA, Adafruit’s wearable electronics platform and accessories.",
  howpublished = "\url{https://blog.adafruit.com/2012/01/20/announcing-the-floraadafruits-wearable-electronics-platform-and-accessories/}",
  note = {Accessed: 2020-06-10}
}


@inproceedings{katterfeldt2009eduwear,
  title={EduWear: smart textiles as ways of relating computing technology to everyday life},
  author={Katterfeldt, Eva-Sophie and Dittert, Nadine and Schelhowe, Heidi},
  booktitle={Proceedings of the 8th International Conference on Interaction Design and Children},
  pages={9--17},
  year={2009}
}

@inproceedings{ngai2010icatch,
  title={i* CATch: a scalable plug-n-play wearable computing framework for novices and children},
  author={Ngai, Grace and Chan, Stephen CF and Ng, Vincent TY and Cheung, Joey CY and Choy, Sam SS and Lau, Winnie WY and Tse, Jason TP},
  booktitle={Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
  pages={443--452},
  year={2010}
}

@inproceedings{ngai2009teeboard,
  title={The TeeBoard: an education-friendly construction platform for e-textiles and wearable computing},
  author={Ngai, Grace and Chan, Stephen CF and Cheung, Joey CY and Lau, Winnie WY},
  booktitle={Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
  pages={249--258},
  year={2009}
}


@article{ngai2013designingicatch,
  title={Designing i* CATch: A multipurpose, education-friendly construction kit for physical and wearable computing},
  author={Ngai, Grace and Chan, Stephen CF and Leong, Hong Va and Ng, Vincent TY},
  journal={ACM Transactions on Computing Education (TOCE)},
  volume={13},
  number={2},
  pages={1--30},
  year={2013},
  publisher={ACM New York, NY, USA}
}

@inproceedings{qi2014sketchingpapercircuits,
  title={Sketching in circuits: designing and building electronics on paper},
  author={Qi, Jie and Buechley, Leah},
  booktitle={Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
  pages={1713--1722},
  year={2014}
}

@inproceedings{rosner2012bookbinding,
  title={The material practices of collaboration},
  author={Rosner, Daniela K},
  booktitle={Proceedings of the ACM 2012 conference on computer supported cooperative work},
  pages={1155--1164},
  year={2012}
}

@inproceedings{cheatle2015furniture,
  title={Digital entanglements: craft, computation and collaboration in fine art furniture production},
  author={Cheatle, Amy and Jackson, Steven J},
  booktitle={Proceedings of the 18th ACM Conference on Computer Supported Cooperative Work \& Social Computing},
  pages={958--968},
  year={2015}
}

@article{post2000ebroidery,
  title={E-broidery: Design and fabrication of textile-based computing},
  author={Post, Ernest Rehmatulla and Orth, Maggie and Russo, Peter R and Gershenfeld, Neil},
  journal={IBM Systems journal},
  volume={39},
  number={3.4},
  pages={840--860},
  year={2000},
  publisher={IBM}
}

@inproceedings{devendorf2017beyond,
  title={Beyond hybrids: Metaphors and margins in design},
  author={Devendorf, Laura and Rosner, Daniela K},
  booktitle={Proceedings of the 2017 Conference on Designing Interactive Systems},
  pages={995--1000},
  year={2017}
}

@inproceedings{devendorf2015being,
  title={Being the machine: reconfiguring agency and control in hybrid fabrication},
  author={Devendorf, Laura and Ryokai, Kimiko},
  booktitle={Proceedings of the 33rd Annual ACM Conference on Human Factors in Computing Systems},
  pages={2477--2486},
  year={2015}
}

@incollection{zoran2013hybrid,
  title={Hybrid basketry: interweaving digital practice within contemporary craft},
  author={Zoran, Amit},
  booktitle={ACM SIGGRAPH 2013 Art Gallery},
  pages={324--331},
  year={2013}
}

@inproceedings{zoran2013freed,
  title={FreeD: a freehand digital sculpting tool},
  author={Zoran, Amit and Paradiso, Joseph A},
  booktitle={Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
  pages={2613--2616},
  year={2013}
}

@inproceedings{tao2017weavemesh,
  title={Weavemesh: A low-fidelity and low-cost prototyping approach for 3d models created by flexible assembly},
  author={Tao, Ye and Wang, Guanyun and Zhang, Caowei and Lu, Nannan and Zhang, Xiaolian and Yao, Cheng and Ying, Fangtian},
  booktitle={Proceedings of the 2017 CHI Conference on Human Factors in Computing Systems},
  pages={509--518},
  year={2017}
}

@book{rosner2018criticalfabulations,
  title={Critical fabulations: reworking the methods and margins of design},
  author={Rosner, Daniela K},
  year={2018},
  publisher={MIT Press}
}

@inproceedings{devendorf2020craftspeople,
  title={Craftspeople as Technical Collaborators: Lessons Learned through an Experimental Weaving Residency},
  author={Devendorf, Laura and Arquilla, Katya and Wirtanen, Sandra and Anderson, Allison and Frost, Steven},
  booktitle={Proceedings of the 2020 CHI Conference on Human Factors in Computing Systems},
  pages={1--13},
  year={2020}
}

@inproceedings{rosner2018corememory,
  title={Making core memory: design inquiry into gendered legacies of engineering and craftwork},
  author={Rosner, Daniela K and Shorey, Samantha and Craft, Brock R and Remick, Helen},
  booktitle={Proceedings of the 2018 CHI Conference on Human Factors in Computing Systems},
  pages={1--13},
  year={2018}
}

@inproceedings{mizrahi2016cooking,
  title={Digital gastronomy: Methods \& recipes for hybrid cooking},
  author={Mizrahi, Moran and Golan, Amos and Mizrahi, Ariel Bezaleli and Gruber, Rotem and Lachnise, Alexander Zoonder and Zoran, Amit},
  booktitle={Proceedings of the 29th Annual Symposium on User Interface Software and Technology},
  pages={541--552},
  year={2016}
}

@inproceedings{jacobs2015hybrid,
  title={Hybrid practice in the Kalahari: design collaboration through digital tools and hunter-gatherer craft},
  author={Jacobs, Jennifer and Zoran, Amit},
  booktitle={Proceedings of the 33rd Annual ACM Conference on Human Factors in Computing Systems},
  pages={619--628},
  year={2015}
}

@book{gershenfeld2008fab,
  title={Fab: the coming revolution on your desktop--from personal computers to personal fabrication},
  author={Gershenfeld, Neil},
  year={2008},
  publisher={Basic Books}
}

@online{sparkfun2018duoskin,
  title =        "Gold Foil Tattoos: Controlling Your Phone With Art",
  howpublished = "\url{http://blog.sparkfuneducation.com/gold-foil-tattoos-controlling-your-phone-with-art}",
  note = {Accessed: 2020-06-10}
}

@inproceedings{bdeir2009littlebits,
  title={Electronics as material: littleBits},
  author={Bdeir, Ayah},
  booktitle={Proceedings of the 3rd International Conference on Tangible and Embedded Interaction},
  pages={397--400},
  year={2009}
}

@article{karuno2016shifu,
  title={Shifu: A Traditional Paper Textile of Japan},
  author={Karuno, Hiroko},
  year={2016}
}

@article{gaver2012annotated,
  title={Annotated portfolios},
  author={Gaver, Bill and Bowers, John},
  journal={interactions},
  volume={19},
  number={4},
  pages={40--49},
  year={2012},
  publisher={ACM New York, NY, USA}
}

@inproceedings{dunne2014social,
  title={The social comfort of wearable technology and gestural interaction},
  author={Dunne, Lucy E and Profita, Halley and Zeagler, Clint and Clawson, James and Gilliland, Scott and Do, Ellen Yi-Luen and Budd, Jim},
  booktitle={2014 36th annual international conference of the IEEE engineering in medicine and biology society},
  pages={4159--4162},
  year={2014},
  organization={IEEE}
}


@online{nsfcareer,
  title =        "NSF Faculty Early Career Development Program (CAREER)",
  howpublished = "\url{https://www.nsf.gov/pubs/2020/nsf20525/nsf20525.htm}",
  note = {Accessed: 2020-06-10}
}


@online{laceweaving,
  title =        "Weaver-Manipulated Lace Weaves",
  howpublished = "\url{https://www.weavezine.com/spring2008/wz\_sp08\_RobynSpady.php.html}",
  note = {Accessed: 2020-06-10}
}

@online{DeflectedDoubleWeave,
  title =        "Handwoven: Deflected Double Weave Technique Series ",
  howpublished = "\url{https://halcyonyarn.com/weaving/5540000E/handwoven-_-deflected-double-weave-_-new-technique-series-_handwoven-ebook-printed-copy}",
  note = {Accessed: 2020-08-01}
}


@online{4hcommonmeasure,
  title =        "4H Common Measures Instruments",
  howpublished = "\url{https://4-h.org/professionals/common-measures/}",
  note = {Accessed: 2020-06-10}
}

@inproceedings{qi2015circuitstickers,
  title={Crafting technology with circuit stickers},
  author={Qi, Jie and Huang, Andrew" bunnie" and Paradiso, Joseph},
  booktitle={Proceedings of the 14th International Conference on Interaction Design and Children},
  pages={438--441},
  year={2015}
}

@inproceedings{hodges2014circuitstickers,
  title={Circuit stickers: peel-and-stick construction of interactive electronic prototypes},
  author={Hodges, Steve and Villar, Nicolas and Chen, Nicholas and Chugh, Tushar and Qi, Jie and Nowacka, Diana and Kawahara, Yoshihiro},
  booktitle={Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
  pages={1743--1746},
  year={2014}
}

@inproceedings{jones2020wearablebits,
  title={Wearable Bits: scaffolding creativity with a prototyping toolkit for wearable e-textiles},
  author={Jones, Lee and Nabil, Sara and McLeod, Amanda and Girouard, Audrey},
  booktitle={Proceedings of the Fourteenth International Conference on Tangible, Embedded, and Embodied Interaction},
  pages={165--177},
  year={2020}
}


@inproceedings{2005lowfloors,
  title={Some reflections on designing construction kits for kids},
  author={Resnick, Mitchel and Silverman, Brian},
  booktitle={Proceedings of the 2005 conference on Interaction design and children},
  pages={117--122},
  year={2005}
}


@inproceedings{searle2015boysneedlework,
  title={Boys' Needlework: Understanding Gendered and Indigenous Perspectives on Computing and Crafting with Electronic Textiles.},
  author={Searle, Kristin A and Kafai, Yasmin B},
  booktitle={ICER},
  pages={31--39},
  year={2015}
}

@article{buechley2012crafting,
  title={Crafting technology: Reimagining the processes, materials, and cultures of electronics},
  author={Buechley, Leah and Perner-Wilson, Hannah},
  journal={ACM Transactions on Computer-Human Interaction (TOCHI)},
  volume={19},
  number={3},
  pages={1--21},
  year={2012},
  publisher={ACM New York, NY, USA}
}

@inproceedings{perner2010kitofnoparts,
  title={Handcrafting textile interfaces from a kit-of-no-parts},
  author={Perner-Wilson, Hannah and Buechley, Leah and Satomi, Mika},
  booktitle={Proceedings of the fifth international conference on Tangible, embedded, and embodied interaction},
  pages={61--68},
  year={2010}
}

@online{futureofworktattoos2020,
  title =        "Office Evolution: Could Microchipped Employees Become The Future of the Workplace?",
  howpublished = "\url{https://www.inverse.com/innovation/microchipped-employees-what-it-would-take}",
  note = {Accessed: 2020-07-30}
}


@online{nationaldefensetattoos2013,
  title =        "Pentagon's Scientists Want a Tattoo That Tracks Troops' Vitals",
  howpublished = "\url{https://www.wired.com/2013/03/sensor-tattoos/}",
  note = {Accessed: 2020-07-30}
}



@online{LorealmyUVpatch2016,
  title =        "L’Oreal My UV Patch",
  howpublished = "\url{http://www.loreal.com/media/pressreleases/2016/jan/loreal-debuts-first-everstretchable-electronic-uv-monitor}",
  note = {Accessed: 2020-07-30}
}


@online{LogicInk,
  title =        "LogicInk",
  howpublished = "\url{http://www.logicink.com}",
  note = {Accessed: 2020-07-30}
}


@online{elderlycare,
  title =        "Technology for Elderly Enhances Health, Safety",
  howpublished = "\url{https://www.agingcare.com/articles/techology-for-elderly-living-at-home-147427.htm}",
  note = {Accessed: 2020-07-30}
}

@article{weiser1999computer,
  title={The computer for the 21st century},
  author={Weiser, Mark},
  journal={ACM SIGMOBILE mobile computing and communications review},
  volume={3},
  number={3},
  pages={3--11},
  year={1999},
  publisher={ACM New York, NY, USA}
}




@online{steam,
  title =        "Science, Technology, Engineering, Arts, and Mathematics (STEAM) Gallery",
  howpublished = "\url{http://www.nsf-i3.org/resources/view/science_technology_engineering_arts_and_mathematics_steam_gallery/}",
  note = {Accessed: 2020-07-30}
}
@online{tessellations,
  title =        "Berber Soepboer and Fioen van Balgooi - Fragment Textiles: 2009",
  howpublished = "\url{https://en.refinity.eu/fragment-textiles.html.}",
  note = {Accessed: 2020-07-30}
}

@article{hur2011tessellations,
  title={Transformative Modular Textile Design},
  author={Hur, ES and Thomas, BG and others},
  journal={Bridges},
  pages={217--224},
  year={2011}
}
@article{wyeth2001electronicblocks,
  title={Electronic blocks: Tangible programming elements for preschoolers},
  author={Wyeth, Peta and Wyeth, Gordon F},
  year={2001},
  publisher={IOC Press}
}

@article{wyeth2008electronicblocks,
  title={How young children learn to program with sensor, action, and logic blocks},
  author={Wyeth, Peta},
  journal={The Journal of the learning sciences},
  volume={17},
  number={4},
  pages={517--550},
  year={2008},
  publisher={Taylor \& Francis}
}


@inproceedings{schweikardt2006roblocks,
  title={roBlocks: a robotic construction kit for mathematics and science education},
  author={Schweikardt, Eric and Gross, Mark D},
  booktitle={Proceedings of the 8th international conference on Multimodal interfaces},
  pages={72--75},
  year={2006}
}


@inproceedings{jones2020swatchbook,
  title={Swatch-bits: Prototyping E-textiles with Modular Swatches},
  author={Jones, Lee and Nabil, Sara and Girouard, Audrey},
  booktitle={Proceedings of the Fourteenth International Conference on Tangible, Embedded, and Embodied Interaction},
  pages={893--897},
  year={2020}
}

@inproceedings{hertenberger2013etextileswatchbook,
  title={2013 e-textile swatchbook exchange: the importance of sharing physical work},
  author={Hertenberger, Anja and Scholz, Barbro and Contrechoc, Beam and Stewart, Becky and Kurbak, Ebru and Perner-Wilson, Hannah and Posch, Irene and Cabral, Isabel and Qi, Jie and Childs, Katharina and others},
  booktitle={Proceedings of the 2014 ACM International Symposium on Wearable Computers: Adjunct Program},
  pages={77--81},
  year={2014}
}
@online{Cubelets,
  title =        "Cubelets",
  howpublished = "\url{http://www.modrobotics.com/cubelets}",
  note = {Accessed: 2020-07-30}
}

@article{bevan2015tinkering,
  title={Learning through STEM-rich tinkering: Findings from a jointly negotiated research project taken up in practice},
  author={Bevan, Bronwyn and Gutwill, Joshua P and Petrich, Mike and Wilkinson, Karen},
  journal={Science Education},
  volume={99},
  number={1},
  pages={98--120},
  year={2015},
  publisher={Wiley Online Library}
}


@inproceedings{jelen2019craftec,
  title={Craftec: Engaging older adults in making through a craft-based toolkit system},
  author={Jelen, Ben and Freeman, Anne and Narayanan, Mina and Sanders, Kate M and Clawson, James and Siek, Katie A},
  booktitle={Proceedings of the Thirteenth International Conference on Tangible, Embedded, and Embodied Interaction},
  pages={577--587},
  year={2019}
}

@online{fabrickit,
  title =        "Fabrickit: DIY Wearable Computing",
  howpublished = "\url{https://boingboing.net/2010/09/29/fabrickit-diy-wearab.html}",
  note = {Accessed: 2020-07-30}
}

@online{cindyhardwarecontacts,
  title =        "Deployment Experiments with Flex PCB and Battery Factories",
  howpublished = "\url{https://www.cindykao.com/Deployments}",
  note = {Accessed: 2020-07-30}
}

@article{haines2014nylonartificial,
  title={Artificial muscles from fishing line and sewing thread},
  author={Haines, Carter S and Lima, M{\'a}rcio D and Li, Na and Spinks, Geoffrey M and Foroughi, Javad and Madden, John DW and Kim, Shi Hyeong and Fang, Shaoli and De Andrade, M{\^o}nica Jung and G{\"o}ktepe, Fatma and others},
  journal={science},
  volume={343},
  number={6173},
  pages={868--872},
  year={2014},
  publisher={American Association for the Advancement of Science}
}

@inproceedings{ivan2016chi,
 author = {Poupyrev, Ivan and Gong, Nan-Wei and Fukuhara, Shiho and Karagozler, Mustafa Emre and Schwesig, Carsten and Robinson, Karen E.},
 title = {Project Jacquard: Interactive Digital Textiles at Scale},
 booktitle = {Proceedings of the 2016 CHI Conference on Human Factors in Computing Systems},
 series = {CHI '16},
 year = {2016},
 isbn = {978-1-4503-3362-7},
 location = {San Jose, California, USA},
 pages = {4216--4227},
 numpages = {12},
 url = {http://doi.acm.org/10.1145/2858036.2858176},
 doi = {10.1145/2858036.2858176},
 acmid = {2858176},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {information interfaces and presentation},
} 

@inproceedings{leong2016procover,
  title={proCover: sensory augmentation of prosthetic limbs using smart textile covers},
  author={Leong, Joanne and Parzer, Patrick and Perteneder, Florian and Babic, Teo and Rendl, Christian and Vogl, Anita and Egger, Hubert and Olwal, Alex and Haller, Michael},
  booktitle={Proceedings of the 29th Annual Symposium on User Interface Software and Technology},
  pages={335--346},
  year={2016}
}

@inproceedings{parzer2017smartsleeve,
  title={SmartSleeve: real-time sensing of surface and deformation gestures on flexible, interactive textiles, using a hybrid gesture detection pipeline},
  author={Parzer, Patrick and Sharma, Adwait and Vogl, Anita and Steimle, J{\"u}rgen and Olwal, Alex and Haller, Michael},
  booktitle={Proceedings of the 30th Annual ACM Symposium on User Interface Software and Technology},
  pages={565--577},
  year={2017}
}

@inproceedings{parzer2018resi,
  title={RESi: A Highly Flexible, Pressure-Sensitive, Imperceptible Textile Interface Based on Resistive Yarns},
  author={Parzer, Patrick and Perteneder, Florian and Probst, Kathrin and Rendl, Christian and Leong, Joanne and Schuetz, Sarah and Vogl, Anita and Schwoediauer, Reinhard and Kaltenbrunner, Martin and Bauer, Siegfried and others},
  booktitle={Proceedings of the 31st Annual ACM Symposium on User Interface Software and Technology},
  pages={745--756},
  year={2018}
}

@inproceedings{zysset2010weaving,
  title={Weaving integrated circuits into textiles},
  author={Zysset, Christoph and Cherenack, Kunigunde and Kinkeldei, Thomas and Tr{\"o}ster, Gerhard},
  booktitle={International Symposium on Wearable Computers (ISWC) 2010},
  pages={1--8},
  year={2010},
  organization={IEEE}
}

@incollection{tomico2013crafting,
  title={Crafting wearables: interaction design meets fashion design},
  author={Tomico, Oscar and van Zijverden, Mascha and Fej{\'e}r, Tom and Chen, Yiyu and Lubbers, Eef and Heuvelings, Meerthe and A{\"\i}ssaoui, Sonia and Schepperheyn, Verena},
  booktitle={CHI'13 Extended Abstracts on Human Factors in Computing Systems},
  pages={2875--2876},
  year={2013}
}


@inproceedings{devendorf2016chi,
 author = {Devendorf, Laura and Lo, Joanne and Howell, Noura and Lee, Jung Lin and Gong, Nan-Wei and Karagozler, M. Emre and Fukuhara, Shiho and Poupyrev, Ivan and Paulos, Eric and Ryokai, Kimiko},
 title = {"I Don'T Want to Wear a Screen": Probing Perceptions of and Possibilities for Dynamic Displays on Clothing},
 booktitle = {Proceedings of the 2016 CHI Conference on Human Factors in Computing Systems},
 series = {CHI '16},
 year = {2016},
 isbn = {978-1-4503-3362-7},
 location = {San Jose, California, USA},
 pages = {6028--6039},
 numpages = {12},
 url = {http://doi.acm.org/10.1145/2858036.2858192},
 doi = {10.1145/2858036.2858192},
 acmid = {2858192},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {ambiguity, clothing-based display, crochet, dynamic textiles, style, weaving},
}


@inproceedings{devendorf2019tei,
 author = {Devendorf, Laura and Di Lauro, Chad},
 title = {Adapting Double Weaving and Yarn Plying Techniques for Smart Textiles Applications},
 booktitle = {Proceedings of the Thirteenth International Conference on Tangible, Embedded, and Embodied Interaction},
 series = {TEI '19},
 year = {2019},
 isbn = {978-1-4503-6196-5},
 location = {Tempe, Arizona, USA},
 pages = {77--85},
 numpages = {9},
 url = {http://doi.acm.org/10.1145/3294109.3295625},
 doi = {10.1145/3294109.3295625},
 acmid = {3295625},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {craft, hand-weaving, smart textiles, yarn plying},
} 

@inproceedings{berzowska2010karma,
  title={Karma chameleon: bragg fiber jacquard-woven photonic textiles},
  author={Berzowska, Joanna and Skorobogatiy, Maksim},
  booktitle={Proceedings of the fourth international conference on Tangible, embedded, and embodied interaction},
  pages={297--298},
  year={2010}
}


@article{granberry2019sma,
  title={Functionally Graded Knitted Actuators with NiTi-Based Shape Memory Alloys for Topographically Self-Fitting Wearables},
  author={Granberry, Rachael and Eschen, Kevin and Holschuh, Brad and Abel, Julianna},
  journal={Advanced Materials Technologies},
  volume={4},
  number={11},
  pages={1900548},
  year={2019},
  publisher={Wiley Online Library}
}


@article{gioberto2013overlockstitch,
  title={Overlock-stitched stretch sensors: characterization and effect of fabric property},
  author={Gioberto, Guido and Dunne, Lucy E},
  journal={Journal of Textile and Apparel, Technology and Management},
  volume={8},
  number={3},
  year={2013}
}

@inproceedings{foo2017bistitch,
  title={Bi-metallic stitched e-textile sensors for sensing salinized liquids},
  author={Foo, Esther W and Pettys-Baker, Robert Mt and Sullivan, Shawn and Dunne, Lucy E},
  booktitle={Proceedings of the 2017 ACM International Symposium on Wearable Computers},
  pages={34--37},
  year={2017}
}






@online{studioforcreativeinquiry_AiR,
  title = "CMU Studio for Creative Inquiry Artist in Residency",
  howpublished = "\url{https://studioforcreativeinquiry.org/wp-content/uploads/2011/02/ArtistResidencyGuidlines.pdf}",
  note = {Accessed: 2020-07-30}
}





@online{subnetAIR,
  title = "University of Salzburg Center for HCI: subnet Artist in Residency",
  howpublished = "\url{https://hci.sbg.ac.at/subnetair/}",
  note = {Accessed: 2020-07-30}
}


@online{Microsoft_AIR,
  title = "Microsoft Research Studio 99 Artist in Residency",
  howpublished = "\url{https://www.microsoft.com/artist-in-residence/}",
  note = {Accessed: 2020-07-30}
}

@online{Google_AIR,
  title = "Google Project Jacquard Artist in Residency",
  howpublished = "\url{https://artsandculture.google.com/story/please-touch-the-thread/YQWRsWXLKfDgvw?hl=en}",
  note = {Accessed: 2020-07-30}
}

@article{ying2012silicon,
  title={Silicon nanomembranes for fingertip electronics},
  author={Ying, Ming and Bonifas, Andrew P and Lu, Nanshu and Su, Yewang and Li, Rui and Cheng, Huanyu and Ameen, Abid and Huang, Yonggang and Rogers, John A},
  journal={Nanotechnology},
  volume={23},
  number={34},
  pages={344004},
  year={2012},
  publisher={IOP Publishing}
}


@online{Autodesk_AIR,
  title = "Autodesk Artist in Residency Program",
  howpublished = "\url{https://www.autodesk.com/technology-centers/residency}",
  note = {Accessed: 2020-07-30}
}


@online{punchlace,
  title = "Knit in Punch Lace",
  howpublished = "\url{http://machineknittingetc.com/knit-in-punch-lace-silver-machine-knitting-institute.html}",
  note = {Accessed: 2020-07-30}
}

@inproceedings{bowers2012logic,
  title={The logic of annotated portfolios: communicating the value of'research through design'},
  author={Bowers, John},
  booktitle={Proceedings of the Designing Interactive Systems Conference},
  pages={68--77},
  year={2012}
}


@inproceedings{dunne2015fashion,
  title={Fashion meets space travel: Engaging girls in STEM through functional apparel design},
  author={Dunne, Lucy E and Morris, Kristen and Reich, Jordyn and Ramaswamy, Harini and Ashdown, Susan P and Kozen, Fran and Coffman, Charlotte},
  year={2015},
  organization={45th International Conference on Environmental Systems}
}

@book{watkins2015functionalclothing,
  title={Functional clothing design: From sportswear to spacesuits},
  author={Watkins, Susan M and Dunne, Lucy},
  year={2015},
  publisher={Bloomsbury Publishing USA}
}

@inproceedings{Kienzle14lightring,
 author = {Kienzle, Wolf and Hinckley, Ken},
 title = {LightRing: Always-available 2D Input on Any Surface},
 booktitle = {Proc. UIST '14},
 year = {2014},
 pages = {157--160},
}

@inproceedings{Silina2015jewelry,
 author = {Silina, Yulia and Haddadi, Hamed},
 title = {New Directions in Jewelry: A Close Look at Emerging Trends and Developments in Jewelry-like Wearable Devices},
 booktitle = {Proc. ISWC '15},
 pages = {49--56},
 year = {2015},
}

@online{IntelMICA,
  title =        "MICA Smart Bracelet Switches on New Fashion, Lifestyle Alerts",
   howpublished =           "\url{https://iq.intel.com/mica-smart-bracelet-switches-on-new-fashion-lifestyle-alerts/}",
   note = {Accessed: 2020-07-30}
}

@article{reeves2015interdiciplineHCI,
  title={Locating the'big hole'in HCI research},
  author={Reeves, Stuart},
  journal={interactions},
  volume={22},
  number={4},
  pages={53--56},
  year={2015},
  publisher={ACM New York, NY, USA}
}


@inproceedings{blackwell2015interdiciplineHCI,
  title={HCI as an Inter-Discipline},
  author={Blackwell, Alan F},
  booktitle={Proceedings of the 33rd Annual ACM Conference Extended Abstracts on Human Factors in Computing Systems},
  pages={503--516},
  year={2015}
}


@incollection{kim1995interdisciplinarycooperation,
  title={Interdisciplinary cooperation},
  author={Kim, Scott},
  booktitle={Readings in Human--Computer Interaction},
  pages={304--311},
  year={1995},
  publisher={Elsevier}
}


@article{blackwell2015filling_interdiciplineHCI,
  title={Filling the big hole in HCI research},
  author={Blackwell, Alan F},
  journal={interactions},
  volume={22},
  number={6},
  pages={37--41},
  year={2015},
  publisher={ACM New York, NY, USA}
}

@article{MedeirosBreathable2019,
author = {Sala de Medeiros, Marina and Chanci, Daniela and Moreno, Carolina and Goswami, Debkalpa and Martinez, Ramses V.},
title = {Waterproof, Breathable, and Antibacterial Self-Powered e-Textiles Based on Omniphobic Triboelectric Nanogenerators},
journal = {Advanced Functional Materials},
volume = {29},
number = {42},
pages = {1904350},
keywords = {energy harvesting, e-textiles, omniphobic fabric, self-powered wearable interfaces, triboelectric nanogenerators},
doi = {https://doi.org/10.1002/adfm.201904350},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/adfm.201904350},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/adfm.201904350},
abstract = {Abstract Multifunctional electronic textiles (e-textiles) incorporating miniaturized electronic devices will pave the way toward a new generation of wearable devices and human–machine interfaces. Unfortunately, the development of e-textiles is subject to critical challenges, such as battery dependence, breathability, satisfactory washability, and compatibility with mass production techniques. This work describes a simple and cost-effective method to transform conventional garments and textiles into waterproof, breathable, and antibacterial e-textiles for self-powered human–machine interfacing. Combining embroidery with the spray-based deposition of fluoroalkylated organosilanes and highly networked nanoflakes, omniphobic triboelectric nanogenerators (RF-TENGs) can be incorporated into any fiber-based textile to power wearable devices using energy harvested from human motion. RF-TENGs are thin, flexible, breathable (air permeability 90.5 mm s−1), inexpensive to fabricate (<0.04\$ cm−2), and capable of producing a high power density (600 µW cm−2). E-textiles based on RF-TENGs repel water, stains, and bacterial growth, and show excellent stability under mechanical deformations and remarkable washing durability under standard machine-washing tests. Moreover, e-textiles based on RF-TENGs are compatible with large-scale production processes and exhibit high sensitivity to touch, enabling the cost-effective manufacturing of wearable human–machine interfaces.},
year = {2019}
}




@article{benford2015HCIturntothecultural,
  title={The ethical implications of HCI's turn to the cultural},
  author={Benford, Steve and Greenhalgh, Chris and Anderson, Bob and Jacobs, Rachel and Golembewski, Mike and Jirotka, Marina and Stahl, Bernd Carsten and Timmermans, Job and Giannachi, Gabriella and Adams, Matt and others},
  journal={ACM Transactions on Computer-Human Interaction (TOCHI)},
  volume={22},
  number={5},
  pages={1--37},
  year={2015},
  publisher={ACM New York, NY, USA}
}


@inproceedings{jacobs2015HCIturntothearts,
  title={Behind The Scenes at HCI's Turn to the Arts},
  author={Jacobs, Rachel and Benford, Steve and Luger, Ewa},
  booktitle={Proceedings of the 33rd Annual ACM Conference Extended Abstracts on Human Factors in Computing Systems},
  pages={567--578},
  year={2015}
}

@book{thomas2014bodyart,
  title={Body art},
  author={Thomas, Nicholas},
  year={2014},
  publisher={Thames \& Hudson World of Art}
}


@inproceedings{rekimoto2001gesturewrist,
  title={Gesturewrist and gesturepad: Unobtrusive wearable interaction devices},
  author={Rekimoto, Jun},
  booktitle={Proceedings Fifth International Symposium on Wearable Computers},
  pages={21--27},
  year={2001},
  organization={IEEE}
}

@phdthesis{kao2018phdthesis,
    Author = {Kao, Hsin-Liu (Cindy)},
    Title = {Hybrid Body Craft},
    School = {Massachusetts Institute of Technology},
    Year = {2018},
}


@book{ryan2014garmentsofparadise,
  title={Garments of paradise: wearable discourse in the digital age},
  author={Ryan, Susan Elizabeth},
  year={2014},
  publisher={MIT Press}
}

@article{starner2001challenges1,
  title={The challenges of wearable computing: Part 1},
  author={Starner, Thad},
  journal={Ieee Micro},
  volume={21},
  number={4},
  pages={44--52},
  year={2001},
  publisher={IEEE}
}

@article{starner2001challenges2,
  title={The challenges of wearable computing: Part 2},
  author={Starner, Thad},
  journal={Ieee Micro},
  volume={21},
  number={4},
  pages={54--67},
  year={2001},
  publisher={IEEE}
}
@article{hsiao_firefighter,
author = {Hongwei Hsiao and Jennifer Whitestone and Tsui-Ying Kau and Brooke Hildreth},
title ={Firefighter Hand Anthropometry and Structural Glove Sizing: A New Perspective},
journal = {Human Factors},
volume = {57},
number = {8},
pages = {1359-1377},
year = {2015},
doi = {10.1177/0018720815594933},
    note ={PMID: 26169309},
}

@BOOK{gupta:anthropometry,
  AUTHOR = "Deepti Gupta and Norsaadah Zakaria",
  TITLE = "Anthropometry, Apparel Sizing and Design",
  PUBLISHER = "Elsevier Science \& Technology",
  ADDRESS = "Cambridge",
  YEAR = "2014"
}

@inproceedings{takaki2020coil,
  title={Coil design for wireless power transfer and communication over hinges of smart glasses},
  author={Takaki, Ken and Sasatani, Takuya and Kasashima, Hironobu and Kawahara, Yoshihiro and Naemura, Takeshi},
  booktitle={Proceedings of the 2020 International Symposium on Wearable Computers},
  pages={79--83},
  year={2020}
}

@article{lin2020wireless,
  title={Wireless battery-free body sensor networks using near-field-enabled clothing},
  author={Lin, Rongzhou and Kim, Han-Joon and Achavananthadith, Sippanat and Kurt, Selman A and Tan, Shawn CC and Yao, Haicheng and Tee, Benjamin CK and Lee, Jason KW and Ho, John S},
  journal={Nature communications},
  volume={11},
  number={1},
  pages={1--10},
  year={2020},
  publisher={Nature Publishing Group}
}

@article{sumiya2019alvus,
  title={Alvus: A reconfigurable 2-d wireless charging system},
  author={Sumiya, Kazunobu and Sasatani, Takuya and Nishizawa, Yuki and Tsushio, Kenji and Narusue, Yoshiaki and Kawahara, Yoshihiro},
  journal={Proceedings of the ACM on Interactive, Mobile, Wearable and Ubiquitous Technologies},
  volume={3},
  number={2},
  pages={1--29},
  year={2019},
  publisher={ACM New York, NY, USA}
}

@inproceedings{jeong2017nfc,
  title={NFC-enabled, tattoo-like stretchable biosensor manufactured by “cut-and-paste” method},
  author={Jeong, Hyoyoung and Ha, Taewoo and Kuang, Irene and Shen, Linxiao and Dai, Zhaohe and Sun, Nan and Lu, Nanshu},
  booktitle={2017 39th Annual International Conference of the IEEE Engineering in Medicine and Biology Society (EMBC)},
  pages={4094--4097},
  year={2017},
  organization={IEEE}
}

@inproceedings{le2019comparison,
  title={A Comparison of Printed Flexible RFID/NFC Antennas for a Microelectronic Measurement System},
  author={Le, Vy and Moser, Patrick and Lemmer, Ulrich and Mackensen, Elke},
  booktitle={2019 IEEE International Conference on RFID Technology and Applications (RFID-TA)},
  pages={49--54},
  year={2019},
  organization={IEEE}
}

@inproceedings{gudan2015ultra,
  title={Ultra-low power 2.4 GHz RF energy harvesting and storage system with- 25dBm sensitivity},
  author={Gudan, Kenneth and Shao, Shuai and Hull, Jonathan J and Ensworth, Joshua and Reynolds, Matthew S},
  booktitle={2015 IEEE international conference on RFID (RFID)},
  pages={40--46},
  year={2015},
  organization={IEEE}
}

@book{yang2006body,
  title={Body sensor networks},
  author={Yang, Guang-Zhong and Yang, Guangzhong},
  volume={1},
  year={2006},
  publisher={Springer}
}

@article{kurs2007wireless,
  title={Wireless power transfer via strongly coupled magnetic resonances},
  author={Kurs, Andre and Karalis, Aristeidis and Moffatt, Robert and Joannopoulos, John D and Fisher, Peter and Solja{\v{c}}i{\'c}, Marin},
  journal={science},
  volume={317},
  number={5834},
  pages={83--86},
  year={2007},
  publisher={American Association for the Advancement of Science}
}

@inproceedings{lin2015wireless,
  title={Wireless power transfer via RFID technology for wearable device applications},
  author={Lin, Ding-Bing and Wang, Tse-Hsuan and Chen, Fu-Jung},
  booktitle={2015 IEEE MTT-S 2015 International Microwave Workshop Series on RF and Wireless Technologies for Biomedical and Healthcare Applications (IMWS-BIO)},
  pages={210--211},
  year={2015},
  organization={IEEE}
}

@inproceedings{bouklachi2019energy,
  title={Energy Harvesting of a NFC Flexible Patch for Medical Applications},
  author={Bouklachi, Madjda and Biancheri-Astier, Marc and Diet, Antoine and Le Bihan, Yann},
  booktitle={2019 IEEE Wireless Power Transfer Conference (WPTC)},
  pages={249--252},
  year={2019},
  organization={IEEE}
}



@inproceedings{molla2017surface,
  title={Surface-mount manufacturing for e-textile circuits},
  author={Molla, Md Tahmidul Islam and Goodman, Steven and Schleif, Nicholas and Berglund, Mary Ellen and Zacharias, Cade and Compton, Crystal and Dunne, Lucy E},
  booktitle={Proceedings of the 2017 ACM International Symposium on Wearable Computers},
  pages={18--25},
  year={2017}
}

@inproceedings{wu2020zebrasense,
  title={ZebraSense: A Double-sided Textile Touch Sensor for Smart Clothing},
  author={Wu, Tony and Fukuhara, Shiho and Gillian, Nicholas and Sundara-Rajan, Kishore and Poupyrev, Ivan},
  booktitle={Proceedings of the 33rd Annual ACM Symposium on User Interface Software and Technology},
  pages={662--674},
  year={2020}
}


@inproceedings{hutchinson2003technologyprobe,
  title={Technology probes: inspiring design for and with families},
  author={Hutchinson, Hilary and Mackay, Wendy and Westerlund, Bo and Bederson, Benjamin B and Druin, Allison and Plaisant, Catherine and Beaudouin-Lafon, Michel and Conversy, St{\'e}phane and Evans, Helen and Hansen, Heiko and others},
  booktitle={Proceedings of the SIGCHI conference on Human factors in computing systems},
  pages={17--24},
  year={2003}
}


@article{Braun_Clarke_2006, 
	title={Using thematic analysis in psychology}, 
	volume={3}, 
	DOI={10.1191/1478088706qp063oa}, 
	number={2}, 
	journal={Qualitative Research in Psychology}, 
	author={Braun Virginia and Clarke Victoria}, 
	year={2006}, 
	pages={77-101}
}


@inproceedings{huang2014technologyprobe,
  title={A technology probe of wearable in-home computer-assisted physical therapy},
  author={Huang, Kevin and Sparto, Patrick J and Kiesler, Sara and Smailagic, Asim and Mankoff, Jennifer and Siewiorek, Dan},
  booktitle={Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
  pages={2541--2550},
  year={2014}
}

@inproceedings{molla2018launderability,
  title={Launderability of surface-insulated cut and sew E-textiles},
  author={Molla, Md Tahmidul Islam and Compton, Crystal and Dunne, Lucy E},
  booktitle={Proceedings of the 2018 ACM International Symposium on Wearable Computers},
  pages={104--111},
  year={2018}
}

@article{tao2017make,
  title={How to make reliable, washable, and wearable textronic devices},
  author={Tao, Xuyuan and Koncar, Vladan and Huang, Tzu-Hao and Shen, Chien-Lung and Ko, Ya-Chi and Jou, Gwo-Tsuen},
  journal={Sensors},
  volume={17},
  number={4},
  pages={673},
  year={2017},
  publisher={Multidisciplinary Digital Publishing Institute}
}



@article{abowd2020internetofmaterails,
  title={The Internet of Materials: A Vision for Computational Materials},
  author={Abowd, Gregory D},
  journal={IEEE Annals of the History of Computing},
  volume={19},
  number={02},
  pages={56--62},
  year={2020},
  publisher={IEEE Computer Society}
}

@article{lazaro2019battery,
  title={Battery-Less Smart Diaper Based on NFC Technology},
  author={Lazaro, Antonio and Boada, Marti and Villarino, Ramon and Girbau, David},
  journal={IEEE Sensors Journal},
  volume={19},
  number={22},
  pages={10848--10858},
  year={2019},
  publisher={IEEE}
}

@article{boada2018battery,
  title={Battery-less soil moisture measurement system based on a NFC device with energy harvesting capability},
  author={Boada, Mart{\'\i} and Lazaro, Antonio and Villarino, Ramon and Girbau, David},
  journal={IEEE Sensors Journal},
  volume={18},
  number={13},
  pages={5541--5549},
  year={2018},
  publisher={IEEE}
}

@inproceedings{wang2018skin+,
  title={SKIN+ Fabricating Soft Fluidic User Interfaces for Enhancing On-Skin Experiences and Interactions},
  author={Wang, Yanan and Luo, Shijian and Gong, Hebo and Xu, Fei and Chen, Rujia and Liu, Shuai and Hansen, Preben},
  booktitle={Extended Abstracts of the 2018 CHI Conference on Human Factors in Computing Systems},
  pages={1--6},
  year={2018}
}

@article{alharbi2018flexible,
  title={Flexible antennas for wearable applications: Recent advances and design challenges},
  author={Alharbi, Saad and Shubair, Raed M and Kiourti, Asimina},
  year={2018},
  publisher={IET}
}

@article{leung2007performance,
  title={Performance of printed polymer-based RFID antenna on curvilinear surface},
  author={Leung, Stanley YY and Lam, David CC},
  journal={IEEE transactions on electronics packaging manufacturing},
  volume={30},
  number={3},
  pages={200--205},
  year={2007},
  publisher={IEEE}
}

@article{ortego2012inkjet,
  title={Inkjet printed planar coil antenna analysis for NFC technology applications},
  author={Ortego, I and Sanchez, N and Garcia, J and Casado, F and Valderas, D and Sancho, JI},
  journal={International Journal of Antennas and Propagation},
  volume={2012},
  year={2012},
  publisher={Hindawi}
}

@article{tran2010copper,
  title={Copper thin film for RFID UHF antenna on flexible substrate},
  author={Tran, Nhan Ai and Tran, Huy Nam and Dang, Mau Chien and Fribourg-Blanc, Eric},
  journal={Advances in Natural Sciences: Nanoscience and Nanotechnology},
  volume={1},
  number={2},
  pages={025016},
  year={2010},
  publisher={IOP Publishing}
}

@article{dejean2005liquid,
  title={Liquid crystal polymer (LCP): A new organic material for the development of multilayer dual-frequency/dual-polarization flexible antenna arrays},
  author={DeJean, G and Bairavasubramanian, R and Thompson, D and Ponchak, GE and Tentzeris, MM and Papapolymerou, J},
  journal={IEEE Antennas and Wireless Propagation Letters},
  volume={4},
  pages={22--26},
  year={2005},
  publisher={IEEE}
}

@article{kiourti2015fabrication,
  title={Fabrication of textile antennas and circuits with 0.1 mm precision},
  author={Kiourti, Asimina and Lee, Cedric and Volakis, John L},
  journal={IEEE Antennas and Wireless Propagation Letters},
  volume={15},
  pages={151--153},
  year={2015},
  publisher={IEEE}
}

@article{kiourti2014high,
  title={High-geometrical-accuracy embroidery process for textile antennas with fine details},
  author={Kiourti, Asimina and Volakis, John L},
  journal={IEEE Antennas and Wireless Propagation Letters},
  volume={14},
  pages={1474--1477},
  year={2014},
  publisher={IEEE}
}

@inproceedings{ozbek2018novel,
  title={Novel manufacturing of advanced smart garments: knitting with spatially-varying, multi-material monofilament},
  author={Ozbek, Simon and Molla, Md Tahmidul Islam and Compton, Crystal and Holschuh, Brad},
  booktitle={Proceedings of the 2018 ACM International Symposium on Wearable Computers},
  pages={120--127},
  year={2018}
}

@inproceedings{he2020plotting,
  title={Plotting with Thread: Fabricating Delicate Punch Needle Embroidery with XY Plotters},
  author={He, Shiqing and Adar, Eytan},
  booktitle={Proceedings of the 2020 ACM Designing Interactive Systems Conference},
  pages={1047--1057},
  year={2020}
}

@inproceedings{goveia2020crafting,
  title={Crafting Research Products through Digital Machine Embroidery},
  author={Goveia da Rocha, Bruna and Tomico, Oscar and Markopoulos, Panos and Tetteroo, Daniel},
  booktitle={Proceedings of the 2020 ACM Designing Interactive Systems Conference},
  pages={341--350},
  year={2020}
}

@inproceedings{goudswaard2020fabriclick,
  title={FabriClick: Interweaving Pushbuttons into Fabrics Using 3D Printing and Digital Embroidery},
  author={Goudswaard, Maas and Abraham, Abel and Goveia da Rocha, Bruna and Andersen, Kristina and Liang, Rong-Hao},
  booktitle={Proceedings of the 2020 ACM Designing Interactive Systems Conference},
  pages={379--393},
  year={2020}
}


@online{futureofworktattoos2020,
  title =        "Office Evolution: Could Microchipped Employees Become The Future of the Workplace?",
  howpublished = "\url{https://www.inverse.com/innovation/microchipped-employees-what-it-would-take}",
  note = {Accessed: 2020-07-30}
}

@inproceedings{yoo2009attachable,
  title={An attachable ECG sensor bandage with planar-fashionable circuit board},
  author={Yoo, Jerald and Yan, Long and Lee, Seulki and Kim, Hyejung and Kim, Binhee and Yoo, Hoi-Jun},
  booktitle={2009 International Symposium on Wearable Computers},
  pages={145--146},
  year={2009},
  organization={IEEE}
}

@inproceedings{arora2018zeusss,
  title={ZEUSSS: Zero energy ubiquitous sound sensing surface leveraging triboelectric nanogenerator and analog backscatter communication},
  author={Arora, Nivedita and Abowd, Gregory D},
  booktitle={The 31st Annual ACM Symposium on User Interface Software and Technology Adjunct Proceedings},
  pages={81--83},
  year={2018}
}

@inproceedings{profita2013e-textileperception,
  title={Don't mind me touching my wrist: a case study of interacting with on-body technology in public},
  author={Profita, Halley P and Clawson, James and Gilliland, Scott and Zeagler, Clint and Starner, Thad and Budd, Jim and Do, Ellen Yi-Luen},
  booktitle={Proceedings of the 2013 International Symposium on Wearable Computers},
  pages={89--96},
  year={2013}
}

@article{locher2007fundamental,
  title={Fundamental building blocks for circuits on textiles},
  author={Locher, Ivo and Troster, Gerhard},
  journal={IEEE Transactions on advanced packaging},
  volume={30},
  number={3},
  pages={541--550},
  year={2007},
  publisher={IEEE}
}

@article{yang2009handling,
  title={Handling movement epenthesis and hand segmentation ambiguities in continuous sign language recognition using nested dynamic programming},
  author={Yang, Ruiduo and Sarkar, Sudeep and Loeding, Barbara},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={32},
  number={3},
  pages={462--477},
  year={2009},
  publisher={IEEE}
}

@inproceedings{uebersax2011real,
  title={Real-time sign language letter and word recognition from depth data},
  author={Uebersax, Dominique and Gall, Juergen and Van den Bergh, Michael and Van Gool, Luc},
  booktitle={2011 IEEE international conference on computer vision workshops (ICCV Workshops)},
  pages={383--390},
  year={2011},
  organization={IEEE}
}

@inproceedings{frati2011using,
  title={Using Kinect for hand tracking and rendering in wearable haptics},
  author={Frati, Valentino and Prattichizzo, Domenico},
  booktitle={2011 IEEE World Haptics Conference},
  pages={317--321},
  year={2011},
  organization={IEEE}
}

@inproceedings{hu2010hand,
  title={Hand pointing estimation for human computer interaction based on two orthogonal-views},
  author={Hu, Kaoning and Canavan, Shaun and Yin, Lijun},
  booktitle={2010 20th International Conference on Pattern Recognition},
  pages={3760--3763},
  year={2010},
  organization={IEEE}
}

@inproceedings{nittala2020physioskin,
  title={PhysioSkin: Rapid Fabrication of Skin-Conformal Physiological Interfaces},
  author={Nittala, Aditya Shekhar and Khan, Arshad and Kruttwig, Klaus and Kraus, Tobias and Steimle, J{\"u}rgen},
  booktitle={Proceedings of the 2020 CHI Conference on Human Factors in Computing Systems},
  pages={1--10},
  year={2020}
}

@inproceedings{nittala2018multi,
  title={Multi-touch skin: A thin and flexible multi-touch sensor for on-skin input},
  author={Nittala, Aditya Shekhar and Withana, Anusha and Pourjafarian, Narjes and Steimle, J{\"u}rgen},
  booktitle={Proceedings of the 2018 CHI Conference on Human Factors in Computing Systems},
  pages={1--12},
  year={2018}
}

@inproceedings{aigner2020embroidered,
  title={Embroidered resistive pressure sensors: A novel approach for textile interfaces},
  author={Aigner, Roland and Pointner, Andreas and Preindl, Thomas and Parzer, Patrick and Haller, Michael},
  booktitle={Proceedings of the 2020 CHI Conference on Human Factors in Computing Systems},
  pages={1--13},
  year={2020}
}



@inproceedings{kim2023knitdema,
  title={Knitdema: robotic textile as personalized edema mobilization device},
  author={Kim, Jin Hee and Stilling, Joan and O'Dell, Michael and Kao, Cindy Hsin-Liu},
  booktitle={Proceedings of the 2023 CHI Conference on Human Factors in Computing Systems},
  pages={1--19},
  year={2023}
}


@inproceedings{kim2021knitdermis,
  title={KnitDermis: Fabricating tactile on-body interfaces through machine knitting},
  author={Kim, Jin Hee and Huang, Kunpeng and White, Simone and Conroy, Melissa and Kao, Cindy Hsin-Liu},
  booktitle={Proceedings of the 2021 ACM Designing Interactive Systems Conference},
  pages={1183--1200},
  year={2021}
}


@inproceedings{kim2022knitskin,
  title={Knitskin: machine-knitted scaled skin for locomotion},
  author={Kim, Jin Hee and Patil, Shreyas Dilip and Matson, Sarina and Conroy, Melissa and Kao, Cindy Hsin-Liu},
  booktitle={Proceedings of the 2022 CHI Conference on Human Factors in Computing Systems},
  pages={1--15},
  year={2022}
}


@inproceedings{olwal2020textile,
  title={E-textile microinteractions: Augmenting twist with flick, slide and grasp gestures for soft electronics},
  author={Olwal, Alex and Starner, Thad and Mainini, Gowa},
  booktitle={Proceedings of the 2020 CHI Conference on Human Factors in Computing Systems},
  pages={1--13},
  year={2020}
}


@inproceedings{forman2019modifiber,
  title={Modifiber: Two-way morphing soft thread actuators for tangible interaction},
  author={Forman, Jack and Tabb, Taylor and Do, Youngwook and Yeh, Meng-Han and Galvin, Adrian and Yao, Lining},
  booktitle={Proceedings of the 2019 CHI Conference on Human Factors in Computing Systems},
  pages={1--11},
  year={2019}
}

@inproceedings{kilic2021omnifiber,
  title={OmniFiber: Integrated fluidic fiber actuators for weaving movement based interactions into the ‘fabric of everyday life’},
  author={Kilic Afsar, Ozgun and Shtarbanov, Ali and Mor, Hila and Nakagaki, Ken and Forman, Jack and Modrei, Karen and Jeong, Seung Hee and Hjort, Klas and H{\"o}{\"o}k, Kristina and Ishii, Hiroshi},
  booktitle={The 34th Annual ACM Symposium on User Interface Software and Technology},
  pages={1010--1026},
  year={2021}
}

@inproceedings{forman2023fiberobo,
  title={FibeRobo: Fabricating 4D Fiber Interfaces by Continuous Drawing of Temperature Tunable Liquid Crystal Elastomers},
  author={Forman, Jack and Kilic Afsar, Ozgun and Nicita, Sarah and Lin, Rosalie Hsin-Ju and Yang, Liu and Hofmann, Megan and Kothakonda, Akshay and Gordon, Zachary and Honnet, Cedric and Dorsey, Kristen and others},
  booktitle={Proceedings of the 36th Annual ACM Symposium on User Interface Software and Technology},
  pages={1--17},
  year={2023}
}


%_______ABOVE: KAO References_______

@inproceedings{AroraZeusss,
author = {Arora, Nivedita and Abowd, Gregory D.},
title = {ZEUSSS: Zero Energy Ubiquitous Sound Sensing Surface Leveraging Triboelectric Nanogenerator and Analog Backscatter Communication},
year = {2018},
isbn = {9781450359498},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3266037.3266108},
doi = {10.1145/3266037.3266108},
abstract = {ZEUSSS (Zero Energy Ubiquitous Sound Sensing Surface), allows physical objects and surfaces to be instrumented with a thin, self-sustainable material that provides acoustic sensing and communication capabilities. We have built a prototype ZEUSSS tag using minimal hardware and flexible electronic components, extending our original self-sustaining SATURN microphone with a printed, flexible antenna to support passive communication via analog backscatter. ZEUSSS enables objects to have ubiquitous wire-free battery-free audio based context sensing, interaction, and surveillance capabilities.},
booktitle = {Adjunct Proceedings of the 31st Annual ACM Symposium on User Interface Software and Technology},
pages = {81–83},
numpages = {3},
keywords = {teng (triboelectric nanogenerator), flexible electronics, battery-free microphone, analog backscatter communication},
location = {Berlin, Germany},
series = {UIST '18 Adjunct}
}

@inproceedings{TriboTribe,
author = {Liu, Xin and Han, Bo and Zheng, Clement and Yen, Ching Chiuan},
title = {Tribo Tribe: Triboelectric Interaction Sensing with 3D Physical Interfaces},
year = {2022},
isbn = {9781450391566},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3491101.3519759},
doi = {10.1145/3491101.3519759},
abstract = {This research introduces “Tribo Tribe”, a technique for fabricating 3D tangible interactive interfaces capable of sensing movement inputs through ubiquitous materials. Tribo Tribe is built on the working principle of Triboelectric Nanogenerators (TENG) to enable self-powered sensing to 3D systems. We introduce a tool kit that facilitates designers and makers to easily customise both prototyping and sensing through TENG technology. We also demonstrate four design possibilities for different fields to illustrate how Tribo Tribe can instrument TENG into 3D physical interactive prototypes (Figure 1).},
booktitle = {Extended Abstracts of the 2022 CHI Conference on Human Factors in Computing Systems},
articleno = {272},
numpages = {6},
keywords = {3D Systems, Self-powered Sensing, TENG, Tangible Interaction, ubiquitous materials.},
location = {New Orleans, LA, USA},
series = {CHI EA '22}
}

@inproceedings{Harrison-OmniTouch,
author = {Harrison, Chris and Benko, Hrvoje and Wilson, Andrew D.},
title = {OmniTouch: wearable multitouch interaction everywhere},
year = {2011},
isbn = {9781450307161},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/2047196.2047255},
doi = {10.1145/2047196.2047255},
abstract = {OmniTouch is a wearable depth-sensing and projection system that enables interactive multitouch applications on everyday surfaces. Beyond the shoulder-worn system, there is no instrumentation of the user or environment. Foremost, the system allows the wearer to use their hands, arms and legs as graphical, interactive surfaces. Users can also transiently appropriate surfaces from the environment to expand the interactive area (e.g., books, walls, tables). On such surfaces - without any calibration - OmniTouch provides capabilities similar to that of a mouse or touchscreen: X and Y location in 2D interfaces and whether fingers are "clicked" or hovering, enabling a wide variety of interactions. Reliable operation on the hands, for example, requires buttons to be 2.3cm in diameter. Thus, it is now conceivable that anything one can do on today's mobile devices, they could do in the palm of their hand.},
booktitle = {Proceedings of the 24th Annual ACM Symposium on User Interface Software and Technology},
pages = {441–450},
numpages = {10},
keywords = {on-demand interfaces, on-body computing, object classification, finger tracking, appropriated surfaces},
location = {Santa Barbara, California, USA},
series = {UIST '11}
}

@INPROCEEDINGS{SmartGlasses,
  author={Feng Lan and Guangtao Zhai and Wei Lin},
  booktitle={TENCON 2015 - 2015 IEEE Region 10 Conference}, 
  title={Lightweight smart glass system with audio aid for visually impaired people}, 
  year={2015},
  volume={},
  number={},
  pages={1-4},
  keywords={Glass;Feature extraction;Blindness;Streaming media;Cities and towns;Prototypes;Headphones;Smart glass system;Intel Edison;blindness;public signs recognition},
  doi={10.1109/TENCON.2015.7372720}}


@inproceedings{olwalsmartglasses,
author = {Olwal, Alex and Balke, Kevin and Votintcev, Dmitrii and Starner, Thad and Conn, Paula and Chinh, Bonnie and Corda, Benoit},
title = {Wearable Subtitles: Augmenting Spoken Communication with Lightweight Eyewear for All-day Captioning},
year = {2020},
isbn = {9781450375146},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3379337.3415817},
doi = {10.1145/3379337.3415817},
abstract = {Mobile solutions can help transform speech and sound into visual representations for people who are deaf or hard-of-hearing (DHH). However, where handheld phones present challenges, head-worn displays (HWDs) could further communication through privately transcribed text, hands-free use, improved mobility, and socially acceptable interactions.  Wearable Subtitles is a lightweight 3D-printed proof-of-concept HWD that explores augmenting communication through sound transcription for a full workday. Using a low-power microcontroller architecture, we enable up to 15 hours of continuous use. We describe a large survey (n=501) and three user studies with 24 deaf/hard-of-hearing participants which inform our development and help us refine our prototypes. Our studies and prior research identify critical challenges for the adoption of HWDs which we address through extended battery life, lightweight and balanced mechanical design (54 g), fitting options, and form factors that are compatible with current social norms.},
booktitle = {Proceedings of the 33rd Annual ACM Symposium on User Interface Software and Technology},
pages = {1108–1120},
numpages = {13},
keywords = {all-day, assistive technology, captions, head-worn displays, hearing accessibility, low-power system, wearables},
location = {Virtual Event, USA},
series = {UIST '20}
}

@book{braun2012thematic,
  title={Thematic analysis.},
  author={Braun, Virginia and Clarke, Victoria},
  year={2012},
  publisher={American Psychological Association}
}

@article{su2021self,
  title={Self-powered respiration monitoring enabled by a triboelectric nanogenerator},
  author={Su, Yuanjie and Chen, Guorui and Chen, Chunxu and Gong, Qichen and Xie, Guangzhong and Yao, Mingliang and Tai, Huiling and Jiang, Yadong and Chen, Jun},
  journal={Advanced Materials},
  volume={33},
  number={35},
  pages={2101262},
  year={2021},
  publisher={Wiley Online Library}
}

@article{feng2022highly,
  title={Highly wearable, machine-washable, and self-cleaning fabric-based triboelectric nanogenerator for wireless drowning sensors},
  author={Feng, Min and Wu, Yang and Feng, Yange and Dong, Yang and Liu, Yubo and Peng, Jialiang and Wang, Nannan and Xu, Shiwei and Wang, Daoai},
  journal={Nano Energy},
  volume={93},
  pages={106835},
  year={2022},
  publisher={Elsevier}
}

@article{younes2023smart,
  title={Smart E-textiles: A review of their aspects and applications},
  author={Younes, Basel},
  journal={Journal of Industrial Textiles},
  volume={53},
  pages={15280837231215493},
  year={2023},
  publisher={SAGE Publications Sage UK: London, England}
}
